Multiple Model Synchronization with Multiary Delta Lenses with Amendment and K-Putput

Multiple (more than 2) model synchronization is ubiquitous and important for model driven engineering, but its theoretical underpinning gained much less attention than the binary case. Specifically, the latter was extensively studied by the bx community in the framework of algebraic models for update propagation called lenses. Now we make a step to restore the balance and propose a notion of multiary delta lens. Besides multiarity, our lenses feature {\em reflective} updates, when consistency restoration requires some amendment of the update that violated consistency. We emphasize the importance of various ways of lens composition for practical applications of the framework, and prove several composition results.

==> figures/diags/alnFwk.tex <==
%\newarrow{Updto}{<}---{>}
\newarrow{Updto}----{>}


%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure*}
\centering
\begin{tabular}{c@{\qquad}c@{\qquad}c}
\begin{diagram}[w=2em,h=1.5em] %(a)
\dbox{A}&& \rCorrto^r &&\dbox{B}\\%
&\seTilearrow{\falt} &&\ldDercorrto(4,4)~{a{*}r}&\\
\dUpdto<a & && &\\%
&&&&\\
\dbox{A'} & &&&
\end{diagram}%
&% --- 2nd column
\begin{diagram}[w=2em,h=1.5em] %(b)
\dbox{A} && \rCorrto^r &&\dbox{B}\\%
&\rdDercorrto(4,4)~{r{*}b} &&\swTilearrow{\balt}\quad~~&\\%
& &&&\dUpdto>b \\%
&&&&\\
&&&&\dbox{B'}
\end{diagram}%
&% -- 3rd column -------
\begin{diagram} %(c)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\dUpdto<a %
& %
\ruDercorrto^{a{*}r~~~~~~~}\luDercorrto^{~~~~~~r{*}b}%
& \dUpdto>b \\%
\dbox{A'} & \rDercorrto^{r'} &\dbox{B'}
\end{diagram}%
\\[50pt]
\multicolumn{2}{c}{%
(a)  arities %
} &
(b) (\asslaw) law
    %\falt{};\balt{} = \balt{};\falt{} %
\end{tabular}
\caption{Alignment operations and their laws \label{fig:align-oper}}%
\end{figure*}
%\vspace{-7ex}
%\end{wrapfigure}


==> figures/diags/binary/ppgPatterns-12.tex <==
%-- version with letters A,B
\cellW=8.0ex%
\cellH=5.0ex
%\begin{figure}[t]
%\centering
\begin{wrapfigure}{L}{0.55\textwidth}
	%	\vspace{-1cm}
	\centering
\begin{tabular}{c@{\qquad}c} %@{\qquad}c} 
%-- cell 11 (row,col) -
\begin{diagram}[w=1.\cellW,h=1.\cellH] 
%%(a) % was 1.1\cellW, 1.1\cellH
%\dbox{A_1} & \rCorrto^r &\dbox{A_2}\\%
%\dUpdto<{u_1} & \seTilearrow{\ppgx{12}}~~~
%            & \dDerupdto>{u'_2} \\%
%\dbox{A'_1} & \rDercorrto^{r'} & A'_2
%\end{diagram}%
%& % column 2 for two rows
%\multirow{2}{*}{%
\begin{diagram}[w=1.1\cellW,h=\cellH] % now (c) was (d)
\dbox{A_1} & \rCorrto^{r} & \dbox{A_2}\\%
\dUpdto<{u_1} && \\
\dbox{A'_1}& \seTilearrow{\rppgx{12}}~~~
            & \dDerupdto>{u'_2} \\%
\dDerupdto<{u'_1} && \\
A''_1 & \rDercorrto^{r''} & A''_2
\end{diagram}%
%}% end multirow
&
%& % column 3 for two rows
%\multirow{2}{*}{%
\begin{diagram}[w=1.1\cellW,h=\cellH] % now (c) was (d)
\dbox{A_1} & \rCorrto^{r} & \dbox{A_2}\\%
%\dUpdto<{u_1} 
&& \dUpdto>{u_2}\\
\dDerupdto>{u'_1} & \swTilearrow{\rppgx{21}}\qquad
            & \dbox{A'_2}\\%
&&\dDerupdto>{u'_2}  \\
A''_1 & \rDercorrto^{r''} & A''_2
\end{diagram}%
%}% end multirow
%\\[30pt]
%&
%%-- cell 21
%\begin{diagram}[w=\cellW,h=\cellH] %(b)
%\dbox{A_1} & \rCorrto^r & \dbox{A_2}\\%
%\dDerupdto<{u'_1} & \swTilearrow{\ppgx{21}}~~~
%            & \dUpdto>{u_2} \\%
%A'_1 & \rDercorrto^{r'} & \dbox{A'_2}
%\end{diagram}%
%& & \\[35pt]
\\ [25pt]
(b1) & (b2)
%\multicolumn{2}{c}{(b)} 
%& %
%%%(c) f-commutativity &
%\multicolumn{2}{c}{(c) monotonicity laws}
\end{tabular}
\vspace{-0.25cm}
\caption{Reflective update propagation
\label{fig:ppgPatterns-reflect}}%
\vspace{-0.5cm}
\end{wrapfigure}


%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/binary/ppgPatterns-3.tex <==
%-- version with letters A,B
\cellW=8.0ex%
\cellH=8.0ex
\begin{figure}[t]
\centering
\begin{tabular}{c@{\qquad}c} %@{\qquad}c} 
\begin{diagram}[w=1.1\cellW,h=0.85\cellH] 
\dbox{A_1} & \rCorrto^{r} & \dbox{A_2}\\%
\dUpdto<{u_1} &
\seTilearrow{\alnx{10}} &
\dDLine>{\id_{A_2}}\\
\dbox{A'_1}
& 
\pile{\rDercorrto^{u_1{*}r} \\ 
\Downarrow\alpha_{10} \\ 
\rCorrto_{r'}}% end pile
& \dbox{A_2}
\\%
%\dbox{A'_1}& %\seTilearrow{\ppg{12}}~~~
\dDerupdto<{u'_1}&\seTilearrow{\rrstx{12}}& \dDerupdto>{u'_2} \\%
A''_1 & \rDercorrto^{r''} & A'_2
\end{diagram}
& %
\begin{diagram}[w=1.1\cellW,h=0.85\cellH] 
\dbox{A_1} & \rCorrto^{r} & \dbox{A_2}\\%
\dDLine<{\id_{A_1}}  &
\swTilearrow{\alnx{20}} &
\dUpdto>{u_2}\\
\dbox{A_1}
& 
\pile{\rDercorrto^{r*u_2} \\ 
\Downarrow\alpha_{20} \\ 
\rCorrto_{r'}}% end pile
& \dbox{A'_2}
\\%
%\dbox{A'_1}& %\seTilearrow{\ppg{12}}~~~
\dDerupdto<{u'_1} &
\swTilearrow{\rrstx{21}} & 
\dDerupdto>{u'_2} \\%
A''_1 & \rDercorrto^{r''} & A'_2
\end{diagram}
\\[55pt]
(c1) & (c2) 
\end{tabular}
\caption{Patterns of update propagation continued
\label{fig:ppgPatterns-3}
}%
\end{figure}

\endinput

==> figures/diags/binary/ppgPatterns-reflect.tex <==
\cellW=7.5ex %8.0ex%
\cellH=5.0ex
%\begin{figure}[t]
%\centering
\begin{wrapfigure}{L}{0.3\textwidth}
	\vspace{-0.5cm}
	\centering
\begin{tabular}{c} %{\quad}c} %@{\qquad}c} 
%\multirow{2}{*}{%
\begin{diagram}[w=1.1\cellW,h=\cellH] % now (c) was (d)
\dbox{A_i} & \rCorrto^{r} & \dbox{A_j}\\%
\dUpdto<{u_i} && \\
\dbox{A'_i}& \seTilearrow{\rppgx{ij}}~~~
            & \dDerupdto>{u'_j} \\%
\dDerupdto<{u'_i} && \\
A''_i & \rDercorrto^{r''} & A''_j
\end{diagram}%
%%%%}% end multirow
% ----
%&  % column 3 for two rows
%%\multirow{2}{*}{%
%\begin{diagram}[w=1.1\cellW,h=\cellH] % now (c) was (d)
%\dbox{A_1} & \rCorrto^{r} & \dbox{A_2}\\%
%%\dUpdto<{u_1} 
%&& \dUpdto>{u_2}\\
%\dDerupdto>{u'_1} & \swTilearrow{\rppgx{21}}\qquad
%            & \dbox{A'_2}\\%
%&&\dDerupdto>{u'_2}  \\
%A''_1 & \rDercorrto^{r''} & A''_2
%\end{diagram}%
%%}% end multirow
\\ [25pt]
%(b1) $j\noteq i$& (b2)
%\multicolumn{2}{c}{(b)} 
%& %
%%%(c) f-commutativity &
%\multicolumn{2}{c}{(c) monotonicity laws}
\end{tabular}
\vspace{-0.25cm}
\caption{$j\noteq i$ %Reflective update propagation
\label{fig:ppgPatterns-reflect}}%
\vspace{-0.5cm}
\end{wrapfigure}
%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/binary/ppgPatterns-simple.tex <==
\cellW=7.25ex%
\cellH=5.0ex
%\begin{figure}
%\centering
\begin{wrapfigure}{L}{0.275\textwidth}
%	\vspace{-1cm}
	\centering
\begin{tabular}{c} %@{\quad}c}%@{\qquad}c} 
%@{\quad}c@{\quad}c}
%-- cell 11 (row,col) -
\begin{diagram}[w=1.\cellW,h=1.\cellH] 
%(a) % was 1.1\cellW, 1.1\cellH
\dbox{A_i} & \rCorrto^r &\dbox{A_j}\\%
\dUpdto<{u_i} & \seTilearrow{\ppgx{ij}}~~~
            & \dDerupdto>{u'_j} \\%
\dbox{A'_i} & \rDercorrto^{r'} & A'_j
\end{diagram}%
%&  % cxell 12
%\begin{diagram}[w=\cellW,h=\cellH] %(b)
%\dbox{A_i} & \rCorrto^r & \dbox{A_2}\\%
%\dDerupdto<{u'_i} & \swTilearrow{\ppgx{2i}}~~~
%            & \dUpdto>{u_2} \\%
%A'_i & \rDercorrto^{r'} & \dbox{A'_2}
%\end{diagram}%
%%\\ [25pt]
%%a1) $i=2,3,4$ & (a2) $i=1,3,4$
%%& (b1) & (b2)
\end{tabular}
\vspace{-0.25cm}
\caption{$j\noteq i$ %Simple update propagation
\label{fig:ppgPatterns-simple}}%
\vspace{-0.5cm}
\end{wrapfigure}
%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/lensDef.tex <==
\cellW=7.ex%
\cellH=5.0ex
%\begin{wrapfigure}{L}{0.47\textwidth}
%\vspace{-3ex}
%	\centering
\begin{diagram}[w=1.\cellW,h=1.\cellH] 
\dbox{\tupA} &\lMapsto^{\quad{:}\prt} & \dbox{R}
\\
\dTo>{\tupu} &&
\\
\dbox{\tupA'} && \dDerupdto >{\tupu''}
\\
\dDerupdto>{\tupu'}	&&
\\
%(A''_1..A''_n)
\tupA'' &\lDermapsto^{\quad{:}\prt} & R''
\\
\end{diagram}%
%%\vspace{-1.ex}
%\caption{Update propagation arity\label{fig:ppgAr}}
%\vspace{-4ex}
%\end{wrapfigure}
%%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/mergeDef.tex <==

\cellW=7.25ex%
\cellH=5.0ex
%\begin{figure} \centering
%\begin{wrapfigure}{R}{0.4\textwidth}%\vspace{-3ex}
%	\centering
\begin{equation}\label{eq:mergeDef}
\begin{diagram}[w=1.\cellW,h=0.65\cellH] 
	&&\dbox{A}&&\\  % row1
	&\ldTo^{u_1}&\dots&\rdTo^{u_n}&\\ % row 2
	\dbox{A'_1}&&[\merge]&& \dbox{A'_n}\\   %row 3
		&\rdDerupdto^{u'_1}&\dots&\ldDerupdto^{u'_n}&\\ % row 4
		&&{A''}&&\\  % row5
\end{diagram}%
\end{equation}
%\vspace{-1.ex}
%\caption{Update merging}\label{fig:updMerge}
%\vspace{-4ex}
%\end{wrapfigure}
%\end{figure}

\endinput

% prep for a better version to show the diagonal 
\begin{equation}\label{eq:mergeDef}
\begin{diagram}[w=1.\cellW,h=0.65\cellH] 
&&\dbox{A}&&\\  % row1
&\ldTo^{u_1}&\dots&\rdTo^{u_n}&\\ % row 2
\dbox{A'_1}&&[\merge]&& \dbox{A'_n}\\   %row 3
&\rdDerupdto^{u'_1}&\dots&\ldDerupdto^{u'_n}&\\ % row 4
&&{A''}&&\\  % row5
\end{diagram}%
\end{equation}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/multiPpg.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.236\textwidth}
    \vspace{-0.75cm}
       \centering
%    %\begin{tabular}{|@\quad c@\quad|@\quad c@\quad|}
%   %\hline\\[5pt]
    \includegraphics[width=0.235\textwidth]% try 1.75 for wrap
    {figures/pdfs/multiPpg}
%       %    \\[5pt] \hline
%   %\end{tabular}
   %\vspace{-0.1cm}
    %\caption{4-ry \syncon \label{fig:multiPpg}}
   \vspace{-0.75cm}
\end{wrapfigure}
%\end{figure}


==> figures/diags/ppgPatterns-align.tex <==
%-- version with letters A,B
\cellW=8.0ex%
\cellH=8.0ex
%\begin{figure}[t]
%\centering
\begin{wrapfigure}{L}{0.3\textwidth}
	\vspace{-0.5cm}
	\centering
\begin{tabular}{c} % @}{\qquad}c} %@{\qquad}c} 
\begin{diagram}[w=1.1\cellW,h=0.85\cellH] 
\dbox{A_i} & \rCorrto^{r} & \dbox{A_j}\\%
\dUpdto<{u_i} &
\seTilearrow{\alnx{i}} &
\dDLine>{\id_{A_j}}\\
\dbox{A'_i}
& 
\pile{\rDercorrto^{r'} \\ 
\Downarrow{:}\alpha_{i} \\ 
\rCorrto_{r'_\alpha}}% end pile
& \dbox{A_j}
\\%
%\dbox{A'_1}& %\seTilearrow{\ppg{12}}~~~
\dDerupdto<{u'_i}&\seTilearrow{\rrstx{ij}}& \dDerupdto>{u'_j} \\%
A''_i & \rDercorrto^{r''} & A''_j
\end{diagram}
%& %
%\begin{diagram}[w=1.1\cellW,h=0.85\cellH] 
%\dbox{A_1} & \rCorrto^{r} & \dbox{A_2}\\%
%\dDLine<{\id_{A_1}}  &
%\swTilearrow{\alnx{20}} &
%\dUpdto>{u_2}\\
%\dbox{A_1}
%& 
%\pile{\rDercorrto^{r*u_2} \\ 
%\Downarrow\alpha_{20} \\ 
%\rCorrto_{r'}}% end pile
%& \dbox{A'_2}
%\\%
%%\dbox{A'_1}& %\seTilearrow{\ppg{12}}~~~
%\dDerupdto<{u'_1} &
%\swTilearrow{\rrstx{21}} & 
%\dDerupdto>{u'_2} \\%
%A''_1 & \rDercorrto^{r''} & A'_2
%\end{diagram}
%\\[55pt]
%(c1) & (c2) 
\end{tabular}
\vspace{-0.25cm}
\caption{$j\noteq i$ %Reflective update propagation
	\label{fig:ppgPatterns-align}}%
\vspace{-0.5cm}
\end{wrapfigure}
%\end{figure}

\endinput

==> figures/diags/ppgPatterns-reflect-reified.tex <==
\cellW=7.25ex%
\cellH=5.0ex
%\newcommand\fakeob{\strut}
%\newcommand\diagdots{\rotatebox[origin=c]{-45}{$\vdots$}}
%\newcommand\horizname[4] %#1 arrow name, #2 gap #3 adjoint symbol #4angle
%{\rotatebox[origin=c]{#4}{$#1\lefteqn{#2#3}$}}
%\begin{figure}
%\centering
\begin{wrapfigure}{L}{0.6\textwidth}
\vspace{-3ex}
	\centering
\begin{tabular}{c} %@{\quad}c}%@{\qquad}c} 
%@{\quad}c@{\quad}c}
%-- cell 11 (row,col) -
\begin{diagram}[w=1.1\cellW,h=1.\cellH] 
% row 1
&& &&&\dbox{A_n}
\\  % row 2
&&&&
\ruLine(5,3)>{\qquad R}
\ruLine(3,3)~{..j\noteq i..}%{\ldots}
& %\lefteqn{\ldots}
\\ %row 2a
&&&\fakeob&&
\\  % row 3
\dbox{A_i} & 
 \rLine                      
  &\dbox{A_1}&&&\dDerupdto~{u'_n}
\\% row 4
\dUpdto<{u_i}&  %\seTilearrow{\ppgx{i}}\hspace{1.5cm}
 &&\dDerupdto<{r'}>{\qquad\vdots} &&                                         
\\% row 5
\dbox{A'_i}&&\dDerupdto~{u'_1} &&& A''_n
\\ % row 6
\dDerupdto<{\amdx{u_i}} &&&&
\ruDashline(5,3)>{\quad R''}
\ruDashline(3,3)~{..j\noteq i..}  %{\pmb{\ldots}}
&
\\ % row 6a
&&&\fakeob&&
\\ % row 7
A''_i&
\rDashline
& A''_1&&&
\end{diagram}%
\end{tabular}
%\vspace{-1.ex}
\caption{Update propagation with reified corrs}
%	\\ 
%(To distinguish given data from those produced by the operation, the former are shown with framed nodes and solid lines, % in \diarefii\ 
%while the latter are non-framed and dashed.)
%}
\label{fig:ppg-reified}
%\vspace{-4ex}
\end{wrapfigure}
%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/ppgPatterns-reflect.tex <==
\cellW=7.25ex%
\cellH=5.0ex
\newcommand\fakeob{\strut}
%\newcommand\diagdots{\rotatebox[origin=c]{-45}{$\vdots$}}
%\newcommand\horizname[4] %#1 arrow name, #2 gap #3 adjoint symbol #4angle
%{\rotatebox[origin=c]{#4}{$#1\lefteqn{#2#3}$}}
%\begin{figure}
%\centering
\begin{wrapfigure}{L}{0.6\textwidth}
\vspace{-3ex}
	\centering
\begin{tabular}{c} %@{\quad}c}%@{\qquad}c} 
%@{\quad}c@{\quad}c}
%-- cell 11 (row,col) -
\begin{diagram}[w=1.1\cellW,h=1.\cellH] 
% row 1
&& &&&\dbox{A_n}
\\  % row 2
&&&&
\ruLine(5,3)>{\qquad R}
\ruLine(3,3)~{..j\noteq i..}%{\ldots}
& %\lefteqn{\ldots}
\\ %row 2a
&&&\fakeob&&
\\  % row 3
\dbox{A_i} & 
 \rLine                      
  &\dbox{A_1}&&&\dDerupdto~{u'_n}
\\% row 4
\dUpdto<{u_i}&  %\seTilearrow{\ppgx{i}}\hspace{1.5cm}
 &&\dDerupdto%<{r'}  %% REIFICATION IS HERE!
 >{\qquad\vdots} &&                                         
\\% row 5
\dbox{A'_i}&&\dDerupdto~{u'_1} &&& A''_n
\\ % row 6
\dDerupdto<{\amdx{u_i}} &&&&
\ruDashline(5,3)>{\quad R''}
\ruDashline(3,3)~{..j\noteq i..}  %{\pmb{\ldots}}
&
\\ % row 6a
&&&\fakeob&&
\\ % row 7
A''_i&
\rDashline
& A''_1&&&
\end{diagram}%
\end{tabular}
%\vspace{-1.ex}
\caption{Update propagation pattern
	\\ 
(To distinguish given data from those produced by the operation, the former are shown with framed nodes and solid lines, % in \diarefii\ 
while the latter are non-framed and dashed.)
}
\label{fig:ppgPatterns-reflect}
%\vspace{-4ex}
\end{wrapfigure}
%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/ppgPatterns-simple.tex <==
\cellW=7.25ex%
\cellH=5.0ex
\newcommand\diagdots{\rotatebox[origin=c]{-45}{$\vdots$}}
\newcommand\horizname[4] %#1 arrow name, #2 gap #3 adjoint symbol #4angle
{\rotatebox[origin=c]{#4}{$#1\lefteqn{#2#3}$}}
%\begin{figure}
%\centering
\begin{wrapfigure}{L}{0.45\textwidth}
	\vspace{-3ex}
	\centering
\begin{tabular}{c} %@{\quad}c}%@{\qquad}c} 
%@{\quad}c@{\quad}c}
%-- cell 11 (row,col) -
\begin{diagram}[w=1.\cellW,h=1.\cellH] 
%(a) % was 1.1\cellW, 1.1\cellH
&& &&\dbox{A_n}
\\  % row 2
&&&
%\ruLine(4,2)>{\horizname{r_n}{\hspace{1,5cm}}{\diagdots}{-22.5}} %
\ruLine(4,2)>{R}
\ruLine~{\ldots}
& %\lefteqn{\ldots}
\dDerupdto>{\pmb{u'_n}}
\\  % row 3
%\dbox{A_i} & \lTo_{~~a_i} &
\dbox{A_i} & 
%\rLine_{~~}^{\qquad\quad\rotatebox[origin=c]{-80}{$ \vdots$}}
\rLine
&\dbox{A_1}&~\vdots& A'_n
\\% row 4
%& &
\dUpdto<{\pmb{u_i}} & %\seTilearrow{\ppgx{i}}\hspace{2cm}
                        & \dDerupdto<{\pmb{u'_1}} &  
% \ruDashto(4,2)~{\hspace{-0.75cm}\horizname{{R}'_n}{\hspace{2.cm}}{\diagdots}{-22.5}} 
    \ruDashline(4,2)>{\hspace{1.cm}R'}
    \ruDashline~{\pmb{\ldots}}
 &
\\% row 5
%\dbox{A'_i} & \lDashto_{~~a'_i} & 
\dbox{A'_i} &
\rDashline%_{a'_1}^{\qquad\quad\rotatebox[origin=c]{-80}{$ \vdots$}}
& A'_1&
\end{diagram}%
%&  % cxell 12
%\begin{diagram}[w=\cellW,h=\cellH] %(b)
%\dbox{A_i} & \rCorrto^\Kcorr & \dbox{A_2}\\%
%\dDerupdto<{u'_i} & \swTilearrow{\ppgx{2i}}~~~
%            & \dUpdto>{u_2} \\%
%A'_i & \rDercorrto^{\Kcorr'} & \dbox{A'_2}
%\end{diagram}%
%%\\ [25pt]
%%a1) $i=2,3,4$ & (a2) $i=1,3,4$
%%& (b1) & (b2)
\end{tabular}
%\vspace{-0.25cm}
\caption{\small Propagation operation: input nodes \& arrows are framed \& solid resp., output ones are unframed \& dashed. Arrow $u_i$ is excluded from the right-face set of arrows.
\label{fig:ppgPatterns-simple}}%
\vspace{-5ex}
\end{wrapfigure}
%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/putput-oldDiag.tex <==
\begin{figure}
\[
\xymatrix{ 
& \spA_i &&&& \spA_j && \\
&A_i\ar[d]_{u_i}="u_i"\ar@{..}^R[rrrr]& && & A_j\ar[dd]_{\ppgr_{ij}(u_i)}="ppg1" \ar@{-->}@/^3pc/[dddd]^{\ppgr_{ij}(u_i;v_i)} &&\\
&A_i'\ar[dl]_{v_i}="v_i"\ar[dr]^{u_i':=\ppgr_{ii}(u_i)}="ui'"
\ar@{}|{[\merge]}[dd]& && &  &&\\
B_i\ar[dr]|{\tilde{v}_i:=\merge_1(v_i,u_i')}\ar@{-->}@/_2.5pc/[ddr]_{\ppgr_{ii}(u_i;v_i)} &&A_i''\ar[dl]^(0.4){\tilde{u'_i}:=\merge_2(v_i,u_i')}\ar@{..}^{R''}[rrr] && & A_j''\ar[dd]_{\ppg^{R''}_{ij}(\tilde{u'_i})}="ppg2"\ar@{}|{=}[r] &&\\
& B_i+_{A_i'}A_i''\ar@{}|(0.7){=}[l]\ar[d]_{\ppg^{R''}_{ii}(\tilde{u'_i})}& && &  \\
& A_i'''\ar@{..}^{R'''}[rrrr]& && & A_j''' &&\\
\ar@{-}@/_1.2pc/^{ \in \Kupd_{A_i'}} "u_i";"v_i"
\ar@{-}@/_0.5pc/_{ \in \Kdisj{}} "v_i";"ui'"
\ar@{-}@/_1pc/^(0.3){ \in \Kupd_{A_j''}} "ppg1";"ppg2"
}
\]
\caption{\lawnamebr{\kputput}{}-Law\label{fig:putput}}
\end{figure}

==> figures/diags/sdLens-letters.tex <==
\cellW=7.25ex%
\cellH=5.0ex
\begin{figure}
\centering
%	\begin{wrapfigure}{R}{0.35\textwidth}
%		\vspace{-1cm}
%		\centering
%-- version with letters A,B
\begin{tabular}{c@{\qquad}c@{\quad}c@{\quad}c}
%-- cell 11 (row,col) -
\begin{diagram}[w=1.1\cellW,h=1.1\cellH] %(a)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\dUpdto<a & \seTilearrow{\fppg}~~~
            & \dDerupdto>b \\%
\dbox{A'} & \rDercorrto^{r'} & B'
\end{diagram}%
& %- cell 1,2 -
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\dbox{A} & \rCorrto^{r} & \dbox{B}\\%
\dUpdto<{[\priv]} & \seTilearrow{\fppg}~~~
            & \dDerupdto>{\ide{}{B}} \\%
\dbox{A} & \rDercorrto^{r} & B
\end{diagram}%
  &   % -cell 1,3
 \begin{diagram}[w=\cellW,h=\cellH] %(a)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\dTo<a & \seTilearrow{\fppg}~~~
            & \dDashto>b \\%
\dbox{A'} & \rDercorrto^{r'} & B'
\end{diagram}%
&     % cell 1,4
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\uTo<a & \seTilearrow{\fppg}~~~
            & \uDashto>b \\%
\dbox{A'} & \rDercorrto^{r'} & B'
\end{diagram}%
%-- row 2 ---
\\[30pt]
%-- cell 2,1
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\dbox{A} & \rCorrto^r & \dbox{B}\\%
\dDerupdto>a & \swTilearrow{\bppg}~~~
            & \dUpdto>b \\%
A' & \rDercorrto^{r'} & \dbox{B'}
\end{diagram}%
& %-- cell 2,2
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\dbox{A} & \rCorrto^{r} & \dbox{B}\\%
\dDerupdto<{\ide{}{A}} & \swTilearrow{\bppg}~~~
            & \dUpdto>{[\priv]} \\%
A & \rDercorrto^{r} & \dbox{B}
\end{diagram}%
&   %-- cell 2,3
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\dDerupdto<a & \swTilearrow{\bppg}~~~
            & \dTo>b \\%
A' & \rDercorrto^{r'} & \dbox{B'}
\end{diagram}%
&   %-- cell 2,4
   \begin{diagram}[w=\cellW,h=\cellH] %(a)
\dbox{A} & \rCorrto^r &\dbox{B}\\%
\uDerupdto<a & \swTilearrow{\bppg}~~~
            & \uUpdto>b \\%
A' & \rDercorrto^{r'} & \dbox{B'}
\end{diagram}%
\\[35pt]
(a) arities &
(b) (\idppglaw)  laws
%& %
%%%(c) f-commutativity &
%\multicolumn{2}{c}{(c) monotonicity laws}
\end{tabular}
\caption{An %\fm 
	\label{fig:intro-bigModel}}
\end{figure}


\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:lens-oper}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/seq-comp.tex <==
%\cellW=5ex%
%\cellH=3.0ex
%\begin{figure}
\begin{wrapfigure}{R}{0.3\textwidth}
\vspace{-3.5em}
	\centering
\begin{tabular}{c} 
\begin{diagram}[w=4ex,h=4ex] 
\\  % row 1
A &  \rLine & B&\rLine&C
\\% row 2
\dUpdto<{u}&&&&                                          
\\% row 3
A'&&\dUpdto~{v}  &&\dUpdto~w
\\ % row 4
\dUpdto<{u'} &&&&
\\ % row 5
A'' & \rLine &B'' &\rLine& C'' %\dUpdto~w
%\\ % row 6
%\dTo~{u^*}&&\dUpdto~{v'}&&
%\\ % row 7
%A''' & \rLine & B''' &\rLine & C'''
\end{diagram}%
\end{tabular}
%\vspace{-1.ex}
\caption{Sequential composition %: $u''_i=u_i;u'_i$
\label{fig:seq-comp}}%
\vspace{-4ex}
\end{wrapfigure}
%\end{figure}

\endinput




==> figures/diags/spans/ppgPatterns-reflect.tex <==
\cellW=7.25ex%
\cellH=5.0ex
%\newcommand\diagdots{\rotatebox[origin=c]{-45}{$\vdots$}}
%\newcommand\horizname[4] %#1 arrow name, #2 gap #3 adjoint symbol #4angle
%{\rotatebox[origin=c]{#4}{$#1\lefteqn{#2#3}$}}
%\begin{figure}
%\centering
\begin{wrapfigure}{L}{0.65\textwidth}
%	\vspace{-1cm}
	\centering
\begin{tabular}{c} %@{\quad}c}%@{\qquad}c} 
%@{\quad}c@{\quad}c}
%-- cell 11 (row,col) -
\begin{diagram}[w=0.8\cellW,h=1.15\cellH] 
%(a) % was 1.1\cellW, 1.1\cellH
&&&& &&\dbox{A_n}
\\  % row 2
&&&&&\ruTo(4,2)~{\hspace{-0.5ex}\horizname{a_n}{\qquad\quad}{\diagdots}{-22.5}}%\lefteqn{{$\ldots$} }} 
& %\lefteqn{\ldots}
%\dDerupdto~{u'_n}
\\  % row 3
\dbox{A_i} & \lTo_{~~~a_i} &\dbox{A_0} & 
\rTo_{a_i}^{\qquad\quad\rotatebox[origin=c]{-80}{$ \vdots$}}
            &\dbox{A_1}&&\dDerupdto~{u''_n}
\\% row 4
\dUpdto<{u_i} &&&  %\seTilearrow{\ppgx{i}}\hspace{1.5cm}
 &&\vdots &                                         
\\% row 5
\dbox{A'_i} && \seTilearrow{\ppgx{i}} %\hspace{1.5cm}
&&\dDerupdto~{u''_1} && A''_n
\\ % row 6
\dDerupdto<{u'_i}&&&&&
\ruDashto(4,2)~{\hspace{-0.5cm}\horizname{a''_n}{\qquad\qquad}{\diagdots}{-20}}
&
\\ % row 7
{A''_i} & \lDashto_{a''_i} & A''_0&
\rDashto_{a''_1}^{\qquad\quad\rotatebox[origin=c]{-80}{$ \vdots$}}
& A''_1&&
\end{diagram}%
%&  % cxell 12
%\begin{diagram}[w=\cellW,h=\cellH] %(b)
%\dbox{A_i} & \rCorrto^r & \dbox{A_2}\\%
%\dDerupdto<{u'_i} & \swTilearrow{\ppgx{2i}}~~~
%            & \dUpdto>{u_2} \\%
%A'_i & \rDercorrto^{r'} & \dbox{A'_2}
%\end{diagram}%
%%\\ [25pt]
%%a1) $i=2,3,4$ & (a2) $i=1,3,4$
%%& (b1) & (b2)
\end{tabular}
\vspace{-0.25cm}
\caption{Reflective update propagation: $u''_i=u_i;u'_i$
\label{fig:ppgPatterns-reflect}}%
\vspace{-0.5cm}
\end{wrapfigure}
%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/spans/ppgPatterns-simple.tex <==
\cellW=7.25ex%
\cellH=5.0ex
\newcommand\diagdots{\rotatebox[origin=c]{-45}{$\vdots$}}
\newcommand\horizname[4] %#1 arrow name, #2 gap #3 adjoint symbol #4angle
{\rotatebox[origin=c]{#4}{$#1\lefteqn{#2#3}$}}
%\begin{figure}
%\centering
\begin{wrapfigure}{L}{0.65\textwidth}
%	\vspace{-1cm}
	\centering
\begin{tabular}{c} %@{\quad}c}%@{\qquad}c} 
%@{\quad}c@{\quad}c}
%-- cell 11 (row,col) -
\begin{diagram}[w=0.9\cellW,h=1.20\cellH] 
%(a) % was 1.1\cellW, 1.1\cellH
&&&& &&\dbox{A_n}
\\  % row 2
&&&&&\ruTo(4,2)~{\horizname{r_n}{\hspace{1,5cm}}{\diagdots}{-22.5}}%\lefteqn{{$\ldots$} }} 
& %\lefteqn{\ldots}
\dDerupdto>{u'_n}
\\  % row 3
\dbox{A_i} & \lTo_{~~a_i} &\dbox{A_0} & 
\rTo_{a_1}^{\qquad\quad\rotatebox[origin=c]{-80}{$ \vdots$}}
            &\dbox{A_1}&~~~~~\vdots& A'_n
\\% row 4
\dUpdto<{u_i} & &&\seTilearrow{\ppgx{i}}\hspace{2cm}
                        & \dDerupdto>{u'_1} &  
 \ruDashto(4,2)~{\hspace{-0.75cm}\horizname{r'_n}{\hspace{2.cm}}{\diagdots}{-22.5}} 
                        &
\\% row 5
\dbox{A'_i} & \lDashto_{~~a'_i} & A'_0&
\rDashto_{a'_1}^{\qquad\quad\rotatebox[origin=c]{-80}{$ \vdots$}}
& A'_1&
\end{diagram}%
%&  % cxell 12
%\begin{diagram}[w=\cellW,h=\cellH] %(b)
%\dbox{A_i} & \rCorrto^r & \dbox{A_2}\\%
%\dDerupdto<{u'_i} & \swTilearrow{\ppgx{2i}}~~~
%            & \dUpdto>{u_2} \\%
%A'_i & \rDercorrto^{r'} & \dbox{A'_2}
%\end{diagram}%
%%\\ [25pt]
%%a1) $i=2,3,4$ & (a2) $i=1,3,4$
%%& (b1) & (b2)
\end{tabular}
%\vspace{-0.25cm}
\caption{$u'_i=\id_{A_i}$ This Fig  is to be lessened!! %Simple update propagation
\label{fig:ppgPatterns-simple}}%
\vspace{-0.5cm}
\end{wrapfigure}
%\end{figure}

\endinput


%%== version with bullets and \circ s =beginFigure
%\begin{wrapfigure}{l}{.25\textwidth}%
%\vspace{-2ex}%
\begin{figure}
\centering
\begin{tabular}{c@{\quad}c@{\quad}c@{\quad}c}
\begin{diagram}[w=\cellW,h=\cellH] %(a)
\bullet & \rCorrto &\bullet\\%
\dUpdto & %\ruDercorrto_{} &\\%
            & \dDerupdto \\%
\bullet & \rDercorrto^{} & \circ
\end{diagram}%
&%
\begin{diagram}[w=\cellW,h=\cellH] %(b)
\bullet & \rCorrto &\bullet\\%
\dDerupdto & %\ruDercorrto_{} &\\%
            & \dUpdto \\%
\circ & \rDercorrto^{} & \bullet
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (c) was (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dUpdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dDerupdto>{\ide{}{}} \\%
\bullet & \rDercorrto^{r} & \circ
\end{diagram}%
&
\begin{diagram}[w=\cellW,h=\cellH] % now (d)
\bullet & \rCorrto^{r} &\bullet\\%
\dDerupdto<{\ide{}{}} & %\ruDercorrto_{} &\\%
            & \dUpdto>{\ide{}{}} \\%
\circ & \rDercorrto^{r} & \bullet
\end{diagram}%
\\[30pt]
(a) \fppg{} & (b) \bppg{} & %
%(c) f-commutativity &
\multicolumn{2}{c}{(c) (\idppglaw) law}
\end{tabular}
\caption{Update propagation operations (a,b)
and their laws \label{fig:ppgPatterns-12}}%
\end{figure}
%\vspace{-7ex}
%\end{wrapfigure}
%===EndFigure


==> figures/diags/weakInvert-paper.tex <==
\begin{figure}
%\centering
\hspace{-7.5pt}
\begin{tabular}{c}
\begin{diagram}[w=1.05\cellW,h=1.1\cellH] %(a)
\dbox{A} & \rCorrto^r     & \dbox{B} & \rCorrto^{r} & \dbox{A}%
               &  \rCorrto^{r} & \dbox{B}
\\%
\dUpdto<a & \seTilearrow{\fppg}~~~ & \dDerupdto>b %
                 & \seTilearrow{\bppg}~~~ & \dDerupdto>{a_{rr}}
                  & \seTilearrow{\fppg}~~~ & \dDerupdto>b
\\%
\dbox{A'} & \rDercorrto^{r'}  & %
B'            & \rDercorrto^{r'_{rr}} & A'_{rr} %
               & \rDercorrto^{r''} & B'
\end{diagram}%
%&    %
\\[30pt]
(a) \fbfppglaw\ law
\\[20pt]
\begin{diagram}[w=1.1\cellW,h=1.1\cellH] %(a)
\dbox{A} & \rCorrto^r     & \dbox{B} & \rCorrto^{r} & \dbox{A}%
               &  \rCorrto^{r} & \dbox{B}
\\%
\dDerupdto<a & \swTilearrow{\bppg}~~~ & \dDerupdto>{b_{rr}} %
                 & \swTilearrow{\fppg}~~~ & \dDerupdto>{a}
                  & \swTilearrow{\bppg}~~~ & \dUpdto>{b}
\\%
{A'} & \rDercorrto^{r''}  & %
    B'_{rr}            & \rDercorrto^{r'_{rr}} & A' %
               & \rDercorrto^{r'} & \dbox{B'}
\end{diagram}%
\\[30pt]
(b) \bfbppglaw\ law
%} % end TR
\end{tabular}
%\papertr%
%{ % paper version
%\caption{Round-tripping laws. Scenario in diagram (b) ``runs'' from the right to the left.\label{fig:invert-laws}}
%}
{%  TR version
\caption{Round-tripping and weak invertibility. Scenario in diagram (b) ``runs'' from the right to the left.}
\label{fig:invert-laws}}
\end{figure}

\endinput % see below for the two column format


\begin{figure}
\centering
\begin{tabular}{c@\quad c}
\begin{diagram}[w=1.05\cellW,h=0.9\cellH] %(a) was 1.05\cellH
\dbox{A} & \rCorrto^r     & \dbox{B} & \rCorrto^{r} & \dbox{A}%
               &  \rCorrto^{r} & \dbox{B}
\\%
\dUpdto<a & \seTilearrow{\fppg}~~~ & \dDerupdto>b %
                 & \seTilearrow{\bppg}~~~ & \dDerupdto>{a_1}
                  & \seTilearrow{\fppg}~~~ & \dDerupdto>b
\\%
\dbox{A'} & \rDercorrto^{r'}  & %
B'            & \rDercorrto^{r_1'} & A_1' %
               & \rDercorrto^{r_1'} & B'
\end{diagram}%
&    %
\begin{diagram}[w=1.1\cellW,h=0.9\cellH] %(a)
\dbox{A} & \rCorrto^r     & \dbox{B} & \rCorrto^{r} & \dbox{A}%
               &  \rCorrto^{r} & \dbox{B}
\\%
\dDerupdto<a & \swTilearrow{\bppg}~~~ & \dDerupdto>{b_{rr}} %
                 & \swTilearrow{\fppg}~~~ & \dDerupdto>{a}
                  & \swTilearrow{\bppg}~~~ & \dUpdto>b
\\%
{A'} & \rDercorrto^{r_1'}  & %
 B_1'            & \rDercorrto^{r_1'} & A' %
               & \rDercorrto^{r'} & \dbox{B'}
\end{diagram}%
\\[40pt]
(a) \fbfppglaw\ law  & (b) \bfbppglaw\ law
\end{tabular}
\caption{Round-tripping laws. (Scenario in diagram (b) ``runs'' from the right to the left.)
\label{fig:invert-laws}}%
\end{figure}


==> getMacros.tex <==
\newlength{\cellH}
\newlength{\cellW}

\input{macros/macros4comments}
% t stands for temporarily
\newcommand\zdmoddtok[4]{\zdmoddok{#1}{#2}{#3}{#4}}
\newcommand\zdmodtok[3]{\zdmodok{#1}{#2}{#3}}
% to make deleted things visible, use
%\renewcommand\zdmoddtok[4]{\zdmodd{#1}{#2}{#3}{#4}}
%\renewcommand\zdmodtok[3]{\zdmod{#1}{#2}{#3}}

\input{macros/shortcuts}
\input{macros/macros-mysections}
\input{macros/macros-general}
\input{macros/macros4textArrows}
\input{macros/macros4diagArrows}
% macros for lens things 
\input{macros/4lenses/macros4lensCompose}
\input{macros/4lenses/macros4tileDiags}
%\input{macros/4lenses/macros4drawingTiles}
\input{macros/4lenses/macros4tileLabels}
\input{macros/4lenses/macros4spaces}
\input{macros/4lenses/macros4operNames}
\input{macros/4lenses/macros4lawNames}
%\input{macros4thisPaper}
\input{macros/thisPaper}
%---









%\input{macrosTR/macros4relations}
% space names w/out arguments
%\input{macrosTR/macros4nonIndNames}
%\input{macrosTR/macros4traject-actpas}
%\input{macrosTR/hamidmacro}
%\input{macrosTR/macros4traject}
%\newcommand\aln{alignment}





==> getPackages.tex <==
\ifprodtf \else \usepackage[T1]{fontenc} \fi
%\usepackage[utf8]{inputenc}
%\usepackage{bickham}
%\usepackage{boondox-cal}
%\usepackage{boondox-calo}
% \usepackage{dutchcal}
\ifprodtf \else  \usepackage[leqno]{amsmath}  \fi
%\usepackage{GSDTR}
\ifprodtf \else \usepackage{fancybox}  \fi
\ifprodtf \else \usepackage{graphicx}  \fi
\ifprodtf \else \usepackage{wrapfig}  \fi
\ifprodtf \else \usepackage[english]{babel}  \fi
\ifprodtf \else \usepackage[utf8x]{inputenc}  \fi
\ifprodtf \else \usepackage{lipsum}  \fi
\ifprodtf \else \usepackage{lineno,hyperref}  \fi
\ifprodtf \else \usepackage[misc,geometry]{ifsym}  \fi

\endinput
\ifprodtf \else \usepackage[english]{babel} \fi
\ifprodtf \else \usepackage{color} \fi
\ifprodtf \else \usepackage[normalem]{ulem}\fi
\ifprodtf \else \usepackage{ucs}\fi
\ifprodtf \else \usepackage{url}\fi
\ifprodtf \else \usepackage{makeidx}\fi
\ifprodtf \else \usepackage{amssymb}\fi

\ifprodtf \else \usepackage[all]{xy}\fi
\ifprodtf \else \usepackage{xspace}\fi
\ifprodtf \else \usepackage{wrapfig}\fi
\ifprodtf \else \usepackage{subfig}\fi

\ifprodtf \else \usepackage{algorithm}\fi
\ifprodtf \else \usepackage{verbatim}\fi
\ifprodtf \else \usepackage{multirow}\fi
%=== previosly were in macros

\ifprodtf \else \usepackage{rotating}\fi
\ifprodtf \else \usepackage{lscape}\fi
\ifprodtf \else \usepackage{epsfig}\fi
\ifprodtf \else \usepackage{color}\fi
\ifprodtf \else\usepackage{float}\fi
\ifprodtf \else \usepackage{amsbsy,wasysym}\fi
\ifprodtf \else \usepackage{amsfonts}\fi
\ifprodtf \else \usepackage{amstext}\fi
\ifprodtf \else \usepackage{amssymb}\fi
\ifprodtf \else \usepackage{mathrsfs}\fi
\ifprodtf \else \usepackage{array}\fi
\ifprodtf \else \usepackage{latexsym}\fi
\ifprodtf \else \usepackage{xspace}\fi





==> macros/4lenses/macros4drawingTiles.tex <==
%\newcommand\xx{\!\!}
%\newcommand\xxx{\!\!\!}
%\newcommand\xxxx{\xxx\xx}

\newcommand\qryincl[2]{\mathsf{i}_{#1}^{#2}}
\newcommand\qryinclq[1]{\qryincl{#1}{Q}}
\newcommand\liftqryincl[2]{\ovr{\mathsf{i}_{#1}^{#2}}}
\newcommand\liftqryinclq[1]{\liftqryincl{#1}{Q}}


\newcommand\arrONarr{\stackrel{\mbox{$\longrightarrow$}}{\smash{\longrightarrow}}}
\newcommand\eeTilearrow[1]{\stackrel{#1}{\smash{\arrONarr}}}
%\newcommand\seTilearrow[2]{\searrow\xxx\xx\searrow{\mathsf{#1}_{#2}^{\mathstrut}}}

% NE staff
%\newcommand\mrklab[1]{\diagopername{#1}}
\newcommand\neTilearrowAB[2]{\mrklab{#1}
           \lefteqn{\,\nearrow\xxx\xx\nearrow}{\mrklab{#2}}
}
\newcommand\neqExeLabel{\neTilearrow{qEx}{e}}
\newcommand\seqExeLabel{\seTilearrow{qEx}{e}}
\newcommand\sevExeLabel{\seTilearrow{vEx}{e}}
\newcommand\nevExeLabel{\neTilearrow{vEx}{e}}
\newcommand\nePBLabel{\neTilearrow{p}{b}}
\newcommand\sePBLabel{\seTilearrow{p}{b}}
\newcommand\neCommLabel{\neTilearrow{[;]}{\xx}}
% SE staff
%\newcommand\seTilearrow[2]{\mrklab{#1}
%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
%}



\newcommand\seTilearrowHru[1]{%\mrklab{#1}
%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
 \lefteqn%
 {~~#1}{\searrow\xxx\xx\searrow}
} %
%%%% Oct 13 %%%%%
%\renewcommand\seTilearrowHru[1]{%\mrklab{#1}
%%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
% \lefteqn%
% {#1}{\searrow\xxx\xx\searrow}
%} %
%%%%%%%%%%%%%%%



%\newcommand\swTilearrowHru[1]{%\mrklab{#1}
%%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
% \lefteqn%
%         {~~#1}{\swarrow\xxx\xx\swarrow}
%}

\newcommand\ssTilearrow[2]{\downarrow\xxx\xx\downarrow^{#1_{#2}^{\mathstrut}}}
\newcommand\ssTilearrowHru[1]{\lefteqn%
{~~#1} \downarrow\xx\xx\downarrow}

% short names
\newcommand\seTilelabel[1]{\seTilearrowHru{#1}}
\newcommand\swTilelabel[1]{\swTilearrowHru{#1}}
\newcommand\ssTilelabel[2]{\ssTilearrowHru{#1}}


\newcommand\sefPrpLabel{\seTilearrow{[fPp}{]}}

% SW stuff
%\newcommand\swTilearrow[2]{\mrklab{#1}
%           \lefteqn{\mrklab{#2}}{\swarrow\xxx\xx\swarrow}
%}

%\renewcommand\swTilearrow[2]{{#1}
%           %\lefteqn
%           {\swarrow\xxx\xx\swarrow}{{#2}}
%}

\newcommand\swbPrpLabel{\swTilearrow{[bPp}{]}}

%\newcommand\swTilearrow[2]{\swarrow\xxx\xx\swarrow^{#1_{#2}^{\mathstrut}}}
% NN stuff
\newcommand\nnTilearrow[2]{\downarrow\xxx\xxx\xx\downarrow^{#1_{#2}^{\mathstrut}}}
\renewcommand\nnTilearrow[2]{\mrklab{#1}\!
           \lefteqn{\uparrow\xxx\xx\uparrow}{\mrklab{#2}}
}
%\renewcommand\nnTilearrow[2]{\mrklab{#1}^{
%              {\uparrow}\!{\uparrow}
%            } %{\mrklab{#2}}
%}
\newcommand\nnsubstLabel{\nnTilearrow{subst~}{}}

\newcommand\seselabel{~~~\seTilearrow{}{}~~~}
\newcommand\swswlabel{~~~\swTilearrow{}{}~~~}



\newcommand\rBlockarrow{\rule{0.25pt}{4.pt}\xx\Rrightarrow}
\newcommand\lBlockarrow{\Lleftarrow\xx\rule{0.25pt}{4.pt}}
\newcommand\sBlockarrow{\downarrow\xx\downarrow\xx\downarrow}
\renewcommand\sBlockarrow{\Downarrow\xxx\Downarrow}
\newcommand\rBlockarrowII{\mbox{$\sqsubset\xx\sqsupset$}\xx\LARGE{\rhd}}


==> macros4thisPaper.tex <==
%-- the upper taken from macros-general
\renewcommand\comprfam[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\comprfam[2]{\left(\mathstrut{#1}{:}\,\;{#2}\right)}
%\renewcommand\comprfam[2]{\left(\mathstrut{#1}\right)_{{#2}}}

%= tuples
\newcommand\tuplenam[1]{\ensuremath{\pmb{#1}}}
\renewcommand\tuplenam[1]{\ensuremath{{#1}}}
\newcommand\tupX[1]{\ensuremath{\tuplenam{#1}}}
\newcommand\tupA{\tupX{A}}
\newcommand\tupu{\tupX{u}}
\newcommand\tupB{\tupX{B}}
\newcommand\tupv{\tupX{v}}

\newcommand\prodX[1]{\ensuremath{\prtbf^{\Pi}\!\!#1}}
\renewcommand\prodX[1]{\ensuremath{#1^{\Pi}}}
\newcommand\prodmspA{\prodX{\mspA}}
\newcommand\prodmspB{\prodX{\mspB}}

\newcommand\bounX[1]{\ensuremath{\prtbf#1}}
\newcommand\bounmspA{\bounX{\mspA}}




\newcommand\xconfig[1]{\ensuremath{\mathsf{#1}}}
\newcommand\Span{\xconfig{Span}}
\newcommand\Cospan{\xconfig{Cospan}}
%\newcommand\K{\spaR}
% -- conseq compatible updates
\newcommand\compUpd[2]{\ensuremath{\mathsf{#1}^{{#2}}}}
\newcommand\seqK{\compUpd{K}{\RHD\!\!\RHD}}
\newcommand\parK{\compUpd{K}{{|}{|}{}}}
\newcommand\spanK[1]{\compUpd{K}{\blacktriangle{#1}}}
\newcommand\disjK[1]{\compUpd{K}{\vartriangle{#1}}}
\newcommand\Kupd{\seqK}
\newcommand\Kseq{\seqK}
%--space of conflict-free/concurr compatible updates
\newcommand\cofrK{\parK}
\newcommand\Kpar{\parK}
\newcommand\Kspan[1]{\spanK{#1}}
\newcommand\Kdisj[1]{\disjK{#1}}

%\endinput

% space of consist corrs
\newcommand\consK{\mspX{K^\bigstar}}
\newcommand\Kcorr{\compUpd{K}{\bigstar}}
%\renewcommand\Kcorr{\mspX{K^{\bigstar}}}
%\renewcommand\Kcorr{\ensuremath{{\spaR}^{}}}




\renewcommand\R[1]{\ensuremath{\mspA^{\bigstar}_{#1}}}
\renewcommand\xarr[1]{\ensuremath{#1%
		^{\footnotesize{\RHD}}}}
\newcommand\prospa[1]{\ensuremath{\Pi#1}}
\newcommand{\kl}{\ekk\times \ell}
\newcommand\exIntro{$\ast$}
\renewcommand\exIntro{\textit{Running example}}
\newcommand\bad{\ensuremath{\dagger}}
\newcommand\prt{\ensuremath{\partial}}
\newcommand\prtbf{\ensuremath{\boldsymbol{\partial}}}
\renewcommand\ta{\ensuremath{\mathsf{t}}}
\renewcommand\so{\ensuremath{\mathsf{s}}}
\cornersize{.5} 
\newcommand\dbox[1]{\fbox{$#1$}}
\renewcommand\dbox[1]{\ovalbox{$#1$}}

\newcommand\mmcol{\ensuremath{{M^{++}}}}
\newcommand\aacol{\ensuremath{{A^{++}}}}

\newcommand\Mplus{\ensuremath{{M^+}}}
\newcommand\Aplus{\ensuremath{{A^+}}}
\newcommand\mmplus{\Mplus}
\newcommand\aaplus{\Aplus}
\newcommand\Mpluss{\ensuremath{{M^{++}}}}
\newcommand\Apluss{\ensuremath{{A^{++}}}}

\newcommand\mmap[1]{\ensuremath{{\mathsf{m}_{#1}}}}
\newcommand\amap[1] {\ensuremath{{\mathsf{a}_{#1}}}}
\newcommand\mplus[1]{\ensuremath{{\mathsf{m}^+_{#1}}}}
\newcommand\aplus[1]{\ensuremath{{\mathsf{a}^+_{#1}}}}


\newcommand\undn{\und{n}}


\newcommand\scenum[1]{\ensuremath{\mathbf{(S#1)}}}
\newcommand\Scenum[1]{\textbf{(Scenario #1)}}
\renewcommand\Scenum[1]{(scenario \scenum{#1})}

\newcommand\xmi[1]{\ensuremath{M_{#1}}}
\newcommand\mo{\xmi{}}
\newcommand\mi{\xmi{1}}
\newcommand\mii{\xmi{2}}
\newcommand\miii{\xmi{3}}
\newcommand\xai[1]{\ensuremath{A_{#1}}}
\newcommand\ao{\xai{}}
\newcommand\ai{{\xai{1}}}
\newcommand\aii{{\xai{2}}}
\newcommand\aiii{{\xai{3}}}


%-- proper names --
\newcommand\addr{\nmf{Addr}}
\newcommand\name{\nmf{name}}
\newcommand\String{\nmf{String}}
\newcommand{\Person}{\nmf{Person}}
\newcommand{\Comp}{\nmf{Company}}
\newcommand{\Company}{\nmf{Company}}
\newcommand{\Commute}{\nmf{Commute}}
\newcommand{\Comm}{\nmf{Commute}}
\newcommand\Addr{\nmf{Addr}}
\newcommand\from{\nmf{from}}
\newcommand\lives{\nmf{lives}}
\newcommand\loc{\nmf{located}}
\newcommand\Empl{\nmf{Empl}}
\newcommand{\eer}{\nmf{empl}\textrm{-}\nmf{er}}
\newcommand{\eee}{\nmf{empl}\textrm{-}\nmf{ee}}
%\newcommand\eer{\nmf{empl{-}er}}
%\newcommand\eee{\nmf{empl{-}ee}}

\newcommand\namefont[1]{\ensuremath{\mathsf{#1}}}
\newcommand\nmf[1]{\namefont{#1}}
\newcommand\ittt[1]{\ensuremath\mathit{#1}} 

\newcommand{\netw}{\nmf{Network}}
\newcommand{\network}{\nmf{Network}}
\newcommand{\person}{\nmf{Person}}
\newcommand{\member}{\nmf{Member}}

\renewcommand\phone{\nmf{Phone}}
\newcommand\EMail{\nmf{Email}}
\newcommand\contact{\nmf{Contact}}
\newcommand{\topic}{\nmf{Topic}}
\newcommand{\str}{\nmf{Str}}
\renewcommand{\inv}{\nmf{inv}}
\newcommand{\PM}{\nmf{P/M}}

\newcommand{\cp}{\nmf{c/p}}
\newcommand{\memb}{\nmf{memb}}
\newcommand{\ident}{\nmf{ident}}
\newcommand{\cell}{\nmf{cell}}
\newcommand{\emails}{\nmf{emails}}
\newcommand{\logins}{\nmf{logins}}
\newcommand{\comm}{\nmf{comm}}
\newcommand{\privv}{\nmf{priv}}
%\newcommand{\from}{\nmf{from}}
\newcommand{\too}{\nmf{to}}
\newcommand{\scope}{\nmf{scope}}
\newcommand{\escope}{\nmf{e}\textrm{-}\nmf{scope}}
\newcommand{\on}{\nmf{on}}
\newcommand{\ret}{\nmf{re}}
\newcommand{\re}{\nmf{re}}
\newcommand{\subj}{\nmf{subj}}
\newcommand{\eon}{\nmf{e}\textrm{-}\nmf{on}}
%===
%\newlength{\cellH}
%\newlength{\cellW}



%=== from JSS paper
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}



\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}

\newcommand\alens{\ensuremath{\lambda}}

% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput

% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}


==> sections/lastParaOfSection1.tex <==
The paper is an essential extension of our FASE'18 paper \cite{me-fase18}. The main additions are i) a new section motivating our design choices, ii) a constrained Putput law (\kputput) and its thorough discussion, including a corresponding extension of the running example, iii) a counterexample showing that invertibility is not preserved by  star composition, iv) two types of parallel composition of multiary lenses, v) Related Work and Future Work sections are essentially extended, particularly, an important subsection about multimodel updates including correspondence updates (categorification) is added. 

==> sections/lensesFinal/asym2sym.tex <==
\mysubsection{Assembling $n$-ary lenses from binary lenses}
This section shows how to assemble $n$-ary lenses from binary asymmetric lenses modelling view computation \cite{me-jot11}.
\begin{mydefin}[Asymmetric Lens, cf. \cite{me-jot11}]
	An {\em asymmetric lens (a-lens)} is a tuple $\ebb^{\preccurlyeq}=(\spaA,\spaB,\get, \putl)$ with \spaA\ a model space called the {\em (abstract) view}, \spaB\ a model space called the {\em base}, \flar{\get}{\spaA}{\spaB} a functor (read ``get the view''), and \putl\ a family of operations $\comprfam{\putl^B}{B\inn\xob{\spaB}}$ (read `'put the view update back'') of the following arity. Provided with a view update \frar{v}{\get(B)}{A'} at the input, operation $\putl^B$ outputs a base update \frar{\putl_\indb(v)=u'}{B}{B''}  
	and a reflected view update \frar{\putl_\inda=v'}{A'}{A''} 
	such that $A''=\get(B'')$. 
A view update \frar{v}{\get(B)}{A'} is called {\em closed} if $\putl^B_\inda(v)=\id_{A'}$. \qed
\end{mydefin}

The following is a specialization of Def.~\ref{def:wblens}.	
\begin{mydefin}[Well-behavedness]\label{def:wb-a-lens}
An a-lens is {\em well-behaved (wb)} if  
it satisfies the following laws for all \zdmodok{$A\in\xob{\spaA}$, $B\in\xob{\spaB}$ and \frar{v}{A}{A'}}{$B\in\xob{\spaB}$ and \frar{v}{\get(B)}{A'}}{}
	
\smallskip
\noindent \begin{tabular}{l@{\qquad}l}
		\lawnamebr{Stability} &
		$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
		\\  
		[\lawgap] \lawnamebr{Reflect0} &	
		$\ppgB_{\inda}(v)\noteq \id_{A'}$ implies 
		$A'\noteq \get(X)$ for all $X\inn\xob{\spaB}$
			\\  [\lawgap] \lawnamebr{Reflect1} &	
		$(v, v')\in \Kupd_{A}$ %for all $u_i$ 
		\\   
		[\lawgap] \lawnamebr{Reflect2} &
		$\ppgB_{\indb}(v;\ppgB_{\inda}(v)) = \ppgB_{\indb}(v)$
		\\ \lawnamebr{PutGet}$_{~~~~~~}$
		&
		%$v;v'=\get(v.\putl_\indb^B) $	% dot version
		$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version
\end{tabular}

\qed 
%
%A wb a-lens is called {\em invertible}, if it also satisfies the law:
%
%\noindent \begin{tabular}{l@{\quad}l}
%\lawnamebr{PutGetPut}$_{~~~~~~}$&
%%$v;v'=\get(v.\putl_\indb^B) $	% dot version
%$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version
%\end{tabular}
\end{mydefin}
In contrast to the symmetric lens case, we added \lawnamebr{Reflect0} and we have included an invertibility condition \lawname{PutGet} into the definition of well-behavedness due to historical traditions. Subsequent results will also provide some justification for this. Note also that \lawname{PutGet} provides a weak rather than strong invertibility: \lawname{Reflect2} implies $\putl^B_\indb(\get(\putl^B_\indb(v)))=\putl^B_\indb(v)$.   \hkmodok{but $\get(\putl^B_\indb(v))=\putl^B_\indb(v)$ does not hold. }{}{??? This equation makes no sense, and I don't know, what you wanted to say here}

\smallskip
Any a-lens $\ebb^{\preccurlyeq} =(\spaA,\spaB,\get, \putl)$ gives rise to a binary symmetric lens $\ebb$. Its carrier consists of model spaces $\spaA$ and $\spB$. Furthermore $\xstar{\ebb} = \xob{\spB}$ with boundary mappings defined as follows: for $R\in\xstar{\ebb}= \xob{\spaB}$, 
%$\partial_\spA^{\ebb}$ being the object part of functor $\get$, 
$\partial_\spA^{\ebb}R=\get(R)$ and $\partial_\spB^\ebb R= R$.  %$id_\xob{\spB}$. 
Thus, the set of corrs $\xstar{\ebb}(A,B)$ is $\{B\}$ if $A=\get(B)$, and is empty otherwise. 

For a corr $B$, we need to define six operations $\ebb.\ppg^B_{\_\_}$. If \frar{v}{A}{A'} is a view update, then 
$\ppg^{B}_{\spA\spB}(v)=\putl^B_\indb(v): B\to B''$, 
$\ppg^{B}_{\spA\spA}(v)=\putl^B_\inda(v): A'\to A''$, and
$\ppg^{B}_{\spA\star}(v)=B''$. The condition $A''=\get(B'')$ for $\ebb^\preccurlyeq$ means that $B''$ is again a consistent corr with the desired boundaries. For a base update \frar{u}{B}{B'} and a corr $B$, 
$\ppg^{B}_{\spB\spA}(u)=\get(u)$,
$\ppg^{B}_{\spB\spB}(u)=\id_{B'}$, and
$\ppg^{B}_{\spB\star}(u)=B'$. Functoriality of $\get$ yields consistency of $B'$. 
 
\begin{lemma}\label{lemma:asymm_symm} Let $\ebb^\preccurlyeq$ be a wb a-lens and $\ebb$ the corresponding symmetric lens. Then all base updates of $\ebb$ are closed, and $\ebb$ is wb and invertible. %, if $\ebb^\preccurlyeq$ is wb. \qed 
 \end{lemma}
 \begin{proof}
 Base updates are closed by the definition of $\ppg_{\spB\spB}$. Well-behavedness follows from wb-ness of $\ebb^\preccurlyeq$. Invertibility has to be proved in two directions: $\ppg_{\spaB\spaA};\ppg_{\spaA\spaB};\ppg_{\spaB\spaA} = \ppg_{\spaB\spaA}$ follows from \lawnamebr{PutGet} and \lawnamebr{Reflect0}, the other direction follows from \lawnamebr{PutGet} and \lawnamebr{Reflect2}, see the remark after Def.\ref{def:wb-a-lens}. 
 \qed
 \end{proof}

  \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  \zdmodok{and invertible}{}{!!!} (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$. 
\end{theorem}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images.
\qed
\end{proof}

\input{figures/pdfs/mergedMetamultimod-uml}
\exIntro. Let $\spA = \spA_i$ be one of the model spaces, and let $\spB$ be the space consisting of all possible merged models together with comprehensive updates, \ie, data typed over the metamodel $M^+$ shown in Fig.\ref{fig:mergedMultiMetamod-uml} and their joined edit sequences. The metamodel unifies all known employment, location, and commuting information. Moreover, for persons and companies the numbers of model spaces, in which the person or company occurs, can be traced back via attribute ''spaces'' (see \cite{DBLP:conf/ecmdafa/KonigD17} for a formal treatment of this tracing). Objects of type \Commute\ are known to be recorded in space $\spaA_3$. We can define the following asymmetric lens $\ebb_i^\ast$: $\get_i$ takes update $u^+:A\to A'$ of data typed over $M^+$ and has output the restricted model containing only objects from the model spaces, in which they are recorded. Furthermore, $\putl$ acts according to the update propagations already discussed in Sect.\ref{sec:example}, but now propagating these updates into comprehensive merged models.   \qed
%
%\exIntro\ Combining a-lenses $\ebb_i^\ast$ in this way yields an $n$-ary lens $\sum_{i=1}^n\ebb_i^\ast$ whose properties can now be inferred from the binary a-lenses. \qed

\smallskip
There is also a backward transformation of (symmetric) lenses to spans of a-lenses. \hkmodok{, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.}{}{We do not use categorical aspects here!} Let $\ell=(\mspaA, \ppg)$ be a {(not necessarily invertible) }wb lens. It gives rise to the following span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$   
where $\spaA_i=\prtbf_i(\mspaA)$, space the objects of $\spaB$ are the conistent multimodels together with modelmodel updates, cf. Def. \ref{def:multispace} and functors $\get_i:\spaB\to \spaA_i$ are projection functors $\prtbf_i$. 
%\footnote{
%In fact, we have already described this construction footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}, where space \spaB\ was denoted by $[\mspaA]$. 
%Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 

 Given $B = (\tupleAWOB, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1'\ldots u'_{i-1} (u_i;u_i') u'_{i+1} \ldots u_n'): (\tupleAWOB, R)\to (\tupleAiiWOB, R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is a direct consequence of the respective definitions. 

An open question is whether the transformation of spans to lenses described in Theorems \ref{thm:LensesFromSpans} and the inverse transformation of lenses to spans described above are inverse algebraic operations. The non-obvious isomorphism for the binary case in \cite{jr-jot17} shows that this is only the case modulo a certain equivalence relation. This relation may be different for our reflective multiary lenses, and we leave the investigation of this question for future research.  

 \endinput
 
%============= Old Version ========= 
 \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$.
% 	
  	Moreover, $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible as soon as the span satisfies the following condition%
 	\footnote{Found for the binary case by Bob Rosebrugh \cite{bob-invert}}: 
% 	$$
% 	\putl^B_{\indb i}
% 	$$
$\PP^B_i=\PP^B_j$ for all $B\in\xob{\spaB}$ and $i,j\le n$, where for given $B$ and $i$,  $\PP^B_i$ is the inverse image of 
$\xarr{\spaB}(\get_i(B),\_)$, \ie,  the set $\compr{\putl^B_{\indb i}(v_i)}{\frar{v_i}{\get_i(B)}{\_}}$. %, then $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible.
\end{theorem}
\shortlong{}{%}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent%
\footnote{To make it precise, we need to introduce a simple notion of lens equivalence, which identify lenses with the same propagation behavior but, perhaps, different sets of corrs -- see. \eg, \cite{jr-jot17}} to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images. \qed
 \end{proof} 
}
For the backward transformation of lenses to spans of a-lenses, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.
\begin{theorem}[Spans from lenses] \label{th:lens2span}Any {(not necessarily invertible) }wb lens $\ell=(\mspaA, \ppg)$ gives rise to a span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$. \\
%{\color{red}We should say already here, how $\ell$ is related to the resulting construction of Thm \ref{thm:LensesFromSpans} for $\ell_i^\preccurlyeq$, see below}
\end{theorem}
\shortlong{}{%}
\begin{proof} Let $\mspA$ have model spaces $\spaA_i$ and corr set $\R$ with corresponding boundary functions $\partial_i$. Let 
\[\spaB = \{(A_1, \ldots, A_n, R)\mid \partial_i(R) = A_i \mbox{ for all }i\}\] 
be the set of all aligned consistent multimodels and $\get_i:\spaB\to \spaA_i$ be projections, \ie\ $\get_i(A_1, \ldots, A_n, R)= A_i$ and $\get_i(u_1, \ldots, u_n)= u_i$\footnote{
Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 
}. Given $B = (A_1, \ldots, A_n, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1', \ldots, u'_{i-1}, u_i;u_i', u'_{i+1} \ldots, u_n'): (A_1, \ldots, A_n, R)\to (A_1'', \ldots, A_n'', R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is an direct consequence of the respective definitions. 
 \qed
\end{proof} 
}
%An important issue is how the two transformations, lenses to spans and spans to lenses, interact. To manage this, we need an $n$-ary counterpart of the theory of lens equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  We leave it for future work. 
It is easy to see that $\Sigma_{i\inn I_\ell}\ell_i^\preccurlyeq = \ell$ for any lens $\ell$, but if we begin with a span of a-lenses $\ebb_i$, $i\inn I$ build a lens $\Sigma_{i\inn I}\ebb_i$ and then build the span $(\Sigma_{i\inn I}\ebb_i)^\preccurlyeq_i$, the two spans are different. This difference could disappear with a suitable notion of span equivalence, which we conjecture should be a straightforward generalization of the equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  %which we think should be generalizable for the $n$-ary case. We leave it for future work. 
%
%\begin{example}
%Running
%\end{example}

\endinput
\begin{theorem}[Sequential composition]
	Let \lensar{\aekk}{\spaA}{\spaB} and  \lensar{\aell}{\spaB}{\spaC} be two wb a-lenses satisfying the following {\em junction condition}: all updates in $\spaB$ obtained by $\ekk$-propagation from \spaA\ are $\ell$-closed. Then there is a uniquely defined wb a-lens \lensar{\aekk;\aell}{\spaA}{\spaC}. %The composition is associative with identity lenses \lensar{\ell_{\id_{\spaB}}}{\spaB}{\spaB} being its units. 
\end{theorem}
 \input{figures/diags/seq-comp} 
 \textit{Proof.} Obviously, composition of \Kupd-preserving functors  
\flar{\get^\ekk}{\spaA}{\spaB} and \flar{\get^\ell}{\spaB}{\spaC} is a \Kupd-preserving functor: $\get^{\ekk;\ell}=\get^\ekk\circ\get^\ell$. Now we define $\putl^{\ekk;\ell}$. 
Let $u$ be an update as shown in \figref{fig:seq-comp} where horizontal lines are \get-corrs. Let $v=\putl^{\ekk B}_\indb(u)$, $u'=\putl^{\ekk B}_\inda(u)$, and $w=\putl^{\ell C}_\indb(v)$ (by the junction condition $v'=\id_{B''}$).  
%Finally, $u^*{=}\,\get^\ekk(v')$.  
Define $\putl^{C~\ekk;\ell}_\indb(u)=w$ and $\putl^{C~\ekk;\ell}_\inda(u)=u'$. Laws \lawname{Reflect1,2, 3} for $\ell;\ekk$ are obvious. %To prove idempotency \lawname{Reflect2}, we note that as $(v, v')\in\Kupd{B''}$ by $\ell.\lawname{Reflect}$, $u''\Kupd_{A''}u^*$ as $u''=u;u'=\get^\ekk(v)$ owing to $\Kupd$-preservation by $\get^\ekk$. Hence, by $\ekk.\lawname{PutPut}$, $\pult^{B \ekk}(u'';u^*)=\putl(u'');\putl(u^*)$
Stability and Putput are obvious too. 



==> sections/lensesFinal/bits-i-pieces.tex <==

 === from the functorial def 
	\[\frar{{\_}^\bigstar_{\mspaA}}{\prodmspA}{\setcat}\]
	where \prodmspA\ denotes the category 
	$\prod\bounmspA =\spaA_1\timm\ldots\timm\spA_n$. We will omit the subindex $\__\mspA$ if it is clear from the context. 
	
		\[\frar{\msp\corr{A}}{\prosing\spA}{\setcat}\]
		such that all sets $\mspA^\bigstar(A)$, $A=(A_1..A_n) \inn \xob{(\prod\spA)}$, are disjoint.
	 To simplify notation, given an update %\frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % 
	 \frar{u}{A}{A'}
	 from a model tuple $A=(A_1..A_n)$ to a model tuple $A'=(A'_1..A'_n)$, 
	 we will write $A^\bigstar$ for the set $\mspA^\bigstar(A)$, and \frar{u^\bigstar}{A^\bigstar}{A'^\bigstar} %{\ovr{A'_i}^\bigstar}
	  for the function $\mspA^\bigstar(u)$. 
	 Analogously, given a tuple model $A$ and a foot update \frar{u_i}{A_i}{A'_i}, function $\ovr{u_i}^\bigstar$ is denoted by $u_i^\bigstar$.	%\zd{so, i decided to keep the notation used in the Fase paper for consistency of the two papers, but in the present one we will use the simplified variant}
	
	Given a model tuple $\tupA = (A_1..A_n)$, elements of the set $ \xstar{\tupA}$ are called {\em \corrce s} or just {\em corrs} over \tupA. Intuitively, a corr $R\in\xstar{\tupA}$ is understood as a correspondence specification interrelating models $A_i$; we will also say that the latter are {\em aligned} via $R$, and that \tupA\ is the {\em boundary} of $R$ and we write $\tupA=\prt R$ (recall the disjointness condition above). A foot update \frar{u_i}{A_i}{A'_i} creates a new corr $R'=u_i^\bigstar(R)\in \ovr{A'_i}^\bigstar$ called the {\em realignment} of the model $(A,R)$.Due to functoriality of $\msp\corr{A}$, the operation of realignment is fully determined by realignment caused by  singular updates: given $u=(u_1...u_n)$, $u^\bigstar=u^\bigstar_1;...;u^\bigstar_n$.
	
	===
	
		\[ 
		\comprfam{\Kcorr_A\subseteq \corr{A}}%
		{{A=(A_1..A_n) \in \xob{(\prod\spA)}}} 
		\]
	 indexed by model tuples. %Note that for an update \frar{u_i}{A_i}{A'_i} and a corr $R\in \Kcorr_A$, we do not require its realignment $R'=u_i^\bigstar(R)$ to be necessary consistent, \ie, it may happen that $R'\notin \Kcorr_{A'}$ and thus consistency restoration is needed. 
	 \par	
	We will write $\sp\corr{A}$ for the class of all corrs, $\Kcorr_\spA$ for its subclass of consistent corrs and, for a given model $A_i\in\xob{\spA_i}$, $\corr{A_i}\eqdef \compr{R\in\sp\corr{A}}{\prt_i R=A}$ for the class of all corrs with a fixed foot $A_i\in \xob{\spA_i}$ and $\Kcorr_{A_i}\subset \corr{A_i}$ for the subclass of all such consistent corrs. 
	
	===
	
	\zdmoddok{For a given model $\nia=(A,R)$, any foot update \frar{u_i}{A_i}{A'_i} (we will also say {\em local} update) gives rise to a ({\em global}) feet update  $\ovr{u_i}=(\id_{A_1}...u_i...\id_{A_n})$, and we write $u_i^\bigstar(R)$ for the corr $R'\eqdef \ovr{u_i}^\bigstar(R)\in A'^\bigstar$ where $A'=(A_1,..,A_{i-1}, A'_i, A_{i+1}, ..,A_n)$. Again, if even $R$ is consistent, its realignment $R'$ may be inconsistent, and then we say that update $u_i$ destroyed the consistency of model \nia.}{}{it seems it's just a repetition}{-4em}
	


==> sections/lensesFinal/latexCode-for-Definition-2.tex <==
\begin{defin}[Well-behaved Model Spaces]\label{def:wbspace}
	\noindent 
{\renewcommand\&{\wedge}
\begin{center}
\begin{tabular}{l@{\quad}l}
	\lawnamebr{\Kupd\ and~ Id}{} &	
	For all $u\inn{\spA}(\_,A)$, $u'\inn{\spaA}(A,\_)$: $(u,\id_A), (\id_A,u')\inn\Kupd_A$, 
	\\ [1.5ex]
		&	
For any three consecutive updates $u,v,w$, we require: 
	\\  %[1ex] 
		\lawnamebr{\Kupd\Kupd }{1}&
			$(u\Kupd\,vw$ $\&$ $v\Kupd w)$ imply 
			$(u\Kupd v$ $\&$ $uv\, \Kupd w)$,
			\\
		\lawnamebr{\Kupd\Kupd }{2} &
		 $(uv\,\Kupd w$ $\&$ $u\Kupd v)$ imply $(v\Kupd w$ $\&$ $u\Kupd\,vw)$,
			 \\
			 & where composition is denoted by concatenation ($uv$ for $u;v$ etc). 
	\\ [1ex]
%\multirow{2}{*}{
\lawnamebr{\Kdisj{}~and ~\Kupd}%}
{} &
For all $(u_1,u_2)\in\Kdisj{}_A$: $(u_i, \widetilde{u_i})\in\Kupd_{A'_i}$, $i=1, 2$,
%\\ & 
where $\widetilde{u_i}=\merge_{A,i}(u_1, u_2)$
		\\ [1.5ex]
	\multirow{2}{*}{\lawnamebr{MergeSym}{}}& For all $\frar{u_1}{A}{A'_1}$, $\frar{u_2}{A}{A'_2}$, if $(\widetilde{u_1}, \widetilde{u_2})=\merge_A(u_1, u_2)$,
	\\ & then $(\widetilde{u_2}, \widetilde{u_1})=\merge_A(u_2, u_1)$ 
	\\ [1.5ex]
	\lawnamebr{MergeId}{}& For all $\frar{u}{A}{A'}$: $\merge_A(u,\id_A) = (\id_{A'},u)$    
\end{tabular}
\end{center} \qed 
}  %end group
\end{defin}
The first condition is the already discussed natural property for sequential compatibility. The pair of conditions below it requires complementing updates not to revert anything done by the other update. The last three conditions are obvious requirements to the operation \merge. 
\par
We assume all our model spaces to be wb and, as a rule, will omit explicit mentioning. Each of the metamodels $M_1$..$M_3$ in the running example gives rise to a (wb) model space of its instances as discussed above.

%---> see below the old fuller version of the def
%
%\begin{defin}[Well-behaved Model Spaces]\label{def:wbspace}
%	\noindent 
%\newpii{A model space is {\em well-behaved (wb)} if the following conditions hold for all $A\in\xob{\spaA}$:
%}{1: conditions $\Kupd_{1,2}$ below are added}{-2em}
%\begin{center}
%	{\renewcommand\&{\wedge}%{\enma{\mathrm{and}}}
%\begin{tabular}{l@{\quad}l}
%	\lawnamebr{\Kupd\ and~ Id}{} &	
%	For all $u\inn{\spA}(\_,A)$, $u'\inn{\spaA}(A,\_)$: $(u,\id_A), (\id_A,u')\inn\Kupd_A$, 
%	\\ [1ex]
%		%\lawnamebr{\Kupd\Kupd }{} 
%		&	
%For any three consecutive updates $u,v,w$, we require: 
%	\\ [1ex] 
%	%\begin{tabular}{l@{\quad}l}
%		\lawnamebr{\Kupd\Kupd }{1}&
%			$(u\Kupd\,vw$ $\&$ $v\Kupd w)$ imply 
%			$(u\Kupd v$ $\&$ $uv\, \Kupd w)$,
%			\\
%		\lawnamebr{\Kupd\Kupd }{2} &
%		 $(uv\,\Kupd w$ $\&$ $u\Kupd v)$ imply $(v\Kupd w$ $\&$ $u\Kupd\,vw)$,
%			 \\
%			 & where composition is denoted by concatenation ($uv$ for $u;v$ etc). %and consider compositing binding stronger than \Kupd.
%%	\end{tabular}
%	\\ [1ex]
%	\multirow{2}{*}{\lawnamebr{\Kdisj{}~and ~\Kupd}}{} &
%	For all $(u_1,u_2)\in\Kdisj{}_A$: $(u_i, \widetilde{u_i})\in\Kupd_{A'_i}$, $i=1..2$
%	\\ & where $\widetilde{u_i}=\merge_{A,i}(u_1, u_2)$
%		\\ [1ex]
%	\multirow{2}{*}{\lawnamebr{Merge Symmetry}{}}& For all $\frar{u_1}{A}{A'_1}$, $\frar{u_2}{A}{A'_2}$, if $(\widetilde{u_1}, \widetilde{u_2})=\merge_A(u_1, u_2)$,
%	\\ & then $(\widetilde{u_2}, \widetilde{u_1})=\merge_A(u_2, u_1)$ 
%%	\\ [1ex]
%%\lawnamebr{MergeSame}{}& For all $\frar{u}{A}{A'}$: 
%%$\merge_A(u, u) = (\id_{A'}, \id_{A'})$  
%	\\ [1ex]
%	\lawnamebr{MergeId}{}& For all $\frar{u}{A}{A'}$: $\merge_A(u,\id_A) = (\id_{A'},u)$    
%\end{tabular} 
%}  %end group
%\end{center} \qed
%%A {\em model space functor} from $\spaA$ to $\spaB$ is a functor $F:|\spaA|\to |\spaB|$, such that $(u,u')\hspace{-0.1em}\in \hspace{-0.1em}\Kupd_A$ implies $(F(u),F(u'))\hspace{-0.1em}\in\hspace{-0.1em}\Kupd_B$. We will denote model spaces and their carriers by the same symbol and often omit explicit mentioning of $\Kupd$.\qed  % (cf. Sect.\ref{sec:modelspaces}). 
%\end{defin}
%The first condition is the already discussed natural property for sequential compatibility. The pair of conditions below it requires complementing updates not to revert anything done by the other update. The last three conditions are obvious requirements to the operation \merge. 
%%\footnote{ Note that we do not claim the converse, namely the existence of a concurrently compatible partner in a sequentially compatible pair.} 
%
%We assume all our model spaces to be wb and, as a rule, will omit explicit mentioning. Each of the metamodels $M_1$..$M_3$ in the running example gives rise to a (wb) model space of its instances as discussed above.
%%\input{figures/diags/mergeDef}


==> sections/lensesFinal/lego-new.tex <==
\section{Compositionality of Update Propagation: Playing Lego with Lenses}\label{sec:lego-seq}
We study how lenses can be composed. Assembling well-behaved and well-tested small components into a bigger one is the quintessence of software engineers working in a team. If, furthermore, a mathematical theorem guarantees that desired properties carry over from the components to the composition, additional integration tests with regard to these properties are no longer necessary. 
\par
In Sect.~\ref{sec:lego-para}, we consider the parallel composition of lenses, which is easily manageable. Sequential composition, in which different lenses share some of their feet, and updates propagated by one lens are taken and propagated further by one or several other lenses, is much more challenging and considered in the other two subsections. In \sectref{sec:lego-star}, we consider ''star-composition'', cf.\ Fig.~\ref{fig:starComposition} and show that under certain additional assumptions (very) well-behavedness carries over from the components to the composition. However, invertibility does not carry over to the composition -- we shows this with a counterexample. In \sectref{sec:lego-spans2lens}, we study how (symmetric) lenses can be assembled from asymmetric ones and prove a theorem on the preservation of properties. 
\par
Since we now work with several lenses, we need a notation for lens' components. Given a lens $\ell = (\mspaA, \ppg)$, we write $\xstar{\ell}$ 
%instead of $\xstar{\mspA}$ 
for the alignment functor in Def.~\ref{def:mspace}. Feet of an aligned multimodel $(A = (A_1\ldots A_n),R)$ are written $A_i = \prt_i^\ell R$ for the $i$-th boundary of corr $R$. Since $A$ is completely determined by $R$ and the boundary assignement $\partial$, we sometimes write $R$ instead of $(A,R)$. Finally, propagation operations of the lens $\ell$ are denoted by $\ell.\ppg_{ij}^{R}$, $\ell.\ppg_{i\star}^{R}$. 

%\input{sections/lensesFinal/lego-para} 
%\input{sections/lensesFinal/lego-star}
%\input{sections/lensesFinal/lego-spans2lens}
%== a major update
\input{sections/lensesFinal/lego-para-new} 
\input{sections/lensesFinal/lego-star-new}
\input{sections/lensesFinal/lego-spans2lens-new}


==> sections/lensesFinal/lego-para-last-old.tex <==
\subsection{Tensorial Lego: Parallel Composition of Lenses
%Parallel constructions
}\label{sec:lego-para}

%We study how lenses can be composed. Parallel constructions are easy to manage and we will consider them in this section to get started. More challenging are sequential constructs, in which different lenses share some of their feet, and updates propagated by one lens are taken and propagated further by one or several other lenses. We consider these in the next \sectref{sec:lego-seq}

%\zdmodd{
%\subsection{Terminal categories and lenses.} A category consisting of one object and one (necessary identity) arrow is called {\em terminal}. All terminal categories are isomorphic; we fix one, whose object is denoted by $1$ while the category is denoted by \trmcat\ (bold 1). The terminal category \trmcat\ gives rise to a unique {\em terminal space} with  $\Kupd_1 = \{(id_1,id_1)\}$.
%%\mysubsection{Parallel constructions}
%%Since we now work with several lenses $\ell$, $\ekk$, \ldots, we introduce some new notation: given a lens $\ell = (\mspaA, \ppg)$, we write $\xstar{\ell}\eqdef \xstar{\mspA}$ for its set of corrs. Feet are written $\prtbf_i^\ell$ ($i$-th boundary space) and $\prt_i^\ell R$ for the $i$-th boundary of a corr $R\in\xstar{\ell}$. Propagation operations of the lens $\ell$ are denoted by $\ell.\ppg_i^R$, $\ell.\ppg_{ij}^{R}$, $\ell.\ppg_{i\star}^{R}$.
% \begin{defin}[Terminal lens \trmlens]\label{ex:TerminalLens} All spaces of $\trmlens$ but one are terminal spaces %\footnote{
% %The terminal category $\trmcat$ (see Sect.\ref{sec:notation}) can only be endowed with $\Kupd = \{(id_1,id_1)\}$ (cf. Sect.\ref{sec:modelspaces}). 
% %}, 
% say, $\spaA_i=\spaA$ for some space \spaA\ and fixed $i$, and $\spaA_j=\trmcat$ for $j\ne i$. The corr set $\R{} = \xob{\spaA}$, the boundary functions are \zdmodok{$\partial_i = \id_{\xob{\spaA}}$ and \frar{\prt_j}{\R{}}{\xob{\trmcat}} is the only possible constant mapping.}{$\prt_iA=A$ and $\prt_{j\noteq i}A=1$. }{} \spaA$_i$-updates are closed and propagated into the only update of $\spaA_j$, $j\noteq i$. \trmlens\ is a wb, invertible lens non-reflective at all its feet.\qed  
%\end{defin}
%}{}{}{10em}

\newpii{Suppose we have several clusters of \synced\ models, \ie, models within the same cluster are \synced\ but models in different clusters are independent. We can model such situations by considering a tuple of $\ell_1,...,\ell_k$, each one working over its own multimodel space $\mspA_i$, $i=1..k$. Although independent w.r.t.  data, clusters are time-related and it make sense to talk about multimodels $\nia_1^t,...,\nia_k^t$ coexisting at some time moment $t$: such a tuple of \mmodel s can be seen as  the state of the multi-multimodel $\nia_1\times\ldots\times\nia_k$ at moment $t$. As model clusters are data-independent, it seems obvious to propagate updates over the multi-\mmodel\ by composing lenses $\ell_i$ in parallel thus forming a lens $\ell_1\times\ldots\times\ell_k$. 
}{2 to be written}{-2em}

We begin with a useful auxiliary construct. 
\newcommand\thislens{\trmext{\ell}{m}}
\begin{defin}[Terminal Extension]
	Let $\ell=(\mspA,\ppg)$ be an $n$-ary lens and $m$ be a non-negative integer. Recall the notion of a terminal lens defined in Example \ref{ex:TerminalLens} on p.~\pageref{ex:TerminalLens}. Now we define $\ell$'s $m$-fold {\em terminal extension} as the $(n{+}m)$-ary lens denoted by $\thislens$ with 
	\begin{itemize}
		\item Boundary spaces: $\prtbf_1^\ell = \spaA_1, \ldots, \prtbf_n^\ell = \spaA_n, \prtbf_{n+1}^\ell = \trmcat, \ldots, \prtbf_{n+m}^\ell = \trmcat$.
		\item Corrs: $\Corrx{\thislens} \eqdef \xstar{\ell}$, and the boundary functions are $\prt_i^{\thislens}=\prt_i^\ell$ for $i\le n$ and the obvious constant mappings $\prt_i^{\thislens} R=1$ for all $n< i\le (m{+}n)$. 
		\item Operations: $(\thislens).\ppg$ are the uniquely defined trivial extensions of operations $\ell.\ppg$. \qed
	\end{itemize}  
\end{defin}
\begin{lemma} If $\ell$ is (very) wb (and invertible), then \thislens\ is (very) wb (and invertible). \qed 
\end{lemma}
\begin{defin}[Parallel Composition]\label{def:para-comp}
	Let $\ekk$ and $\ell$ be two lenses of the same arity. Their {\em multiplicative parallel composition} is the $n$-ary lens $\kl$ with 
	\begin{itemize}
		\item Boundary spaces: $\prtbf_i^{\kl} = \prtbf_i^\ekk\times \prtbf_i^\ell$ for all $1\le i \le n$, 
		\item Corrs: $\Corrx{\kl} = \xstar{\ekk}\times\xstar{\ell}$ with boundaries $\partial_i^{(\kl)}= (\partial_i^\ekk, \partial_i^\ell)$ for all $i$
		\item Operations: % of $\kl.\ppg$ defined as follows: 
		If $(\frar{u_i}{A_i}{A'_i}, \frar{v_i}{B_i}{B'_i})$ is an update of $\prtbf_i^{\kl}$ and $R\in \xstar{\ekk_i}(A_i)$ and $Q\in\xstar{\ell_i}(B_i)$ are corrs, then \[(\kl).\ppg_{ij}^{(R,Q)}(u_i,v_i) \eqdef (\ekk.\ppg_{ij}^R(u_i), \ell.\ppg_{ij}^Q(v_i))\]
		and 
		\[(\kl).\ppg_{i\star}^{(R,Q)}(u_i,v_i) \eqdef (\ekk.\ppg_{i\star}^R(u_i), \ell.\ppg_{i\star}^Q(v_i)).\]
	\end{itemize}
	Furthermore, $\Kupd_{\!A\times B}$ and $\Kdisj{}_{A\times B}$ are the obvious rearrangement of elements of $\Kupd_{A}\times \Kupd_{B}$ and $\Kdisj{}_{A}\times \Kdisj{}_{B}$. 
	\qed
\end{defin}
\begin{lemma} If $\ekk$ and $\ell$ are (very) wb (and invertible), then $\kl$ is (very) wb (and invertible).
\end{lemma}
\begin{proof}
	All verifications can be carried out componentwise.\qed
\end{proof}
The two lemmas imply
\begin{theorem}[Parallel Composition] Let $\ekk$ and $\ell$ be two lenses with, perhaps, different arities $m\le n$. Then the $n$-ary lens 
	$(\trmext{\ekk}{n-m})\times \ell$
	(the parallel composition of $\ekk$ and $\ell$) is (very) wb (and invertible) as soon as $\ell$ and $\ekk$ are such.  \qed
\end{theorem}


==> sections/lensesFinal/lego-para-new.tex <==
\subsection{Tensorial Lego: Parallel Composition of Lenses
%Parallel constructions
}\label{sec:lego-para}

%We study how lenses can be composed. Parallel constructions are easy to manage and we will consider them in this section to get started. More challenging are sequential constructs, in which different lenses share some of their feet, and updates propagated by one lens are taken and propagated further by one or several other lenses. We consider these in the next \sectref{sec:lego-seq}

%\zdmodd{
%\subsection{Terminal categories and lenses.} A category consisting of one object and one (necessary identity) arrow is called {\em terminal}. All terminal categories are isomorphic; we fix one, whose object is denoted by $1$ while the category is denoted by \trmcat\ (bold 1). The terminal category \trmcat\ gives rise to a unique {\em terminal space} with  $\Kupd_1 = \{(id_1,id_1)\}$.
%%\mysubsection{Parallel constructions}
%%Since we now work with several lenses $\ell$, $\ekk$, \ldots, we introduce some new notation: given a lens $\ell = (\mspaA, \ppg)$, we write $\xstar{\ell}\eqdef \xstar{\mspA}$ for its set of corrs. Feet are written $\prtbf_i^\ell$ ($i$-th boundary space) and $\prt_i^\ell R$ for the $i$-th boundary of a corr $R\in\xstar{\ell}$. Propagation operations of the lens $\ell$ are denoted by $\ell.\ppg_i^R$, $\ell.\ppg_{ij}^{R}$, $\ell.\ppg_{i\star}^{R}$.
% \begin{defin}[Terminal lens \trmlens]\label{ex:TerminalLens} All spaces of $\trmlens$ but one are terminal spaces %\footnote{
% %The terminal category $\trmcat$ (see Sect.\ref{sec:notation}) can only be endowed with $\Kupd = \{(id_1,id_1)\}$ (cf. Sect.\ref{sec:modelspaces}). 
% %}, 
% say, $\spaA_i=\spaA$ for some space \spaA\ and fixed $i$, and $\spaA_j=\trmcat$ for $j\ne i$. The corr set $\R{} = \xob{\spaA}$, the boundary functions are \zdmodok{$\partial_i = \id_{\xob{\spaA}}$ and \frar{\prt_j}{\R{}}{\xob{\trmcat}} is the only possible constant mapping.}{$\prt_iA=A$ and $\prt_{j\noteq i}A=1$. }{} \spaA$_i$-updates are closed and propagated into the only update of $\spaA_j$, $j\noteq i$. \trmlens\ is a wb, invertible lens non-reflective at all its feet.\qed  
%\end{defin}
%}{}{}{10em}

We begin with a useful auxiliary construct. 
\newcommand\thislens{\trmext{\ell}{m}}
\begin{defin}[Terminal Extension]
	Let $\ell=(\mspA,\ppg)$ be an $n$-ary lens and $m$ be a non-negative integer. Then $\ell$'s $m$-fold {\em terminal extension} (cf. Example \ref{ex:TerminalLens}) is the $(n{+}m)$-ary lens denoted by $\thislens$ with 
	\begin{itemize}
		\item Boundary spaces: $\prtbf_1^\ell = \spaA_1, \ldots, \prtbf_n^\ell = \spaA_n, \prtbf_{n+1}^\ell = \trmcat, \ldots, \prtbf_{n+m}^\ell = \trmcat$.
		\item Corrs: $(\thislens)^\bigstar \eqdef \xstar{\ell}$ has boundary functions $\prt_i^{\thislens}=\prt_i^\ell$ for $i\le n$ and the obvious constant mappings $\prt_i^{\thislens} R=1$ for all $n< i\le (m{+}n)$. 
		\item Operations: $(\trmext{\ell}{m}).\ppg$ are the uniquely defined trivial extensions of operations $\ell.\ppg$. \qed
	\end{itemize}  
\end{defin}
\begin{lemma} If $\ell$ is (very) wb (and invertible), then \trmext\ is (very) wb (and invertible). \qed 
\end{lemma}
\begin{defin}[Parallel Composition]\label{def:para-comp}
	Let $\ekk$ and $\ell$ be two lenses of the same arity. Their {\em multiplicative parallel composition} is the $n$-ary lens $\kl$ with 
	\begin{itemize}
		\item Boundary spaces: $\prtbf_i^{\kl} = \prtbf_i^\ekk\times \prtbf_i^\ell$ for all $1\le i \le n$, 
		\item Corrs: $\xstar{(\kl)} = \xstar{\ekk}\times\xstar{\ell}$ with boundaries $\partial_i^{(\kl)}= (\partial_i^\ekk, \partial_i^\ell)$ for all $i$
		\item Operations: % of $\kl.\ppg$ defined as follows: 
		If $(\frar{u_i}{A_i}{A'_i}, \frar{v_i}{B_i}{B'_i})$ is an update of $\prtbf_i^{\kl}$ and $R\in \xstar{\ekk_i}(A_i)$ and $Q\in\xstar{\ell_i}(B_i)$ are corrs, then \[(\kl).\ppg_{ij}^{(R,Q)}(u_i,v_i) \eqdef (\ekk.\ppg_{ij}^R(u_i), \ell.\ppg_{ij}^Q(v_i))\]
		and 
		\[(\kl).\ppg_{i\star}^{(R,Q)}(u_i,v_i) \eqdef (\ekk.\ppg_{i\star}^R(u_i), \ell.\ppg_{i\star}^Q(v_i)).\]
	\end{itemize}
	Furthermore, $\Kupd_{\!A\times B}$ and $\Kdisj{}_{A\times B}$ are the obvious rearrangement of elements of $\Kupd_{A}\times \Kupd_{B}$ and $\Kdisj{}_{A}\times \Kdisj{}_{B}$. 
	\qed
\end{defin}
\begin{lemma} If $\ekk$ and $\ell$ are (very) wb (and invertible), then $\kl$ is (very) wb (and invertible).
\end{lemma}
\begin{proof}
	All verifications can be carried out componentwise.\qed
\end{proof}
The two lemmas imply
\begin{theorem}[Parallel Composition] Let $\ekk$ and $\ell$ be two lenses with, perhaps, different arities $m\le n$. Then the $n$-ary lens 
	$(\trmext{\ekk}{n-m})\times \ell$
	(the parallel composition of $\ekk$ and $\ell$) is (very) wb (and invertible) as soon as $\ell$ and $\ekk$ are such.  \qed
\end{theorem}


==> sections/lensesFinal/lego-para.tex <==
\subsection{Tensorial Lego: Parallel Composition of Lenses
%Parallel constructions
}\label{sec:lego-para}

%We study how lenses can be composed. Parallel constructions are easy to manage and we will consider them in this section to get started. More challenging are sequential constructs, in which different lenses share some of their feet, and updates propagated by one lens are taken and propagated further by one or several other lenses. We consider these in the next \sectref{sec:lego-seq}

%\zdmodd{
%\subsection{Terminal categories and lenses.} A category consisting of one object and one (necessary identity) arrow is called {\em terminal}. All terminal categories are isomorphic; we fix one, whose object is denoted by $1$ while the category is denoted by \trmcat\ (bold 1). The terminal category \trmcat\ gives rise to a unique {\em terminal space} with  $\Kupd_1 = \{(id_1,id_1)\}$.
%%\mysubsection{Parallel constructions}
%%Since we now work with several lenses $\ell$, $\ekk$, \ldots, we introduce some new notation: given a lens $\ell = (\mspaA, \ppg)$, we write $\xstar{\ell}\eqdef \xstar{\mspA}$ for its set of corrs. Feet are written $\prtbf_i^\ell$ ($i$-th boundary space) and $\prt_i^\ell R$ for the $i$-th boundary of a corr $R\in\xstar{\ell}$. Propagation operations of the lens $\ell$ are denoted by $\ell.\ppg_i^R$, $\ell.\ppg_{ij}^{R}$, $\ell.\ppg_{i\star}^{R}$.
% \begin{defin}[Terminal lens \trmlens]\label{ex:TerminalLens} All spaces of $\trmlens$ but one are terminal spaces %\footnote{
% %The terminal category $\trmcat$ (see Sect.\ref{sec:notation}) can only be endowed with $\Kupd = \{(id_1,id_1)\}$ (cf. Sect.\ref{sec:modelspaces}). 
% %}, 
% say, $\spaA_i=\spaA$ for some space \spaA\ and fixed $i$, and $\spaA_j=\trmcat$ for $j\ne i$. The corr set $\R{} = \xob{\spaA}$, the boundary functions are \zdmodok{$\partial_i = \id_{\xob{\spaA}}$ and \frar{\prt_j}{\R{}}{\xob{\trmcat}} is the only possible constant mapping.}{$\prt_iA=A$ and $\prt_{j\noteq i}A=1$. }{} \spaA$_i$-updates are closed and propagated into the only update of $\spaA_j$, $j\noteq i$. \trmlens\ is a wb, invertible lens non-reflective at all its feet.\qed  
%\end{defin}
%}{}{}{10em}

We begin with a useful auxiliary construct. 
\newcommand\thislens{\trmext{\ell}{m}}
\begin{defin}[Terminal Extension]
	Let $\ell=(\mspA,\ppg)$ be an $n$-ary lens and $m$ be a non-negative integer. Then $\ell$'s $m$-fold {\em terminal extension} (cf. Example \ref{ex:TerminalLens}) is the $(n{+}m)$-ary lens denoted by $\thislens$ with 
	\begin{itemize}
		\item Boundary spaces: $\prtbf_1^\ell = \spaA_1, \ldots, \prtbf_n^\ell = \spaA_n, \prtbf_{n+1}^\ell = \trmcat, \ldots, \prtbf_{n+m}^\ell = \trmcat$.
		\item Corrs: $(\thislens)^\bigstar \eqdef \xstar{\ell}$ has boundary functions $\prt_i^{\thislens}=\prt_i^\ell$ for $i\le n$ and the obvious constant mappings $\prt_i^{\thislens} R=1$ for all $n< i\le (m{+}n)$. 
		\item Operations: $(\trmext{\ell}{m}).\ppg$ are the uniquely defined trivial extensions of operations $\ell.\ppg$. \qed
	\end{itemize}  
\end{defin}
\begin{lemma} If $\ell$ is (very) wb (and invertible), then \trmext\ is (very) wb (and invertible). \qed 
\end{lemma}
\begin{defin}[Parallel Composition]\label{def:para-comp}
	Let $\ekk$ and $\ell$ be two lenses of the same arity. Their {\em multiplicative parallel composition} is the $n$-ary lens $\kl$ with 
	\begin{itemize}
		\item Boundary spaces: $\prtbf_i^{\kl} = \prtbf_i^\ekk\times \prtbf_i^\ell$ for all $1\le i \le n$, 
		\item Corrs: $\xstar{(\kl)} = \xstar{\ekk}\times\xstar{\ell}$ with boundaries $\partial_i^{(\kl)}= (\partial_i^\ekk, \partial_i^\ell)$ for all $i$
		\item Operations: % of $\kl.\ppg$ defined as follows: 
		If $(\frar{u_i}{A_i}{A'_i}, \frar{v_i}{B_i}{B'_i})$ is an update of $\prtbf_i^{\kl}$ and $R\in \xstar{\ekk_i}(A_i)$ and $Q\in\xstar{\ell_i}(B_i)$ are corrs, then \[(\kl).\ppg_{ij}^{(R,Q)}(u_i,v_i) \eqdef (\ekk.\ppg_{ij}^R(u_i), \ell.\ppg_{ij}^Q(v_i))\]
		and 
		\[(\kl).\ppg_{i\star}^{(R,Q)}(u_i,v_i) \eqdef (\ekk.\ppg_{i\star}^R(u_i), \ell.\ppg_{i\star}^Q(v_i)).\]
	\end{itemize}
	Furthermore, $\Kupd_{\!A\times B}$ and $\Kdisj{}_{A\times B}$ are the obvious rearrangement of elements of $\Kupd_{A}\times \Kupd_{B}$ and $\Kdisj{}_{A}\times \Kdisj{}_{B}$. 
	\qed
\end{defin}
\begin{lemma} If $\ekk$ and $\ell$ are (very) wb (and invertible), then $\kl$ is (very) wb (and invertible).
\end{lemma}
\begin{proof}
	All verifications can be carried out componentwise.\qed
\end{proof}
The two lemmas imply
\begin{theorem}[Parallel Composition] Let $\ekk$ and $\ell$ be two lenses with, perhaps, different arities $m\le n$. Then the $n$-ary lens 
	$(\trmext{\ekk}{n-m})\times \ell$
	(the parallel composition of $\ekk$ and $\ell$) is (very) wb (and invertible) as soon as $\ell$ and $\ekk$ are such.  \qed
\end{theorem}


==> sections/lensesFinal/lego-seq.tex <==
\subsection{Star composition}\label{sec:lego-star}

%<<<<<<< HEAD
%\input{figures/pdfs/starComposition.tex} 
%\exIntro\ Let's call $\ekk$ the $n$-ary lens with already discussed update propagations for synchronizing multimodels $(A_1A_2A_3)$ in the example in Sect.\ref{sec:example}. Suppose now that each element in $\xob{\spB_1}$ is the contents of a database table with columns for person's names, a foreign key to her address, and its employer (thus $M_1$ in Fig.\ref{fig:multiMetamod-uml} is mapped to a corresponding database schema). A consistent corr $R_1$ of lens $\ebb_1$ aligns this table contents with models in $A_1$\footnote{
%Think of a certain OR-Mapping policy.
%}. In the same way $\ebb_2$ keeps models $A_2\in \xob{\spaA_2}$ and contents $B_2$ of some other storage facility\footnote{
%\ldots with some other mapping policy}  
%in sync. In both cases, updates (from elsewhere) in the database tables are allowed. Writing new data to database table $B_i$ caused by an update $u_i:A_i\to A_I'$ certainly means that this $\spaA_i$-update is $\ebb_i$-closed, because application data $A_i$ will not additionally be amended during table access. This yields the first part of the junction condition. Now, suppose in table $B_1\in \xob{\spB_1}$ a person can only directly be added, if the company she works for is also provided, \ie\, adding Mary without its employer is impossible. If there are similar restrictions for updates of $B_2$, then the second part of the junction condition holds. 
%=======
%\input{figures/pdfs/starComposition.tex} 
%\exIntro.  
%\textit{Running example.} 

\newcommand\stepp[1]{%\par\noindent 
	{\bf Step #1:}}
\input{figures/diags/star-comp-example}
\subsubsection{\ref{sec:lego-star}.1 Running example continued.} Diagram in \figriv\ presents a refined view of our example, which explicitly includes relational storage models $B_ {1,2}$ for the two data sources. We assume that object models $A_{1,2}$ are views of data $B_{1,2 }$ that may have tables and attributes invisible in $A_{1,2}$ (in other words, we assume that views $A_i$ are projections of $B_i$). We further assume that \syncon\ of bases $B_i$ and their views $A_i$ is realized by simple {\em constant-complement} lenses $\ebb_i$, $i=1,2$ (see, \eg, \cite{jr-?}), with $R_i$ being traceability mappings.  %In more detail,  suppose that metamodels $M_{1,2}$ in  Fig.\ref{fig:multiMetamod-uml} are views of the respective relational schemas $S_{1,2}$, \eg, $S_1$ has table \Person\ with the primary key \name\ and foreign keys to tables \Addr\ and \Company, and other tables or/and attributes specifying additional data about \Person\ not visible in $M_1$. Similarly, schema $S_2$ may specify data about companies not visible in $M_2$. Then any $M_i$'s instance $A_i$ is mapped to an $S_i$' instance $B_i$ with a respective traceability mapping (corr) $R_i$, $i=1,2$.  Finally, suppose that $\ebb_i$ is a lens \syncing\ object views and their relational storage in a typical ORM-way. %$\xstar{\ebb_1}(A_1,B_1)$ is $\{R_1\}$.  %$R_1$ of lens $\ebb_1$ aligns this table with models in $A_1$
Finally, let $\ekk$ be a lens \syncing\ models $A_1,A_2,A_3$ as described in \sectref{sec:example}, and $R\inn\xstar{\ekk}(A_1,A_2,A_3)$ be a corr for some $A_3$ not shown in the figure.  

Now we consider the following update propagation scenario. 
Suppose that at some moment we have consistency $(R_1,R,R_2)$ of all five models, and then $B_1$ is changed with an update \frar{u}{B_1}{B'_1} that, say, adds to $B_1$ a record of Mary working for Google as discussed in \sectref{sec:example}. Consistency is restored in four propagation steps shown by double-arrows labeled by $x{:}y$ with $x$ the step number and $y$ the lens doing the propagation. %  
\stepp{1} lens $\ebb_1$ propagates update $u_1$ to $v'_1$ that adds (Mary, Google) to $A_1$ with no amendment to $u_1$ as $v_1$ is just a view of $u_1$ so that $B'_1=B''_1$. Note also the updated traceability mapping \corar{R'_1}{B'_1}{A'_1}. %(later we will make this requirement formal in Def.~\ref{def:wbalens}).
% 
\stepp{2}  lens $\ekk$ propagates $v'_1$ to $v''_2$ that adds (Google, Mary) to $A_2$, and amends $v'_1$ with $v''_1$ that adds (Mary, IBM) to $A''_1$; a new consistent corr $R''$ is also computed.  
%
\stepp{3} lens $\ebb_3$ propagates $v''_2$ to $u'''_2$ that adds a record of Mary's employment by Google to $B_2$ with, perhaps, some other specific relational storage changes not visible in $A_2$. We assume that no amendment to $v''_2$ is needed as 
%We also assume that update $v''_2$ (which is $\ekk$-closed by Def.~\ref{def:wblens} of a wb lens) is also $\ebb_2$-closed as 
otherwise access to relational storage would amend application data, and thus we have a consistent corr $R'''_2$ as shown. This is an important general requirement for the joint work of lenses $\ekk$ and $\ebb_2$:  $A_2$ updates delivered by $\ekk$ should be $\ebb_2$-closed. 
%
\stepp{4} lens $\ebb_1$ maps update $v''_1$ (see above in Step 2) backward to  $u'''_1$ that adds (Mary, IBM) to $B'_1$ so that $B'''_1$ includes both (Mary, Google) and (Mary, IBM) and a respective consistent corr $R'''_1$ is provided. %as all other models  in the bottom line of \figriv.  
There is no amendment for $v''_1$ as, again, otherwise access to relational storage would affect application data. 

Thus, all five models in the bottom line of \figriv\ ($A''_3$ is not shown) are mutually consistent and all show that Mary is employed by IBM and Google. \Syncon\ is restored and we can consider the entire scenario as propagation of $u_1$ to $u'''_2$ and its amendment with $u'''_1$ so that finally we have a consistent corr $(R'''_1,R'',R'''_2)$ interrelating $B'''_1, A''_3, B'''_2$. It is easy to see that amendment $u'''_1$  is compatible with $u_1$ (nothing is undone), \ie, satisfy the condition $(u_1,u'''_1)\inn\Kupd_{B'_1}$, and the other two equations required by \lawname{Reflect2-3} hold for the pair $(u_1,u'''_1)$ as well. For our simple projection view, these conditions will hold for other updates too, and we have a well-behaved propagation from $B_1$ to $B_2$ (and trivially to $A_3$). Similarly, we have a wb propagation form $B_2$ to $B_1$ and $A_3$. Thus, we have a wb ternary lens \syncing\ spaces $\spaB_1, \spaB_2$ and $\spaA_3$. 



In our case of a simple relationship between models $B_1$ and $A_1$ ($A_1$ is a projection view of $B_1$), the latter condition is obvious.  However, ensuring it and other ``lens-junction'' conditions employed above can be a challenging issue in a general situation. Below we present a simple sufficient condition to ensure a properly behaved composition for a general situation.  
% 
%Writing new data to database table $B_i$ due to $\spaA_i$-updates certainly means that all these updates are $\ebb_i$-closed: application data $A_i$ are not additionally amended during table access. This yields the second junction condition. Now, suppose in table $B_1\in \xob{\spB_1}$ a person can only be added, if the company she works for is also provided, \ie\, adding Mary without its employer is impossible. If there are similar restrictions for updates of $B_2$, then the first junction condition holds. 

%The next fact is the most important!!!
%The extended scenario now automatically enables to keep the database contents in sync: If there is any external change (not caused from $\spaA_i$-updates) in one of the databases, it is faithfully propagated to the other database tables. 

%>>>>>>> edits thru the whole paper

\vspace{-4ex}
\subsubsection{\ref{sec:lego-star}.2 Formal definition.}\label{def:star-comp}
%\input{figures/pdfs/starComposition.tex}
\input{figures/pdfs/starComposition.tex}

Suppose we have an $n$-ary lens $\ekk=(\mspaA,\ppg)$, and for every $i\le n$, a binary lens $\ebb_i =(\spaA_i, \spaB_i, \ebb_i.\ppg)$, with the first model space $\spaA_i$ being the $i$th model space of $\ekk$ (see Fig.\ref{fig:starComposition}, where $\ekk$ is depicted in the center and $\ebb_i$ are ellipses adjoint to $\ekk$'s feet).We also assume the following {\em Junction Conditions: For any $i\in\{1,\ldots,n\}$, all updates propagated to space $\spaA_i$ by lens $\ebb_i$ are $\ekk$-closed, and all updates propagated to $\spaA_i$ by lens $\ekk$ are $\ebb_i$-closed.} 

Below we will write a corr $R_i\in \xstar{\ebb_i}(A_i, B_i)$ as  \corar{\acorr_i}{A_i}{B_i}, and the sixtuple of operations $\ebb_i.\ppg^{\acorr_i}$ as the family  $\comprfam{\ebb_i.\ppg^{\acorr_i}_{xy}}{x\inn\{\spA,\spB\}, y\inn\{\spA,\spB,\star\}}$. Likewise we write $\partial_{x}$ with $x\in\{\spaA, \spaB\}$ for the boundary function of binary lenses $\ebb_i$.

The above configuration gives rise to the following consecutive update propagations: Given a model tuple $(B_1 \ldots B_n)\in \spB_1\times \cdots \times \spB_n$ and $\ebb_i$-corrs $R_i\in \xstar{\ebb_i}(A_i, B_i)$. An update \frar{v_i}{B_i}{B'_i} in $\xupd{\spB_i}$ can be propagated by $\ebb_i$. We obtain   
     \frar{u_i =\ebb_i.\ppg^{R_i}_{\spB\spA}(v_i)}{A_i}{A'_i}, \corar{R'_i=\ebb_i.\ppg^{R_i}_{\spB\star}(v_i)}{A'_i}{B'_i}. Assume now that there is a corr $R\in \xstar{\ekk}(A_1, \ldots, A_n)$, then we can propagate further via $\ekk$: \frar{u'_j=\ekk.\ppg^R_{ij}(u_i)}{A_j}{A'_j}
   for all $j\in\{1,\ldots,n\}$ where $\ekk.\ppg^R_{ii}(u_i)=\id_{A'_i}$ by the junction condition. We also obtain $R'=\ekk.\ppg^R_{i\star}(u_i)$ such that $\partial_j^\ekk R'=A'_i$ for all $i$. In the last step,  we define \frar{v'_j=\ebb_j.\ppg^{R_j}_{\spA\spB}(u'_j)}{B_j}{B'_j} and $\corar{R'_j=\ebb_j.\ppg^{\acorr_j}_{\spA\star}(u_j')} {A'_j}{B'_j}$ for all $j\noteq i$. 

%\begin{mydefin}[Star composition]\label{def:star-comp}
The star composition of the above configuration is the following $n$-ary lens $\ell$, whose carrier is the tuple of model spaces $\spaB_1, \ldots, \spaB_n$ and  corrs are tuples $(R, R_1, \ldots, R_n)$
with $R\in \xstar{\ekk}$ and $R_i\in \xstar{\ebb_i}$, such that $\partial_i^{\ekk}R = \partial_{\spaA}^{\ebb_i}R_i$ for all $i\in 1..n$. Moreover, $\partial_i^{\ell}(R, R_1, \ldots, R_n) = \partial^{\ebb_i}_{\spaB}R_i$, \ie, the $\ekk$-corr $R$ determines intermediate boundaries $A_1, \ldots, A_n$ which are extended via $\ebb_i$-corrs to the new boundaries $B_1, \ldots, B_n$, cf.\ Fig.\ref{fig:starComposition}.  

Operations are defined according to the above described consecutive update propagation process: $\ell.\ppg^{(R, R_1...R_n)}_{ij}(v_i)=v'_j$, if $j\noteq i$, $\ell.\ppg^{(R, R_1...R_n)}_{ii}(v_i)=\ebb_i.\ppg^{\acorr_i}_{\spB\spB}(v_i)$, and $\ell.\ppg^{(R, R_1....R_n)}_{i\star}(v_i)=(R', R_1'...R_n')$ (here, the second junction condition is needed). 
   We thus have a lens $\ell$ denoted by $\ekk\star(\ebb_1, \ldots, \ebb_n)$.\qed
%\end{mydefin}
\vspace{-1ex}
%\begin{theorem}[Star Composition]
%	\label{th:star-comp}
%	\begin{enumerate}
%	  \item \label{th:star-comp1}If lens $\ekk$ fulfills \lawnamebr{Stability}, all lenses $\ebb_i$ are wb, and the junction condition holds, then composition $\ekk\star(\ebb_1, \ldots, \ebb_n)$ is wb, too.
%	  \item \label{th:star-comp2}If $\ekk$ and all $\ebb_i$ are invertible, then $\ekk\star(\ebb_1, \ldots, \ebb_n)$ is invertible, too
%	\end{enumerate}
%\end{theorem}
\begin{theorem}[Star Composition]
	\label{th:star-comp}
	{\em (i)} If lens $\ekk$ fulfills \lawnamebr{Stability}, all lenses $\ebb_i$ are wb, and the junction condition holds, then composition $\ekk\star(\ebb_1, \ldots, \ebb_n)$ is wb too. {\em (ii)} If $\ekk$ and all $\ebb_i$ are invertible, then $\ekk\star(\ebb_1, \ldots, \ebb_n)$ is invertible too.
\end{theorem}
\vspace{-2ex}
\begin{proof}
%\ref{th:star-comp1}: 
(i) Proving \lawnamebr{Stability} and \lawnamebr{Reflect1} is straightforward. \lawnamebr{Reflect2-3} also follow immediately, since the first step of the above propagation procedure already enjoys idempotency by \lawnamebr{Reflect2-3} for $\ebb_i$. 
%
%\ref{th:star-comp2}: 
(ii) The six mappings $f_1 \eqdef \ebb_i.\ppg_{\spB\spA}^{R_i}$, $f_2 \eqdef \ekk.\ppg^R_{ij}$, $f_3 \eqdef \ebb_j.\ppg^{R_j}_{\spA\spB}$ and $g_3 \eqdef \ebb_j.\ppg^{R_j}_{\spB\spA}$, $g_2 \eqdef \ekk.\ppg^R_{ji}$, $g_1 \eqdef \ebb_i.\ppg^{R_i}_{\spA\spB}$ have to be investigated. Let furthermore $f\eqdef f_1;f_2;f_3$ and $g \eqdef g_3;g_2;g_1$. Law \lawnamebr{Invert} is fulfilled for $\ekk\star(\ebb_1, \ldots, \ebb_n)$, if  
$g(v_j')$ is contained in the preimage of $v_j'$ under $f$, \ie, in the set $f^{-1}(v_j')$ (this is an obvious alternative formulation of the law). Since $f^{-1}(v_j') = f_1^{-1}(f_2^{-1}(f_3^{-1}(v_j')))$, this follows from invertibility of $\ebb_j, \ekk$, and $\ebb_i$, again using the alternative formulation of \lawnamebr{Invert}.
\end{proof}
%\exIntro. %The most important consequence for the example goes here!!!! 
%Any (external) database update in one of the tables $B_i$ is propagated to the other database tables by first adjusting data in $A_i$, then using the policies of the $n$-ary lens $\ekk$ in order to keep all $A_j$'s in sync and, finally, propagating these changes back to the respective persistency layer. If wb and invertibility properties hold for $\ekk$ and for $\ebb_i$, then the lens $\ekk\star(\ebb_1,\ebb_2,\ebb_3)$ keeping in sync the three relational storages is also wb and invertible. 



==> sections/lensesFinal/lego-spans2lens-new.tex <==
\subsection{Sequential Lego 2: Assembling $n$-ary Lenses from Binary Lenses}\label{sec:lego-spans2lens}
This section shows how to assemble $n$-ary (symmetric) lenses from binary asymmetric lenses modelling view computation \cite{me-jot11}. As the latter is a typical bx, the well-behavedness of asymmetric lenses has important distinctions from well-behavedness of general (symmetric mx-tailored) lenses.
\begin{defin}[Asymmetric Lens, cf. \cite{me-jot11}]
	An {\em asymmetric lens (a-lens)} is a tuple $\ebb^{\preccurlyeq}=(\spaA,\spaB,\get, \putl)$ with \spaA\ a model space called the {\em (abstract) view}, \spaB\ a model space called the {\em base}, \flar{\get}{\spaA}{\spaB} a functor (read ``get the view''), and \putl\ a family of operations $\comprfam{\putl^B}{B\in\xob{\spaB}}$ (read ``put the view update back'') of the following arity. Provided with a view update \frar{v}{\get(B)}{A'} at the input, operation $\putl^B$ outputs a base update \frar{\putl^B_\indb(v)=u'}{B}{B''}  
	and a reflected view update \frar{\putl^B_\inda(v)=v'}{A'}{A''} 
	such that $A''=\get(B'')$. 
A view update \frar{v}{\get(B)}{A'} is called {\em closed} if $\putl^B_\inda(v)=\id_{A'}$. \qed
\end{defin}
The following is a specialization of Def.~\ref{def:wblens}, in which consistency between a base $B$ and a view $A$ is understood as equality $\get(B)=A$.
\begin{defin}[Well-behavedness]\label{def:wbalens}
An a-lens is {\em well-behaved (wb)} if it satisfies the following laws for all $B\in\xob{\spaB}$, \frar{v}{\get(B)}{A'}, and \frar{u}{B}{B'}:
%
\\[1ex]
\lawgap=1ex
\noindent \begin{tabular}{l@{\quad}l}
		\lawnamebr{Hippocr1}{\frar{u}{B}{B'}
		} & 
		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
		\\ [\lawgap]\lawnamebr{Hippocr2}{
		\frar{v}{\get(B)}{A'}
		}	& 
			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
		\\  [\lawgap] \lawnamebr{\reflectzero}{
		%\frar{v}{\get(B)}{A'}
		} &	
		%$\ppgB_{\inda}(v)\noteq \id_{A'}$ implies 
		%$A'\noteq \get(X)$ for all $X\in\xob{\spaB}$
		if $A'=\get(X)$ for some $X\inn\xob{\spB}$, then $\ppgB_{\inda}(v)=\id_{A'}$
		\\  [\lawgap] \lawnamebr{Reflect1}{
		%\frar{v}{\get(B)}{A'}
		} &	
		$(v, \ppgB_{\inda}(v))\in \Kupd_{A'}$ %for all $u_i$ 
		\\  [\lawgap] \lawnamebr{Reflect2}{
		%\frar{v}{\get(B)}{A'}
		} &
		$\ppgB_{\indb}(v;\ppgB_{\inda}(v)) = \ppgB_{\indb}(v)$
		\\ [\lawgap] \lawnamebr{PutGet}{
		%\frar{v}{\get(B)}{A'}
		} & %$_{~~~~~~}$
			%$v;v'=\get(v.\putl_\indb^B) $	% dot version
		$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version 
\end{tabular} \\
\rule{0mm}{0mm}\qed
\end{defin}
\hk{I removed subindexes because it is very likely that after the final updats, the intro piece will be on the same page}
%A wb a-lens is called {\em invertible}, if it also satisfies the law:
%
%\noindent \begin{tabular}{l@{\quad}l}
%\lawnamebr{PutGetPut}$_{~~~~~~}$&
%%$v;v'=\get(v.\putl_\indb^B) $	% dot version
%$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version
%\end{tabular}

In contrast to the general lens case, a wb a-lens features \lawname{\reflectzero} --- a sort of a self-Hippocratic law regulating the necessity of amendments: the latter is not allowed as soon as consistency can be restored without amendment. Another distinction is inclusion of a strong invertibility law \lawname{PutGet} into the definition of well-behavedness: 
 %due to historical traditions. %Subsequent results will also provide some justification for this. 
\lawname{PutGet}{} together with \lawname{Reflect2} provide (weak) invertibility: $\putl^B_\indb(\get(\putl^B_\indb(v)))=\putl^B_\indb(v)$.   
\lawname{Reflect3} is omitted as it is implied by \lawname{Reflect0} and \lawname{PutGet}.  

Any a-lens $\ebb^{\preccurlyeq} =(\spaA,\spaB,\get, \putl)$ gives rise to a binary symmetric lens $\ebb$. Its carrier consists of model spaces $\spaA$ and $\spB$, for which we assume $\Kupd$ and $\Kdisj{}$ to be defined such that the spaces are well-behaved, cf.\ Def.~\ref{def:wbspace}. The set of corrs of a pair $(A,B)\in \xob{\spA}\times \xob{\spB}$ is the singleton $\{\etosing{(A,B)}\}$ with $\prt_\spA\etosing{(A,B)}=A$ and $\prt_\spB\etosing{(A,B)}=B$, 
%the boundary mappings are the projections, 
realignment is thus trivial, and consistent corrs are exactly those \etosing{(A,B)}, for which $A = \get(B)$.

For a consistent corr $\etosing{B}={(\get(B), B)}$, we need to define six operations $\ebb.\ppghB_{\_\_}$. Below we will write the upper index as $B$ rather than $\hat B$ to ease the notation. For a  view update \frar{v}{A}{A'} and the corr \etosing{B}, we define 
 $$
\ppgB_{\spA\spB}(v)=\putl^B_\indb(v){:}\, B\to B'', \;
%
\ppgB_{\spA\spA}(v)=\putl^B_\inda(v){:}\, A'\to A'', \;
% \mbox{ and }
\ppgB_{\spA\star}(v)=\etosing{B''}
$$
 The condition $A''=\get(B'')$ for $\ebb^\preccurlyeq$ means that \etosing{B''} is again a consistent corr with the desired boundaries. For a base update \frar{u}{B}{B'} and the corr \etosing{B}, we define
$$\ppgB_{\spB\spA}(u)=\get(u),\;
\ppgB_{\spB\spB}(u)=\id_{B'},\; %and
\ppgB_{\spB\star}(u)=\etosing{B'}
$$ Functoriality of $\get$ yields consistency of $\widehat{B'}$.

\begin{defin}[Very well-behaved a-lenses] \label{def:putput_a}
		A wb a-lens is called {\em very well behaved (very wb)}, if the \corring\ binary symmetric lens is such.  %additionally fulfills \lawnamebr{PutPut}, 
		cf.  Def.~\ref{def:putput}.
Of course, this definition restricts the behaviour only for the $\putl$-part of the a-lens (hence the name of the law), since functor $\get$ is compositional anyway. \qed
\end{defin}

\begin{lemma}\label{lemma:asymm_symm} Let $\ebb^\preccurlyeq$ be a (very) wb a-lens and $\ebb$ the corresponding symmetric lens. Then all base updates of $\ebb$ are closed, and $\ebb$ is (very) wb and invertible. 
 \end{lemma}
 \begin{proof}
 Base updates are closed by the definition of $\ppg_{\spB\spB}$. Well-behavedness follows from wb-ness of $\ebb^\preccurlyeq$. Invertibility has to be proved in two directions: $\ppg_{\spaB\spaA};\ppg_{\spaA\spaB};\ppg_{\spaB\spaA} = \ppg_{\spaB\spaA}$ follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect0}, the other direction follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect2}, see the remark after Def.\ref{def:wbalens}. The ''vwb''-implication follows directly from Def.\ref{def:putput_a}. 
 \qed
 \end{proof}

  \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of (very) wb asymmetric lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ with a common base \spaB\ of all $\ebb_i^{\preccurlyeq}$ gives rise to a (very) wb symmetric lens denoted by $\Sigma_{i\le n}^\spB\ebb_i^{\preccurlyeq}$. 
\end{theorem}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent to the star-composition of Def.~\ref{def:star-comp}.3, in which lens $\ekk=\idlensnb$ (cf. Ex.~\ref{ex:idLens}) and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. The ``very wb''-part follows directly from Def.~\ref{def:putput_a}. Note that a corr in $\xstar{(\Sigma_{i=1\le n}^\spB\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries being the respective $\get_i$-images.
\qed
\end{proof}
The theorem shows that combining a-lenses in this way yields an $n$-ary symmetric lens, whose properties can automatically be inferred from the binary a-lenses.
\input{figures/pdfs/mergedMetamultimod-uml}

\exIntro. Figure~\ref{fig:mergedMetamod-uml} shows a metamodel $M^+$ obtained by merging the three metamodels $M_{1,2,3}$ from \figri\ without loss and duplication of information. In addition, for persons and companies, the identifiers of their  original model spaces can be traced back via attribute ''spaces'' 
(\Commute-objects are known to appear in space $\spA_3$ and hence do not need such an attribute). As shown in \cite{DBLP:conf/ecmdafa/KonigD17}, any consistent multimodel $(A_1...A_n, R)$ can be merged into a comprehensive model $A^+$ instantiating $M^+$. Let 
$\spB$ be the space of such together with their comprehensive updates \frar{u^+}{A^+}{A'^+}. 

For a given $i\le 3$, we can define the following a-lens $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$:
$\get_i$ takes update $u^+$ as above and outputs its restriction to the model containing only objects recorded in space $\spA_i$. Operation $\putl_i$ takes an update \frar{v_i}{A_i}{A'_i} and first propagates it to all directions as discussed in \sectref{sec:example}, then merges these propagated local updates into a comprehensive  \spaB-update between comprehensive models. This yields a span of a-lenses that implements the same \syncon\ behaviour as the symmetric lens discussed in \sectref{sec:example}.

\noindent {\em\bf  From (symmetric) lenses to spans of a-lenses.} There is also a backward transformation of (symmetric) lenses to spans of a-lenses. Let $\ell=(\mspaA, \ppg)$ be a (very) wb lens. It gives rise to the following span of (very) wb a-lenses $\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i)$   
where space $\spaB$ has objects $(A_1\ldots A_n,R)$ with $R\in (A_1\ldots A_n)^\bigstar$ a consistent corr, and arrows are the update tuples of $\mspA$. Functors $\get_i:\spaB\to \spaA_i$ are projection functors. Given $B = (\tupleAWOB, R)$ and local update \frar{u_i}{A_i}{A'_i}, let

%\noindent 
\frar{\putl^B_{i\indb}(u_i)\eqdef(u_1',..,u'_{i-1}, (u_i;u_i'), u'_{i+1},..,u_n')}
{(A_1... A_n,R)}{(A''_1... A''_n,R'')}
\\[1ex] 
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ (all $j$) and $R'' = \ppg_{i\star}^R(u_i)$. Finally, $\putl^B_{i\inda}(v_i)\eqdef\ppg^R_{ii}(u_i)$. 
Validity of \lawname{Hippocr1-2}, \lawname{Reflect0}, \lawname{PutGet} directly follows from the above definitions. This yields 
\begin{theorem}\label{theo:lens2span}
Let $\ell = (\mspA, \ppg)$ be a (very) wb symmetric lens. Then the multi-span 
\[(\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i) \mid i\le n)\]
of (very) wb a-lenses has the same synchronisation behaviour w.r.t.\ model spaces $(\prtbf_i(\mspaA)\mid i\le n)$.  
\qed
\end{theorem}

An open question is whether the span-to-lens transformation in Thm.\ref{thm:LensesFromSpans} and the lens-to-span transformation of Thm.~\ref{theo:lens2span} are mutually inverse. The results for the binary case in \cite{jr-jot17} show that this is only the case modulo certain equivalence relations. These equivalences may be different for our reflective multiary lenses, and we leave this important question for future research.  

 \endinput
 
%============= Old Version ========= 
 \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$.
% 	
  	Moreover, $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible as soon as the span satisfies the following condition%
 	\footnote{Found for the binary case by Bob Rosebrugh \cite{bob-invert}}: 
% 	$$
% 	\putl^B_{\indb i}
% 	$$
$\PP^B_i=\PP^B_j$ for all $B\in\xob{\spaB}$ and $i,j\le n$, where for given $B$ and $i$,  $\PP^B_i$ is the inverse image of 
$\xarr{\spaB}(\get_i(B),\_)$, \ie,  the set $\compr{\putl^B_{\indb i}(v_i)}{\frar{v_i}{\get_i(B)}{\_}}$. %, then $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible.
\end{theorem}
\shortlong{}{%}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent%
\footnote{To make it precise, we need to introduce a simple notion of lens equivalence, which identify lenses with the same propagation behavior but, perhaps, different sets of corrs -- see. \eg, \cite{jr-jot17}} to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images. \qed
 \end{proof} 
}
For the backward transformation of lenses to spans of a-lenses, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.
\begin{theorem}[Spans from lenses] \label{th:lens2span}Any {(not necessarily invertible) }wb lens $\ell=(\mspaA, \ppg)$ gives rise to a span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$. \\
%{\color{red}We should say already here, how $\ell$ is related to the resulting construction of Thm \ref{thm:LensesFromSpans} for $\ell_i^\preccurlyeq$, see below}
\end{theorem}
\shortlong{}{%}
\begin{proof} Let $\mspA$ have model spaces $\spaA_i$ and corr set $\R$ with corresponding boundary functions $\partial_i$. Let 
\[\spaB = \{(A_1, \ldots, A_n, R)\mid \partial_i(R) = A_i \mbox{ for all }i\}\] 
be the set of all aligned consistent multimodels and $\get_i:\spaB\to \spaA_i$ be projections, \ie\ $\get_i(A_1, \ldots, A_n, R)= A_i$ and $\get_i(u_1, \ldots, u_n)= u_i$\footnote{
Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 
}. Given $B = (A_1, \ldots, A_n, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1', \ldots, u'_{i-1}, u_i;u_i', u'_{i+1} \ldots, u_n'): (A_1, \ldots, A_n, R)\to (A_1'', \ldots, A_n'', R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is an direct consequence of the respective definitions. 
 \qed
\end{proof} 
}
%An important issue is how the two transformations, lenses to spans and spans to lenses, interact. To manage this, we need an $n$-ary counterpart of the theory of lens equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  We leave it for future work. 
It is easy to see that $\Sigma_{i\in I_\ell}\ell_i^\preccurlyeq = \ell$ for any lens $\ell$, but if we begin with a span of a-lenses $\ebb_i$, $i\in I$ build a lens $\Sigma_{i\in I}\ebb_i$ and then build the span $(\Sigma_{i\in I}\ebb_i)^\preccurlyeq_i$, the two spans are different. This difference could disappear with a suitable notion of span equivalence, which we conjecture should be a straightforward generalization of the equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  %which we think should be generalizable for the $n$-ary case. We leave it for future work. 
%
%\begin{example}
%Running
%\end{example}

\endinput
\begin{theorem}[Sequential composition]
	Let \lensar{\aekk}{\spaA}{\spaB} and  \lensar{\aell}{\spaB}{\spaC} be two wb a-lenses satisfying the following {\em junction condition}: all updates in $\spaB$ obtained by $\ekk$-propagation from \spaA\ are $\ell$-closed. Then there is a uniquely defined wb a-lens \lensar{\aekk;\aell}{\spaA}{\spaC}. %The composition is associative with identity lenses \lensar{\ell_{\id_{\spaB}}}{\spaB}{\spaB} being its units. 
\end{theorem}
 \input{figures/diags/seq-comp} 
 \textit{Proof.} Obviously, composition of \Kupd-preserving functors  
\flar{\get^\ekk}{\spaA}{\spaB} and \flar{\get^\ell}{\spaB}{\spaC} is a \Kupd-preserving functor: $\get^{\ekk;\ell}=\get^\ekk\circ\get^\ell$. Now we define $\putl^{\ekk;\ell}$. 
Let $u$ be an update as shown in \figref{fig:seq-comp} where horizontal lines are \get-corrs. Let $v=\putl^{\ekk B}_\indb(u)$, $u'=\putl^{\ekk B}_\inda(u)$, and $w=\putl^{\ell C}_\indb(v)$ (by the junction condition $v'=\id_{B''}$).  
%Finally, $u^*{=}\,\get^\ekk(v')$.  
Define $\putl^{C~\ekk;\ell}_\indb(u)=w$ and $\putl^{C~\ekk;\ell}_\inda(u)=u'$. Laws \lawname{Reflect1,2, 3} for $\ell;\ekk$ are obvious. %To prove idempotency \lawname{Reflect2}, we note that as $(v, v')\in\Kupd{B''}$ by $\ell.\lawname{Reflect}$, $u''\Kupd_{A''}u^*$ as $u''=u;u'=\get^\ekk(v)$ owing to $\Kupd$-preservation by $\get^\ekk$. Hence, by $\ekk.\lawname{PutPut}$, $\pult^{B \ekk}(u'';u^*)=\putl(u'');\putl(u^*)$
Stability and Putput are obvious too. 



==> sections/lensesFinal/lego-spans2lens.tex <==
\subsection{Sequential Lego 2: Assembling $n$-ary Lenses from Binary Lenses}\label{sec:lego-spans2lens}
This section shows how to assemble $n$-ary (symmetric) lenses from binary asymmetric lenses modelling view computation \cite{me-jot11}. As the latter is a typical bx, the well-behavedness of asymmetric lenses has important distinctions from well-behavedness of general (symmetric mx-tailored) lenses.
\begin{defin}[Asymmetric Lens, cf. \cite{me-jot11}]
	An {\em asymmetric lens (a-lens)} is a tuple $\ebb^{\preccurlyeq}=(\spaA,\spaB,\get, \putl)$ with \spaA\ a model space called the {\em (abstract) view}, \spaB\ a model space called the {\em base}, \flar{\get}{\spaA}{\spaB} a functor (read ``get the view''), and \putl\ a family of operations $\comprfam{\putl^B}{B\in\xob{\spaB}}$ (read ``put the view update back'') of the following arity. Provided with a view update \frar{v}{\get(B)}{A'} at the input, operation $\putl^B$ outputs a base update \frar{\putl^B_\indb(v)=u'}{B}{B''}  
	and a reflected view update \frar{\putl^B_\inda(v)=v'}{A'}{A''} 
	such that $A''=\get(B'')$. 
A view update \frar{v}{\get(B)}{A'} is called {\em closed} if $\putl^B_\inda(v)=\id_{A'}$. \qed
\end{defin}
The following is a specialization of Def.~\ref{def:wblens}, in which consistency between a base $B$ and a view $A$ is understood as equality $\get(B)=A$.
\begin{defin}[Well-behavedness]\label{def:wbalens}
An a-lens is {\em well-behaved (wb)} if it satisfies the following laws for all $B\in\xob{\spaB}$, \frar{v}{\get(B)}{A'}, and \frar{u}{B}{B'}:
%
\\[1ex]
\lawgap=1ex
\noindent \begin{tabular}{l@{\quad}l}
%		\lawnamebr{Hippocr1}{
%        \frar{u}{B}{B'}
%		} & 
%		if $\get(B) = \get(B')$, then $\get(u) = \id_{\get(B)}$
%		\\ [\lawgap]\lawnamebr{Hippocr2}{
%		\frar{v}{\get(B)}{A'}
%		}	& 
%			if $A'=\get{B}$, then $\ppgB_\indb(v) = \id_B$,   $\ppgB_\inda(v)=\id_{\get(B)}$
%		%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
\lawnamebr{Stability}{
	%\frar{v}{\get(B)}{A'}
}	& 
if %\frar{v}{\get(B)}{A'} is identity, 
   $v=\id_{\get(B)}$, then $\ppgB_\indb(v) = \id_B$ and  $\ppgB_\inda(v)=\id_{\get(B)}$
%$\ppgB_{\indb}(\id_{\get(B)})=\id_{B}$
		\\  [\lawgap] \lawnamebr{\reflectzero}{
		    % \frar{v}{\get(B)}{A'}
		} &	
		%$\ppgB_{\inda}(v)\noteq \id_{A'}$ implies 
		%$A'\noteq \get(X)$ for all $X\in\xob{\spaB}$
		if $A'=\get(X)$ for some $X\inn\xob{\spB}$, then $\ppgB_{\inda}(v)=\id_{A'}$
		\\  [\lawgap] \lawnamebr{Reflect1}{
		%\frar{v}{\get(B)}{A'}
		} &	
		$(v, \ppgB_{\inda}(v))\in \Kupd_{A'}$ %for all $u_i$ 
		\\  [\lawgap] \lawnamebr{Reflect2}{
		%\frar{v}{\get(B)}{A'}
		} &
		$\ppgB_{\indb}(v;\ppgB_{\inda}(v)) = \ppgB_{\indb}(v)$
		\\ [\lawgap] \lawnamebr{PutGet}{
		%\frar{v}{\get(B)}{A'}
		} & %$_{~~~~~~}$
			%$v;v'=\get(v.\putl_\indb^B) $	% dot version
		$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version 
\end{tabular} \\
\rule{0mm}{0mm}\qed
\end{defin}
%\hk{I removed subindexes because it is very likely that after the final updats, the intro piece will be on the same page}
%A wb a-lens is called {\em invertible}, if it also satisfies the law:
%
%\noindent \begin{tabular}{l@{\quad}l}
%\lawnamebr{PutGetPut}$_{~~~~~~}$&
%%$v;v'=\get(v.\putl_\indb^B) $	% dot version
%$v;\putl^B_\inda(v)=\get(\putl_\indb^B(v)) $   % bracket version
%\end{tabular}

In contrast to the general lens case, a wb a-lens features \lawname{\reflectzero} --- a sort of a self-Hippocratic law regulating the necessity of amendments: the latter is not allowed as soon as consistency can be restored without amendment. Another distinction is inclusion of a strong invertibility law \lawname{PutGet} into the definition of well-behavedness: 
 %due to historical traditions. %Subsequent results will also provide some justification for this. 
\lawname{PutGet}{} together with \lawname{Reflect2} provide (weak) invertibility: $\putl^B_\indb(\get(\putl^B_\indb(v)))=\putl^B_\indb(v)$.   
\lawname{Reflect3} is omitted as it is implied by \lawname{Reflect0} and \lawname{PutGet}.  

Any a-lens $\ebb^{\preccurlyeq} =(\spaA,\spaB,\get, \putl)$ gives rise to a binary symmetric lens $\ebb$. Its carrier consists of model spaces $\spaA$ and $\spB$, for which we assume $\Kupd$ and $\Kdisj{}$ to be defined such that the spaces are well-behaved, cf.\ Def.~\ref{def:wbspace}. The set of corrs of a pair $(A,B)\in \xob{\spA}\times \xob{\spB}$ is the singleton $\{\etosing{(A,B)}\}$ with $\prt_\spA\etosing{(A,B)}=A$ and $\prt_\spB\etosing{(A,B)}=B$, 
%the boundary mappings are the projections, 
\zdhl{realignment is thus trivial}{ALIGH}, and consistent corrs are exactly those \etosing{(A,B)}, for which $A = \get(B)$.

For a consistent corr $\etosing{B}={(\get(B), B)}$, we need to define six operations $\ebb.\ppghB_{\_\_}$. Below we will write the upper index as $B$ rather than $\hat B$ to ease the notation. For a  view update \frar{v}{A}{A'} and the corr \etosing{B}, we define 
 $$
\ppgB_{\spA\spB}(v)=\putl^B_\indb(v){:}\, B\to B'', \;
%
\ppgB_{\spA\spA}(v)=\putl^B_\inda(v){:}\, A'\to A'', \;
% \mbox{ and }
\ppgB_{\spA\star}(v)=\etosing{B''}
$$
 The condition $A''=\get(B'')$ for $\ebb^\preccurlyeq$ means that \etosing{B''} is again a consistent corr with the desired boundaries. For a base update \frar{u}{B}{B'} and the corr \etosing{B}, we define
$$\ppgB_{\spB\spA}(u)=\get(u),\;
\ppgB_{\spB\spB}(u)=\id_{B'},\; %and
\ppgB_{\spB\star}(u)=\etosing{B'}
$$ Functoriality of $\get$ yields consistency of $\widehat{B'}$.

\begin{defin}[Very well-behaved a-lenses] \label{def:putput_a}
		A wb a-lens is called {\em very well behaved (very wb)}, if the \corring\ binary symmetric lens is such.  %additionally fulfills \lawnamebr{PutPut}, 
		cf.  Def.~\ref{def:putput}.
Of course, this definition restricts the behaviour only for the $\putl$-part of the a-lens (hence the name of the law), since functor $\get$ is compositional anyway. \qed
\end{defin}

\begin{lemma}\label{lemma:asymm_symm} Let $\ebb^\preccurlyeq$ be a (very) wb a-lens and $\ebb$ the corresponding symmetric lens. Then all base updates of $\ebb$ are closed, and $\ebb$ is (very) wb and invertible. 
 \end{lemma}
 \begin{proof}
 Base updates are closed by the definition of $\ppg_{\spB\spB}$. Well-behavedness follows from wb-ness of $\ebb^\preccurlyeq$. Invertibility has to be proved in two directions: $\ppg_{\spaB\spaA};\ppg_{\spaA\spaB};\ppg_{\spaB\spaA} = \ppg_{\spaB\spaA}$ follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect0}, the other direction follows from \lawnamebr{PutGet}{} and \lawnamebr{Reflect2}, see the remark after Def.\ref{def:wbalens}. The ''vwb''-implication follows directly from Def.\ref{def:putput_a}. 
 \qed
 \end{proof}

  \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of (very) wb asymmetric lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ with a common base \spaB\ of all $\ebb_i^{\preccurlyeq}$ gives rise to a (very) wb symmetric lens denoted by $\Sigma_{i\le n}^\spB\ebb_i^{\preccurlyeq}$. 
\end{theorem}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent to the star-composition of Def.~\ref{def:star-comp}.3, in which lens $\ekk=\idlensnb$ (cf. Ex.~\ref{ex:idLens}) and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. The ``very wb''-part follows directly from Def.~\ref{def:putput_a}. Note that a corr in $\xstar{(\Sigma_{i=1\le n}^\spB\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries being the respective $\get_i$-images.
\qed
\end{proof}
The theorem shows that combining a-lenses in this way yields an $n$-ary symmetric lens, whose properties can automatically be inferred from the binary a-lenses.
\input{figures/pdfs/mergedMetamultimod-uml}

\exIntro. Figure~\ref{fig:mergedMetamod-uml} shows a metamodel $M^+$ obtained by merging the three metamodels $M_{1,2,3}$ from \figri\ without loss and duplication of information. In addition, for persons and companies, the identifiers of their  original model spaces can be traced back via attribute ''spaces'' 
(\Commute-objects are known to appear in space $\spA_3$ and hence do not need such an attribute). As shown in \cite{DBLP:conf/ecmdafa/KonigD17}, any consistent multimodel $(A_1...A_n, R)$ can be merged into a comprehensive model $A^+$ instantiating $M^+$. Let 
$\spB$ be the space of such together with their comprehensive updates \frar{u^+}{A^+}{A'^+}. 

For a given $i\le 3$, we can define the following a-lens $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$:
$\get_i$ takes update $u^+$ as above and outputs its restriction to the model containing only objects recorded in space $\spA_i$. Operation $\putl_i$ takes an update \frar{v_i}{A_i}{A'_i} and first propagates it to all directions as discussed in \sectref{sec:example}, then merges these propagated local updates into a comprehensive  \spaB-update between comprehensive models. This yields a span of a-lenses that implements the same \syncon\ behaviour as the symmetric lens discussed in \sectref{sec:example}.

\noindent {\em\bf  From (symmetric) lenses to spans of a-lenses.} There is also a backward transformation of (symmetric) lenses to spans of a-lenses. Let $\ell=(\mspaA, \ppg)$ be a (very) wb lens. It gives rise to the following span of (very) wb a-lenses $\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i)$   
where space $\spaB$ has objects $(A_1\ldots A_n,R)$ with $R\in (A_1\ldots A_n)^\bigstar$ a consistent corr, and arrows are the update tuples of $\mspA$. Functors $\get_i:\spaB\to \spaA_i$ are projection functors. Given $B = (\tupleAWOB, R)$ and local update \frar{u_i}{A_i}{A'_i}, let

%\noindent 
\frar{\putl^B_{i\indb}(u_i)\eqdef(u_1',..,u'_{i-1}, (u_i;u_i'), u'_{i+1},..,u_n')}
{(A_1... A_n,R)}{(A''_1... A''_n,R'')}
\\[1ex] 
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ (all $j$) and $R'' = \ppg_{i\star}^R(u_i)$. Finally, $\putl^B_{i\inda}(v_i)\eqdef\ppg^R_{ii}(u_i)$. 
Validity of \lawname{Hippocr1-2}, \lawname{Reflect0}, \lawname{PutGet} directly follows from the above definitions. This yields 
\begin{theorem}\label{theo:lens2span}
Let $\ell = (\mspA, \ppg)$ be a (very) wb symmetric lens. Then the multi-span 
\[(\ell_i^\preccurlyeq=(\prtbf_i(\mspaA),\spaB,\get_i, \putl_i) \mid i\le n)\]
of (very) wb a-lenses has the same synchronisation behaviour w.r.t.\ model spaces $(\prtbf_i(\mspaA)\mid i\le n)$.  
\qed
\end{theorem}

An open question is whether the span-to-lens transformation in Thm.\ref{thm:LensesFromSpans} and the lens-to-span transformation of Thm.~\ref{theo:lens2span} are mutually inverse. The results for the binary case in \cite{jr-jot17} show that this is only the case modulo certain equivalence relations. These equivalences may be different for our reflective multiary lenses, and we leave this important question for future research.  

 \endinput
 
%============= Old Version ========= 
 \begin{theorem}[Lenses from Spans]\label{thm:LensesFromSpans} An $n$-ary span of wb a-lenses $\ebb^{\preccurlyeq}_i=(\spaA_i, \spaB,$ $\get_i, \putl_i)$, $i=1..n$ (note the common base \spaB\ of all $\ebb_i$) gives rise to a wb  (symmetric) lens $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$.
% 	
  	Moreover, $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible as soon as the span satisfies the following condition%
 	\footnote{Found for the binary case by Bob Rosebrugh \cite{bob-invert}}: 
% 	$$
% 	\putl^B_{\indb i}
% 	$$
$\PP^B_i=\PP^B_j$ for all $B\in\xob{\spaB}$ and $i,j\le n$, where for given $B$ and $i$,  $\PP^B_i$ is the inverse image of 
$\xarr{\spaB}(\get_i(B),\_)$, \ie,  the set $\compr{\putl^B_{\indb i}(v_i)}{\frar{v_i}{\get_i(B)}{\_}}$. %, then $\Sigma_{i=1}^n\ebb_i^{\preccurlyeq}$ is invertible.
\end{theorem}
\shortlong{}{%}
\begin{proof}
An $n$-ary span of a-lenses $\ebb_i^{\preccurlyeq}$ (all of them interpreted as symmetric lenses $\ebb_i$ as explained above) is a construct equivalent%
\footnote{To make it precise, we need to introduce a simple notion of lens equivalence, which identify lenses with the same propagation behavior but, perhaps, different sets of corrs -- see. \eg, \cite{jr-jot17}} to the star-composition of Def.~\ref{def:star-comp}, in which lens $\ekk=\idlensna$ and peripheral lenses are lenses $\ebb_i$. The junction condition is satisfied as all base updates are $\ebb_i$-closed for all $i$ by Lemma \ref{lemma:asymm_symm}, and also trivially closed for any identity lens. The theorem thus follows from Theorem~\ref{th:star-comp}. Note that a corr in $\xstar{(\Sigma_{i=1}^n\ebb_i^{\preccurlyeq})}$ 
 is nothing but a single model $B\in\xob{\spaB}$ with boundaries the respective $\get_i$-images. \qed
 \end{proof} 
}
For the backward transformation of lenses to spans of a-lenses, we use our observation in footnote~\ref{ft:mspa-as-cat} on p.~\pageref{ft:mspa-as-cat}.
\begin{theorem}[Spans from lenses] \label{th:lens2span}Any {(not necessarily invertible) }wb lens $\ell=(\mspaA, \ppg)$ gives rise to a span of wb a-lenses $\ell_i^\preccurlyeq=(\spaA_i,\spaB,\get_i, \putl_i)$. \\
%{\color{red}We should say already here, how $\ell$ is related to the resulting construction of Thm \ref{thm:LensesFromSpans} for $\ell_i^\preccurlyeq$, see below}
\end{theorem}
\shortlong{}{%}
\begin{proof} Let $\mspA$ have model spaces $\spaA_i$ and corr set $\R$ with corresponding boundary functions $\partial_i$. Let 
\[\spaB = \{(A_1, \ldots, A_n, R)\mid \partial_i(R) = A_i \mbox{ for all }i\}\] 
be the set of all aligned consistent multimodels and $\get_i:\spaB\to \spaA_i$ be projections, \ie\ $\get_i(A_1, \ldots, A_n, R)= A_i$ and $\get_i(u_1, \ldots, u_n)= u_i$\footnote{
Recall the definition of multimodel updates in Def.\ref{def:multispace}: There is no update component for $R$ 
}. Given $B = (A_1, \ldots, A_n, R)$ and update \frar{u_i}{A_i}{A'_i}, we define
\[\putl^B_{i\indb}(u_i)=(u_1', \ldots, u'_{i-1}, u_i;u_i', u'_{i+1} \ldots, u_n'): (A_1, \ldots, A_n, R)\to (A_1'', \ldots, A_n'', R''),\]
where $u_j' \eqdef \ppg^R_{ij}(u_i)$ for all $j$, $R'' = \ppg_{i\star}^R(u_i)$ and $\putl^B_{i\inda}(v_i)=\ppg^R_{ii}(u_i)$. 

That well-behavedness carries over from $\ell$ to the a-lenses is an direct consequence of the respective definitions. 
 \qed
\end{proof} 
}
%An important issue is how the two transformations, lenses to spans and spans to lenses, interact. To manage this, we need an $n$-ary counterpart of the theory of lens equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  We leave it for future work. 
It is easy to see that $\Sigma_{i\in I_\ell}\ell_i^\preccurlyeq = \ell$ for any lens $\ell$, but if we begin with a span of a-lenses $\ebb_i$, $i\in I$ build a lens $\Sigma_{i\in I}\ebb_i$ and then build the span $(\Sigma_{i\in I}\ebb_i)^\preccurlyeq_i$, the two spans are different. This difference could disappear with a suitable notion of span equivalence, which we conjecture should be a straightforward generalization of the equivalence developed by Johnson and Rosebrugh in \cite{jr-jot17} for the binary case.  %which we think should be generalizable for the $n$-ary case. We leave it for future work. 
%
%\begin{example}
%Running
%\end{example}

\endinput
\begin{theorem}[Sequential composition]
	Let \lensar{\aekk}{\spaA}{\spaB} and  \lensar{\aell}{\spaB}{\spaC} be two wb a-lenses satisfying the following {\em junction condition}: all updates in $\spaB$ obtained by $\ekk$-propagation from \spaA\ are $\ell$-closed. Then there is a uniquely defined wb a-lens \lensar{\aekk;\aell}{\spaA}{\spaC}. %The composition is associative with identity lenses \lensar{\ell_{\id_{\spaB}}}{\spaB}{\spaB} being its units. 
\end{theorem}
 \input{figures/diags/seq-comp} 
 \textit{Proof.} Obviously, composition of \Kupd-preserving functors  
\flar{\get^\ekk}{\spaA}{\spaB} and \flar{\get^\ell}{\spaB}{\spaC} is a \Kupd-preserving functor: $\get^{\ekk;\ell}=\get^\ekk\circ\get^\ell$. Now we define $\putl^{\ekk;\ell}$. 
Let $u$ be an update as shown in \figref{fig:seq-comp} where horizontal lines are \get-corrs. Let $v=\putl^{\ekk B}_\indb(u)$, $u'=\putl^{\ekk B}_\inda(u)$, and $w=\putl^{\ell C}_\indb(v)$ (by the junction condition $v'=\id_{B''}$).  
%Finally, $u^*{=}\,\get^\ekk(v')$.  
Define $\putl^{C~\ekk;\ell}_\indb(u)=w$ and $\putl^{C~\ekk;\ell}_\inda(u)=u'$. Laws \lawname{Reflect1,2, 3} for $\ell;\ekk$ are obvious. %To prove idempotency \lawname{Reflect2}, we note that as $(v, v')\in\Kupd{B''}$ by $\ell.\lawname{Reflect}$, $u''\Kupd_{A''}u^*$ as $u''=u;u'=\get^\ekk(v)$ owing to $\Kupd$-preservation by $\get^\ekk$. Hence, by $\ekk.\lawname{PutPut}$, $\pult^{B \ekk}(u'';u^*)=\putl(u'');\putl(u^*)$
Stability and Putput are obvious too. 



==> sections/lensesFinal/lego-star-new.tex <==
\subsection{Sequential Lego 1: Star Composition}\label{sec:lego-star}

\newcommand\stepp[1]{%\par\noindent 
	{\bf Step #1:}}
\renewcommand\stepp[1]{%\par\noindent 
	{\newline\indent  \bf Step #1:}}

\input{figures/diags/star-comp-example}
\subsubsection{Running Example Continued.} Diagram in \figriv\ presents a refinement of our example, which explicitly includes relational storage models $B_ {1,2}$ for the two data sources. We assume that object models $A_{1,2}$ are simple projective views of databases $B_{1,2}$: data in $A_i$ are copied from $B_i$ without any transformation, while additional tables and attributes that $B_i$-data may have are excluded from the view  $A_i$.   Synchronisation of bases $B_i$ and their views $A_i$ can be realized by simple {\em constant-complement} lenses $\ebb_i$, $i=1,2$ (see, \eg, \cite{jrw-mscs12}), such that consistent corrs $R_i\in \xstar{\ebb_i}(B_i,A_i)$ (in fact traceability mappings) are exactly those for which the projection of $B_i$ yields $A_i$.

 Finally, let $\ekk$ be a lens \syncing\ models $A_1,A_2,A_3$ as described in \sectref{sec:example}, and $R\in\xstar{\ekk}(A_1,A_2,A_3)$ be a corr for some $A_3$ not shown in the figure.  

Consider the following update propagation scenario. 
Suppose that at some moment we have consistency $(R_1,R,R_2)$ of all five models, and then $B_1$ is updated with \frar{u_1}{B_1}{B'_1} that, say, adds to $B_1$ a record of Mary working for Google as discussed in \sectref{sec:example}. Consistency is restored with a four-step propagation procedure shown by double-arrows labeled by $x{:}y$ with $x$ the step number and $y$ the lens doing the propagation. %  
\stepp{1} lens $\ebb_1$ propagates update $u_1$ to $v'_1$ that adds (Mary, Google) to view $A_1$ with no amendment to $u_1$ as $v'_1$ is just a projection of $u_1$, thus, $B'_1=B''_1$. Note also the updated traceability mapping $R'_1\in \xstar{\ebb_1}(B'_1,A'_1)$
% 
\stepp{2}  lens $\ekk$ propagates $v'_1$ to $v''_2$ that adds (Google, Mary) to $A_2$, and amends $v'_1$ with $v''_1$ that adds (Mary, IBM) to $A'_1$; a new consistent corr $R''$ is also computed.  
%
\stepp{3} lens $\ebb_2$ propagates $v''_2$ to $u'''_2$ that adds Mary's employment by Google to $B_2$ with, perhaps, some other specific relational storage changes not visible in $A_2$. We assume no amendment to $v''_2$ as otherwise access to relational storage would amend application data. Thus we have a consistent corr $R'''_2$ as shown.
%
\stepp{4} lens $\ebb_1$ maps update $v''_1$ (see above in Step 2) backward to  $u'''_1$ that adds (Mary, IBM) to $B'_1$ so that $B'''_1$ includes both (Mary, Google) and (Mary, IBM) and a respective consistent corr $R'''_1$ is provided.  
There is no amendment for $v''_1$ by the same reason as in Step 3. 

Thus, all five models in the bottom line of \figriv\ ($A''_3$ is not shown) are mutually consistent and all show that Mary is employed by IBM and Google. \Syncon\ is restored, and we can consider the entire scenario as propagation of $u_1$ to $u'''_2$ and its amendment with $u'''_1$ so that finally we have a consistent corr $(R'''_1,R'',R'''_2)$ interrelating $B'''_1, A''_3, B'''_2$. Amendment $u'''_1$  is compatible with $u_1$ as nothing is undone and condition $(u_1,u'''_1)\in\Kupd_{B'_1}$ holds;  the other two equations required by \lawname{Reflect2-3} for the pair $(u_1,u'''_1)$ also hold. For our simple projection views, these conditions will hold for other updates too, and we have a well-behaved propagation from $B_1$ to $B_2$ (and trivially to $A_3$). Similarly, we have a wb propagation from $B_2$ to $B_1$ and $A_3$. Propagation from $A_3$ to $B_{1,2}$ is non-reflective and done in two steps: first lens $\ekk$ works, then lenses $\ebb_i$ work as described above (and updates produced by $\ekk$ are $\ebb_i$-closed). Thus, we have built a wb ternary lens \syncing\ spaces $\spaB_1, \spaB_2$ and $\spaA_3$ by joining lenses $\ebb_1$ and $\ebb_2$ to the central lens $\ekk$. 
\par
\input{figures/diags/star-comp-example-steps}
\subsubsection{Discussion.} Reflection is a crucial aspect of lens composition. The inset figure describes the scenario above as a transition system and shows that Steps 3 and 4 can be performed in either order. It is the non-trivial amendment created in Step 2 that causes the necessity of Step 4, otherwise Step 3 would finish consistency restoration (with Step 4 being an idle transition ). On the other hand, if update $v''_2$ in \figriv\ would not be closed for lens $\ebb_2$, we'd have yet another concurrent step complicating the scenario. Fortunately for our example with simple projective views, Step 4 is simple and provides a non-conflicting amendment, but the case of more complex views beyond the constant-complement class needs care and investigation. Below we specify a simple situation of lens composition with reflection a priori excluded, and leave more complex cases for future work.       

\subsubsection{Formal Definition of Star Composition}\label{def:star-comp}
Suppose we have an $n$-ary lens $\ekk=(\mspaA,\ekk.\ppg)$ with $\mspaA$ based on the model space tuple $\spA = (\spA_1\ldots \spA_n)$,  and for every $i\le n$ a binary lens $\ebb_i =(\spaB_i, \spaA_i, \ebb_i.\ppg)$, with the second model space $\spaA_i$ being the $i$th model space of $\ekk$ (see Fig.\ref{fig:starComposition}, where $\ekk$ is depicted in the center and $\ebb_i$ are shown as ellipses adjoint to $\ekk$'s feet). We also assume that the following {\em Junction Conditions} hold:\\
{\em For any $i\le n$, all updates propagated to $\spaA_i$ by lens $\ebb_i$ are $\ekk$-closed, and all updates propagated to $\spaA_i$ by lens $\ekk$ are $\ebb_i$-closed.} 

Below we will write the sixtuple of operations $\ebb_i.\ppg^{\acorr_i}$ as the family  \[\comprfam{\ebb_i.\ppg^{\acorr_i}_{xy}}{x\in\{\spA,\spB\}, y\in\{\spA,\spB,\star\}}.\] Likewise we write $\prt^{\ebb_i}_{x}$ with $x\in\{\spaA, \spaB\}$ for the boundary functions of lenses $\ebb_i$.

The above configuration gives rise to the following $n$-ary lens $\ell$. The carrier is the tuple of model spaces $\spaB_1...\spaB_n$ together with their already contained compatible consecutive updates and mergeable updates, resp. Let $B = (B_1\ldots B_n)$ be a model tuple in the carrier, then we define 
\[\xstar\ell(B) = \{(R, R_1...R_n) \mid \exists A = (A_1\ldots A_n) \inn \prod\xob{\spA}: R \in \xstar{\ekk}(A), R_i\in \xstar{\ebb_i}(B_i, A_i)\}\] 
\par 
Note that the disjointment requirement of corr sets in Def.~\ref{def:mspace} yields uniqueness of $A$ in the definition of $\xstar{\ell}(B)$. Thus the realignment function $\xstar{\ell}(u_1\ldots u_n)$ of an update tuple consisting of local updates $\frar{u_i}{B_i}{B_i'}$ can uniqueley be defined: It takes a corr tuple $(R, R_1...R_n)$ and assigns to it the tuple 
\[(R, \xstar{\ebb_1}(u_1,\id_{A_1})...\xstar{\ebb_n}(u_n,\id_{A_n})),\]
i.e.\ it aligns according to idle updates of unique $(A_1\ldots A_n)$ in lens $\ekk$.
\par
\input{figures/pdfs/starComposition.tex}
Consistent corrs are exactly the tuples $(R, R_1...R_n)$, in which $R$ and all $R_i$ are in $\Kcorr$ of their respective Multispaces. This yields $\prt_i^{\ell}(R, R_1...R_n) = \prt^{\ebb_i}_{\spaB}R_i$ (see Fig.\ref{fig:starComposition}). Propagation operations are defined as compositions of consecutive lens' executions as described below (we will use the dot notation for operation  application and write $x.\mathsf{op}$ for $\mathsf{op}(x)$, where $x$ is an argument). 
 
 Given a model tuple $(B_1...B_n)\in \spB_1\timm...\timm \spB_n$, a corr $(R, R_1...R_n)$, and update \frar{v_i}{B_i}{B'_i} in $\xupd{\spB_i}$,
 we define, first for $j\noteq i$, 
 
 $$
 v_i.\;\ell.\ppg^{(R, R_1...R_n)}_{ij}\;\eqdef\;
 v_i.(\ebb_i.\ppg_{\spB\spA}^{R_i}).
 (\ekk.\ppg^R_{ij}).
 (\ebb_j.\ppg^{R_j}_{\spA\spB}),
 $$
 
 \noindent and then 
 $v_i.\,\ell.\ppg^{(R, R_1...R_n)}_{ii}\;\eqdef\; v_i.\,\ebb_i.\ppg_{\spB\spB}^{R_i}$.
 % 
 Note that all internal amendments to $u_i=v_i.(\ebb_i.\ppg_{\spB\spA}^{R_i})$ produced by $\ekk$, and to $u'_j=u_i.(\ekk.\ppg_{ij}^{R})$
 produced by $\ebb_j$, are identities due to the Junction conditions. This allows us to set corrs properly and finish propagation with the three steps above: 
 %
 $v_i.\; \ell.\ppg^{(R,R_1...R_n)}_{i\star}\;\eqdef\;
 (R', R'_1...R'_n)
 $
 % \noindent
  where 
 %
 $R'= u_i.\,\ekk.\ppg^R_{i\star}$,  
 $R'_j=u'_j.\,\ebb_j.\ppg^{R_j}_{\spA\star}$ for $j\noteq i$, and $R'_i=v_i.\;\ebb_i.\ppg^{R_i}_{\spB\star}$.
 We thus have a lens $\ell$ denoted by $\ekk^\star(\ebb_1, \ldots, \ebb_n)$. \qed

\begin{theorem}[Star Composition]\label{th:star-comp}
Given a star configuration of lenses as above. Let all underlying model spaces be well-behaved, cf. Def.~\ref{def:wbspace}. Let lens $\ekk$ fulfill \lawname{Hippocr} and let the Junction conditions hold. Then the following statements hold: 
\begin{enumerate}
  \item\label{th:star-comp1} If all lenses $\ebb_i$ are wb, then the composed lens $\ekk^\star(\ebb_1, \ldots, \ebb_n)$ is also wb.
  \item\label{th:star-comp2} If lens $\ekk$ and all lenses $\ebb_i$ are vwb, then $\ekk^\star(\ebb_1, \ldots, \ebb_n)$ is vwb, too. 
\end{enumerate}
\end{theorem}
\begin{proof}
For part \ref{th:star-comp1} we need to show that Hippocraticness carries over. Let therefore an update tuple $\overline{u_i} = (\id_{A_1}\ldots u_i\ldots \id_{A_n})$ with $u_i:B_i\to B_i'$ and a consistent corr tuple $(R, R_1\ldots R_n)$ be given. Let the aligned corr $\xstar{\ell}(\overline{u_i})\in \Kcorr$ be consistent. Since it differs from the old one only for the $i$-th component, this means that $\ebb_i.\ppg^{R_i}_{BA}(u_i) = \id_{A_i}$ by hippocraticness of $\ebb_i$. Since $\ekk$ and the other $\ebb_j$ fulfill hippocraticness, they are  stable by corollary \ref{cor:1}, hence further propagations remain identies, as desired.   
 
\lawname{Reflect1-3} follow immediately from the definition of $\ell.\ppg_{ii}$ above, since the first step of the above propagation procedure already enjoy sequential compatibility and idempotency by \lawname{Reflect1{-}3} for $\ebb_i$. 
\par 
Part \ref{th:star-comp2}: If all model spaces are well-behaved, then operation \merge\ preserves identities, cf. Def.~\ref{def:wbspace}. Then law \lawnamebr{PutPut}\ for any lens $\ekk$ reduces to the simplified form $\ppg_{ij}^R(u_i;v_i) = \ppg_{ij}(u_i);\ppg_{ij}(v_i)$, if $u_i$ and $v_i$ are $\ekk$-closed. The Junction condition and the fact, that operation $\ppg$ preserves the $\Kupd$-property, guarantee that propagation of composed updates from $\spA_i$ to $\spA_j$ and further to $\spB_j$ is not disturbed by reflective updates. Hence, \lawnamebr{PutPut}{} carries over from $\ebb_i$ to $\ekk^\star(\ebb_1, \ldots, \ebb_n)$.  
\qed
\end{proof}
\subsubsection{Invertibility-Counterexample:} We consider a simple model space with objects $\{\perp,a,b,\ldots\}$ with a finite set of natural numbers $a,b,\ldots$. There are updates $set_x:\perp\to x$ and of course identity updates. Think of a simple system, in which a primarily undefined ($\perp$) value is set to a certain value (one of the given numbers) and is never changed again. Let especially $\spB_1$ be such a space with numbers $a=0, b=2, c=6$. Let $\spA$ be similar but now with values $a=2, b=5, c=6$, cf. Fig.~\ref{fig:counterex}, where only updates are shown and are now named $x$ instead of $set_x$.
\par
\begin{figure}
\[\xymatrix{
\spB_1 \ar@/^1pc/[rr]^{\ppg_{\spB\spA}}&\ebb_1& 
\spA \ar@/_1pc/[rr]_{\ppg_{\spA\spB}}
	\ar@/^1pc/[ll]^{\ppg_{\spA\spB}}
&\ebb_2& \spB_2\ar@/_1pc/[ll]_{\ppg_{\spB\spA}} \\
0 \ar[rr]&& 2\ar[dll]\ar[rr] && 4\ar[dll] \\
2 \ar@<-1.ex>[urr] && 5\ar@<-1.ex>[urr]\ar[dll] &&  \\
6 \ar[rr]&& \ar@<1.ex>[ll] 6\ar[rr] && 7\ar@<1.ex>[ll] \\
}
\]
\caption{Schematic description of counterexample}\label{fig:counterex}
\end{figure}
 $\ebb_1$ synchronises spaces $\spB_1$ and $\spA$. The set of corrs for a pair $(x,y)\in \xob{\spB_1}\times \xob{\spA}$ is the singleton set $\{(x,y)\}$. A corr is consistent, if and only if $x,y$ are both natural numbers or both equal to $\perp$, i.e.\ consistency means that both values have the same definedness state. Alignment is obvious (because all corr sets are singletons). Propagation functions are defined according to the arrows in Fig.~\ref{fig:counterex}, e.g.\ $\ebb_1.\ppg_{\spB\spA}^{(\perp,\perp)}(set_0) = ((0,2),set_2)$. In the same way, $\ebb_2$ is defined, the space $\spB_2$, however, contains only two numbers $4$ and $7/$ (see the right part in Fig.~\ref{fig:counterex}). In general, all propagation functions take an update $set_x$ and corr $(\perp,\perp)$ and synchronize by setting the target value to the value which is nearest to $x$.
\par 
Space $\spA$ in the middle can be extended to a (trivially hippocratic) identity lens $\ekk = \idlensna$ with $n=2$, cf.\ Example \ref{ex:idLens}, such that we obtain star composition $\ell:=\ekk^\star(\ebb_1, \ldots, \ebb_n)$,  which trivially fulfills the Junction Conditions.   
\par
For all spaces mergeable pairs are only those with at least one identitity and the same necessarily holds for $\Kupd$, hence all spaces are well-behaved, cf. Def.~\ref{def:wbspace}. It is now easy to see that 
\[\mbox{Invertibility of components}\not\Rightarrow\mbox{Invertibility of composition},\] 
because by examining all possible $\ppg$-compositions one finds that both lenses $\ebb_{1/2}$ are invertible (e.g.\ $0.(\ebb_1.\ppg_{\spB\spA}).(\ebb_1.\ppg_{\spA\spB}).(\ebb_1.\ppg_{\spB\spA}) = 2 = 0.(\ebb_1.\ppg_{\spB\spA})$). Trivially, the identity lens is invertible. But the star composed structure is not, since 
\[0.(\ekk.\ppg_{12}).(\ekk.\ppg_{21}).(\ekk.\ppg_{12}) = 7 \ne 4 = 0.\ekk.\ppg_{12}\]
(we omitted superscripts $R$, because they are clear from the context).



==> sections/lensesFinal/lego-star.tex <==
\subsection{Sequential Lego 1: Star Composition}\label{sec:lego-star}

\newcommand\stepp[1]{%\par\noindent 
	{\bf Step #1:}}
\renewcommand\stepp[1]{%\par\noindent 
	{\newline\indent  \bf Step #1:}}

\input{figures/diags/star-comp-example}
\subsubsection{Running Example Continued.} Diagram in \figriv\ presents a refinement of our example, which explicitly includes relational storage models $B_ {1,2}$ for the two data sources. We assume that object models $A_{1,2}$ are simple projective views of databases $B_{1,2}$: data in $A_i$ are copied from $B_i$ without any transformation, while additional tables and attributes that $B_i$-data may have are excluded from the view  $A_i$.   Synchronisation of bases $B_i$ and their views $A_i$ can be realized by simple {\em constant-complement} lenses $\ebb_i$, $i=1,2$ (see, \eg, \cite{jrw-mscs12}), such that consistent corrs $R_i\in \xstar{\ebb_i}(B_i,A_i)$ (in fact traceability mappings) are exactly those for which the projection of $B_i$ yields $A_i$.

 Finally, let $\ekk$ be a lens \syncing\ models $A_1,A_2,A_3$ as described in \sectref{sec:example}, and $R\in\xstar{\ekk}(A_1,A_2,A_3)$ be a corr for some $A_3$ not shown in the figure.  

Consider the following update propagation scenario. 
Suppose that at some moment we have consistency $(R_1,R,R_2)$ of all five models, and then $B_1$ is updated with \frar{u_1}{B_1}{B'_1} that, say, adds to $B_1$ a record of Mary working for Google as discussed in \sectref{sec:example}. Consistency is restored with a four-step propagation procedure shown by double-arrows labeled by $x{:}y$ with $x$ the step number and $y$ the lens doing the propagation. %  
\stepp{1} lens $\ebb_1$ propagates update $u_1$ to $v'_1$ that adds (Mary, Google) to view $A_1$ with no amendment to $u_1$ as $v'_1$ is just a projection of $u_1$, thus, $B'_1=B''_1$. Note also the updated traceability mapping $R'_1\in \xstar{\ebb_1}(B'_1,A'_1)$
% 
\stepp{2}  lens $\ekk$ propagates $v'_1$ to $v''_2$ that adds (Google, Mary) to $A_2$, and amends $v'_1$ with $v''_1$ that adds (Mary, IBM) to $A'_1$; a new consistent corr $R''$ is also computed.  
%
\stepp{3} lens $\ebb_2$ propagates $v''_2$ to $u'''_2$ that adds Mary's employment by Google to $B_2$ with, perhaps, some other specific relational storage changes not visible in $A_2$. We assume no amendment to $v''_2$ as otherwise access to relational storage would amend application data. Thus we have a consistent corr $R'''_2$ as shown.
%
\stepp{4} lens $\ebb_1$ maps update $v''_1$ (see above in Step 2) backward to  $u'''_1$ that adds (Mary, IBM) to $B'_1$ so that $B'''_1$ includes both (Mary, Google) and (Mary, IBM) and a respective consistent corr $R'''_1$ is provided.  
There is no amendment for $v''_1$ by the same reason as in Step 3. 

Thus, all five models in the bottom line of \figriv\ ($A''_3$ is not shown) are mutually consistent and all show that Mary is employed by IBM and Google. \Syncon\ is restored, and we can consider the entire scenario as propagation of $u_1$ to $u'''_2$ and its amendment with $u'''_1$ so that finally we have a consistent corr $(R'''_1,R'',R'''_2)$ interrelating $B'''_1, A''_3, B'''_2$. Amendment $u'''_1$  is compatible with $u_1$ as nothing is undone and condition $(u_1,u'''_1)\in\Kupd_{B'_1}$ holds;  the other two equations required by \lawname{Reflect2-3} for the pair $(u_1,u'''_1)$ also hold. For our simple projection views, these conditions will hold for other updates too, and we have a well-behaved propagation from $B_1$ to $B_2$ (and trivially to $A_3$). Similarly, we have a wb propagation from $B_2$ to $B_1$ and $A_3$. Propagation from $A_3$ to $B_{1,2}$ is non-reflective and done in two steps: first lens $\ekk$ works, then lenses $\ebb_i$ work as described above (and updates produced by $\ekk$ are $\ebb_i$-closed). Thus, we have built a wb ternary lens \syncing\ spaces $\spaB_1, \spaB_2$ and $\spaA_3$ by joining lenses $\ebb_1$ and $\ebb_2$ to the central lens $\ekk$. 
\par
\input{figures/diags/star-comp-example-steps}
\subsubsection{Discussion.} Reflection is a crucial aspect of lens composition. The inset figure describes the scenario above as a transition system and shows that Steps 3 and 4 can be performed in either order. It is the non-trivial amendment created in Step 2 that causes the necessity of Step 4, otherwise Step 3 would finish consistency restoration (with Step 4 being an idle transition ). On the other hand, if update $v''_2$ in \figriv\ would not be closed for lens $\ebb_2$, we'd have yet another concurrent step complicating the scenario. Fortunately for our example with simple projective views, Step 4 is simple and provides a non-conflicting amendment, but the case of more complex views beyond the constant-complement class needs care and investigation. Below we specify a simple situation of lens composition with reflection a priori excluded, and leave more complex cases for future work.       

\subsubsection{Formal Definition of Star Composition}\label{def:star-comp}
Suppose we have an $n$-ary lens $\ekk=(\mspaA,\ekk.\ppg)$ with $\mspaA$ based on the model space tuple $\spA = (\spA_1\ldots \spA_n)$,  and for every $i\le n$ a binary lens $\ebb_i =(\spaB_i, \spaA_i, \ebb_i.\ppg)$, with the second model space $\spaA_i$ being the $i$th model space of $\ekk$ (see Fig.\ref{fig:starComposition}, where $\ekk$ is depicted in the center and $\ebb_i$ are shown as ellipses adjoint to $\ekk$'s feet). We also assume that the following {\em Junction Conditions} holds for all $i\le n$:
%\begin{equation}\label{eq:junction}
%\tag*{\lawnamebr{Junction}{i}}
%\mbox{
%\begin{tabular}{l@{\quad}ll}
%\multirow{2}{*}{%\lawnamebr{}{}
%}  & % row 1
%%For any $i\le n$, all 
%All updates propagated to $\spaA_i$ by lens $\ebb_i$ are $\ekk$-closed,
%\\ [0.5ex] & % row 2
%and all updates propagated to $\spaA_i$ by lens $\ekk$ are $\ebb_i$-closed.
%\end{tabular}
%}
%\end{equation}
\begin{equation}\label{eq:junction}
\tag*{\lawnamebr{Junction}{i}}
\mbox{
	\begin{tabular}{l}
     % row 1
	%For any $i\le n$, all 
	All updates propagated to $\spaA_i$ by lens $\ebb_i$ are $\ekk$-closed,
	\\ [0.5ex] % row 2
	and all updates propagated to $\spaA_i$ by lens $\ekk$ are $\ebb_i$-closed.
	\end{tabular}
}
\end{equation}

%\lawnamebr{Junction}{}}
%\mbox{\em For any $i\le n$, all updates propagated to $\spaA_i$ by lens $\ebb_i$ are $\ekk$-closed, and all updates propagated to $\spaA_i$ by lens $\ekk$ are $\ebb_i$-closed.} 

Below we will write the sixtuple of operations $\ebb_i.\ppg^{\acorr_i}$ as the family  \[\comprfam{\ebb_i.\ppg^{\acorr_i}_{xy}}{x\in\{\spA,\spB\}, y\in\{\spA,\spB,\star\}}.\] Likewise we write $\prt^{\ebb_i}_{x}$ with $x\in\{\spaA, \spaB\}$ for the boundary functions of lenses $\ebb_i$.

The above configuration gives rise to the following $n$-ary lens $\ell$. The carrier is the tuple of model spaces $\spaB_1...\spaB_n$ together with their already contained compatible consecutive updates and mergeable updates, resp. Let $B = (B_1\ldots B_n)$ be a model tuple in the carrier, then we define 
\[\xstar\ell(B) = \{(R, R_1...R_n) \mid \exists A = (A_1\ldots A_n) \inn \prod\xob{\spA}: R \in \xstar{\ekk}(A), R_i\in \xstar{\ebb_i}(B_i, A_i)\}\] 
\par 
\zdmodd{Note that the disjointment requirement of corr sets in Def.~\ref{def:mspace} yields uniqueness of $A$ in the definition of $\xstar{\ell}(B)$. Thus the realignment function $\xstar{\ell}(u_1\ldots u_n)$ of an update tuple consisting of local updates $\frar{u_i}{B_i}{B_i'}$ can uniqueley be defined: It takes a corr tuple $(R, R_1...R_n)$ and assigns to it the tuple
	\\  %\[
$(R, \xstar{\ebb_1}(u_1,\id_{A_1})...\xstar{\ebb_n}(u_n,\id_{A_n}))$,
% \]
\\
i.e.\ it aligns according to idle updates of unique $(A_1\ldots A_n)$ in lens $\ekk$.
}{}{ALIGN}{-2em}
\par
\input{figures/pdfs/starComposition.tex}
Consistent corrs are exactly the tuples $(R, R_1...R_n)$, in which $R$ and all $R_i$ are in $\Kcorr$ of their respective Multispaces. This yields $\prt_i^{\ell}(R, R_1...R_n) = \prt^{\ebb_i}_{\spaB}R_i$ (see Fig.\ref{fig:starComposition}). Propagation operations are defined as compositions of consecutive lens' executions as described below (we will use the dot notation for operation  application and write $x.\mathsf{op}$ for $\mathsf{op}(x)$, where $x$ is an argument). 
 
 Given a model tuple $(B_1...B_n)\in \spB_1\timm...\timm \spB_n$, a corr $(R, R_1...R_n)$, and update \frar{v_i}{B_i}{B'_i} in $\xupd{\spB_i}$,
 we define, first for $j\noteq i$, 
 
 $$
 v_i.\;\ell.\ppg^{(R, R_1...R_n)}_{ij}\;\eqdef\;
 v_i.(\ebb_i.\ppg_{\spB\spA}^{R_i}).
 (\ekk.\ppg^R_{ij}).
 (\ebb_j.\ppg^{R_j}_{\spA\spB}),
 $$
 
 \noindent and then 
 $v_i.\,\ell.\ppg^{(R, R_1...R_n)}_{ii}\;\eqdef\; v_i.\,\ebb_i.\ppg_{\spB\spB}^{R_i}$.
 % 
 Note that all internal amendments to $u_i=v_i.(\ebb_i.\ppg_{\spB\spA}^{R_i})$ produced by $\ekk$, and to $u'_j=u_i.(\ekk.\ppg_{ij}^{R})$
 produced by $\ebb_j$, are identities due to the Junction conditions. This allows us to set corrs properly and finish propagation with the three steps above: 
 %
 $v_i.\; \ell.\ppg^{(R,R_1...R_n)}_{i\star}\;\eqdef\;
 (R', R'_1...R'_n)
 $
 % \noindent
  where 
 %
 $R'= u_i.\,\ekk.\ppg^R_{i\star}$,  
 $R'_j=u'_j.\,\ebb_j.\ppg^{R_j}_{\spA\star}$ for $j\noteq i$, and $R'_i=v_i.\;\ebb_i.\ppg^{R_i}_{\spB\star}$.
 We thus have a lens $\ell$ denoted by $\ekk^\star(\ebb_1, \ldots, \ebb_n)$. \qed

\begin{theorem}[Star Composition]\label{th:star-comp}
Given a star configuration of lenses as above. Let all underlying model spaces be well-behaved, cf. Def.~\ref{def:wbspace}. Let lens $\ekk$ fulfill \lawname{Hippocr} and let the Junction conditions hold. Then the following statements hold: 
\begin{enumerate}
  \item\label{th:star-comp1} If all lenses $\ebb_i$ are wb, then the composed lens $\ekk^\star(\ebb_1, \ldots, \ebb_n)$ is also wb.
  \item\label{th:star-comp2} If lens $\ekk$ and all lenses $\ebb_i$ are vwb, then $\ekk^\star(\ebb_1, \ldots, \ebb_n)$ is vwb, too. 
\end{enumerate}
\end{theorem}
\begin{proof}
For part \ref{th:star-comp1} we need to show that \zdmod{Hippocraticness}{\lawname{Stability}}{HIPPOCR} carries over. Let therefore an update tuple $\overline{u_i} = (\id_{A_1}\ldots u_i\ldots \id_{A_n})$ with $u_i:B_i\to B_i'$ and a consistent corr tuple $(R, R_1\ldots R_n)$ be given. Let the aligned corr $\xstar{\ell}(\overline{u_i})\in \Kcorr$ be consistent. Since it differs from the old one only for the $i$-th component, this means that $\ebb_i.\ppg^{R_i}_{BA}(u_i) = \id_{A_i}$ by \zdmod{hippocraticness}{}{HIPPOCR} of $\ebb_i$. \zdhl{Since $\ekk$ and the other $\ebb_j$ fulfill hippocraticness, they are  stable by corollary \ref{cor:1}, hence further propagations remain identies, as desired.}{ALIGN}   
 
\lawname{Reflect1-3} follow immediately from the definition of $\ell.\ppg_{ii}$ above, since the first step of the above propagation procedure already enjoy sequential compatibility and idempotency by \lawname{Reflect1{-}3} for $\ebb_i$. 
\par 
Part \ref{th:star-comp2}: If all model spaces are well-behaved, then operation \merge\ preserves identities, cf. Def.~\ref{def:wbspace}. Then law \lawnamebr{PutPut}\ for any lens $\ekk$ reduces to the simplified form $\ppg_{ij}^R(u_i;v_i) = \ppg_{ij}(u_i);\ppg_{ij}(v_i)$, if $u_i$ and $v_i$ are $\ekk$-closed. The Junction condition and the fact, that operation $\ppg$ preserves the $\Kupd$-property, guarantee that propagation of composed updates from $\spA_i$ to $\spA_j$ and further to $\spB_j$ is not disturbed by reflective updates. Hence, \lawnamebr{PutPut}{} carries over from $\ebb_i$ to $\ekk^\star(\ebb_1, \ldots, \ebb_n)$.  
\qed
\end{proof}
\subsubsection{Invertibility-Counterexample:} We consider a simple model space with objects $\{\perp,a,b,\ldots\}$ with a finite set of natural numbers $a,b,\ldots$. There are updates $set_x:\perp\to x$ and of course identity updates. Think of a simple system, in which a primarily undefined ($\perp$) value is set to a certain value (one of the given numbers) and is never changed again. Let especially $\spB_1$ be such a space with numbers $a=0, b=2, c=6$. Let $\spA$ be similar but now with values $a=2, b=5, c=6$, cf. Fig.~\ref{fig:counterex}, where only updates are shown and are now named $x$ instead of $set_x$.
\par
\begin{figure}
\[\xymatrix{
\spB_1 \ar@/^1pc/[rr]^{\ppg_{\spB\spA}}&\ebb_1& 
\spA \ar@/_1pc/[rr]_{\ppg_{\spA\spB}}
	\ar@/^1pc/[ll]^{\ppg_{\spA\spB}}
&\ebb_2& \spB_2\ar@/_1pc/[ll]_{\ppg_{\spB\spA}} \\
0 \ar[rr]&& 2\ar[dll]\ar[rr] && 4\ar[dll] \\
2 \ar@<-1.ex>[urr] && 5\ar@<-1.ex>[urr]\ar[dll] &&  \\
6 \ar[rr]&& \ar@<1.ex>[ll] 6\ar[rr] && 7\ar@<1.ex>[ll] \\
}
\]
\caption{Schematic description of counterexample}\label{fig:counterex}
\end{figure}
 $\ebb_1$ synchronises spaces $\spB_1$ and $\spA$. The set of corrs for a pair $(x,y)\in \xob{\spB_1}\times \xob{\spA}$ is the singleton set $\{(x,y)\}$. A corr is consistent, if and only if $x,y$ are both natural numbers or both equal to $\perp$, i.e.\ consistency means that both values have the same definedness state. Alignment is obvious (because all corr sets are singletons). Propagation functions are defined according to the arrows in Fig.~\ref{fig:counterex}, e.g.\ $\ebb_1.\ppg_{\spB\spA}^{(\perp,\perp)}(set_0) = ((0,2),set_2)$. In the same way, $\ebb_2$ is defined, the space $\spB_2$, however, contains only two numbers $4$ and $7/$ (see the right part in Fig.~\ref{fig:counterex}). In general, all propagation functions take an update $set_x$ and corr $(\perp,\perp)$ and synchronize by setting the target value to the value which is nearest to $x$.
\par 
Space $\spA$ in the middle can be extended to a (trivially hippocratic) identity lens $\ekk = \idlensna$ with $n=2$, cf.\ Example \ref{ex:idLens}, such that we obtain star composition $\ell:=\ekk^\star(\ebb_1, \ldots, \ebb_n)$,  which trivially fulfills the Junction Conditions.   
\par
For all spaces mergeable pairs are only those with at least one identitity and the same necessarily holds for $\Kupd$, hence all spaces are well-behaved, cf. Def.~\ref{def:wbspace}. It is now easy to see that 
\[\mbox{Invertibility of components}\not\Rightarrow\mbox{Invertibility of composition},\] 
because by examining all possible $\ppg$-compositions one finds that both lenses $\ebb_{1/2}$ are invertible (e.g.\ $0.(\ebb_1.\ppg_{\spB\spA}).(\ebb_1.\ppg_{\spA\spB}).(\ebb_1.\ppg_{\spB\spA}) = 2 = 0.(\ebb_1.\ppg_{\spB\spA})$). Trivially, the identity lens is invertible. But the star composed structure is not, since 
\[0.(\ekk.\ppg_{12}).(\ekk.\ppg_{21}).(\ekk.\ppg_{12}) = 7 \ne 4 = 0.\ekk.\ppg_{12}\]
(we omitted superscripts $R$, because they are clear from the context).



==> sections/lensesFinal/lego.tex <==
\section{Compositionality of Update Propagation: Playing Lego with Lenses}\label{sec:lego-seq}
We study how lenses can be composed. Assembling well-behaved and well-tested small components into a bigger one is the quintessence of software engineers working in a team. If, furthermore, a mathematical theorem guarantees that desired properties carry over from the components to the composition, additional integration tests with regard to these properties are no longer necessary. 
\par
In Sect.~\ref{sec:lego-para}, we consider the parallel composition of lenses, which is easily manageable. Sequential composition, in which different lenses share some of their feet, and updates propagated by one lens are taken and propagated further by one or several other lenses, is much more challenging and considered in the other two subsections. In \sectref{sec:lego-star}, we consider ''star-composition'', cf.\ Fig.~\ref{fig:starComposition} and show that under certain additional assumptions (very) well-behavedness carries over from the components to the composition. However, invertibility does not carry over to the composition -- we shows this with a counterexample. In \sectref{sec:lego-spans2lens}, we study how (symmetric) lenses can be assembled from asymmetric ones and prove a theorem on the preservation of properties. 
\par
Since we now work with several lenses, we need a notation for lens' components. Given a lens $\ell = (\mspaA, \ppg)$, we write $\xstar{\ell}$ 
%instead of $\xstar{\mspA}$ 
for the alignment functor in Def.~\ref{def:mspace}. Feet of an aligned multimodel $(A = (A_1\ldots A_n),R)$ are written $A_i = \prt_i^\ell R$ for the $i$-th boundary of corr $R$. Since $A$ is completely determined by $R$ and the boundary assignement $\partial$, we sometimes write $R$ instead of $(A,R)$. Finally, propagation operations of the lens $\ell$ are denoted by $\ell.\ppg_{ij}^{R}$, $\ell.\ppg_{i\star}^{R}$. 

\input{sections/lensesFinal/lego-para} 
\input{sections/lensesFinal/lego-star}
\input{sections/lensesFinal/lego-spans2lens}

==> sections/lensesFinal/modSpaces-big.tex <==
\subsection{Model Spaces}% and Correspondences}
\label{sec:modelspaces}
Basically, a {\em model space} is a category, whose nodes are called {\em model states} or just {\em models}, and arrows are {\em (directed) deltas} or {\em updates}. For an arrow \frar{u}{A}{A'}, we treat $A$ as the state of the model before update $u$, $A'$ as the state after the update, and $u$ as an update specification.  Structurally, it is a specification of correspondences between $A$ and $A'$. Operationally, it is an edit sequence (edit log) that changed $A$ to $A'$. The formalism does not prescribe what updates are, but assumes that they form a category, \ie, there may be different updates from state $A$ to state $A'$; updates are composable; and idle updates \frar{\id_A}{A}{A} (doing nothing) are the units of the composition. 

In addition, 
\begin{defin}[Model spaces] A {\em model space} is a tuple 
	
	$\spaA=(|\spaA|, \Kupd, \Kspan{}, \Kdisj{}, \merge, \rsl)$ with the following components.  
	
(i) $|\spaA|$ is a category (the {\em carrier}) of models and updates; we will often write \spA\ for |\spA|, and \xob{\spA}, \xarr{\spA} and $\spA(A,A'$) for sets of objects \xob{|\spA|}, all arrows \xarr{|\spA|}, and fixed-hom arrows $\xarr{\spA}(A,A')$ resp. 
	
(ii) $\Kupd=\comprfam{\Kupd_A\subset \spA(\_,A)\timm\spaA(A,\_)}{A\inn\xob{|\spA|}}$ is a family of {\em sequential compatibility} relations  for sequential update pairs, 

(iii) $\Kspan{}=\comprfam{\Kspan{n}_A\subset\Span^nA}{A\inn\xob{\spA}, n\ge 2}$ is a family of {\em concurrently compatible} or {\em conflict-free} spans of updates (where the black triangle aims to remind us about the span configuration). We will omit index $n$ is it is clear from the context or is not important.

(iv) $\Kdisj{}=\comprfam{\Kdisj{n}_A\subset\Kspan{n}_A}{A\inn\xob{\spA}, n\ge 2}$ is a family of spans of {\em disjoint} updates. 

(v) $\merge=\comprfam{\merge_A^n}{A\inn\xob{\spA}, n\ge 2}$ is a family of merge operations that takes a conflict-free span from $\Kspan{n}_A$ and returns a cospan as shown in \eqref{eq:mergeDef} such that $u_i=u'_i$ for all $i\le n$ and hence a unique update \frar{\Sigma_i u_i}{A}{A''} is defined.  

%(vi) $\rsl=\comprfam{\rsl^n}{n\ge 2}$ is a family of conflict resolution operations that take a span of updates $u\in\Span^n_A$ with \frar{u_i}{A}{A'_i}, and returns a family of amendments \frar{u'_i}{A'_i}{A''_i} such that the span \frar{u''_i=u_i;u'_i}{A}{A''_i}, $i\le n$ is conflict-free, \ie, $u''\in \Kspan{n}_A$.

%Operation that takes a span $u\in\Span^n_A$, resolves conflicts via \rsl, $u''=\rsl^n_A(u)\in\Kspan{n}_A$, and then merges, \frar{\Sigma_i u''_i}{A}{A'''} is denoted by $\merge^+$. %, \ie, $u^{\mathsf{iv}} = \merge^+(u)$.  

\noindent The following conditions are required to hold.  
\zd{There was an essentially updated version of those conditions, but it was lost :()}	

\smallskip\noindent
\begin{tabular}{l@{\qquad}l}
	\lawnamebr{Neutrality~\Kupd}{} &	
	$(u,\id_A)\inn\Kupd_A$, $(\id_A,u')\inn\Kupd_A$ for all $A\in\xob{\spaA}$, $u\inn{\spA}(\_,A)$, $u'\inn{\spaA}(A,\_)$
	\\ [1ex]
	\lawnamebr{Universality}{}&
	if $\tupu\in\Kspan{}_A$, then $\merge(\tupu)=\colim(\tupu)$
	%$\merge^n(\tupu)=\merge^n(\tupu^\pi)$  for any permutation $\pi\in n^n$, 
	\\
	&\zd{in normal cases, the converse should also true: $\merge(u)=\colim(u)$ implies $u\in\Kspan{}$,}
	\\
	&\zd{but taking this as a general definition of \Kspan{} needs thinking }
		\\ [1ex] 
	\lawnamebr{\Kupd\Kspan{}}{}&
		if $\tupu\in\Kspan{n}_A$, then $(u_i,u'_i)\in\Kseq_{A'_i}$ for all $i=1..n$
				\\ [1ex]
	\lawnamebr{Neutrality~\Kspan{}}{} &	
	a) $\Kspan{1}_A=\Span^1A=\spA(A,\_)$
	\\ &
	b) 	for $m\ge 1$, if $\tupu\in\Kspan{m}$, then $(\tupu,\id_{m+1}...\id_{m+k})\in\Kspan{m+k}$
	\\ [1ex]
	\lawnamebr{Restriction}{} &
	if $\tupu\in\Kspan{n}_A$ and $m$ is a ``subset'' of $n$, then $\restr{\tupu\!}{m}\in\Kspan{m}_A$
	\\ [1ex]
	\lawnamebr{yyy}{} &	
		xxxxxxxxxxxxxxxxxxxx     \qed
\end{tabular}\\
	%A {\em model space functor} from $\spaA$ to $\spaB$ is a functor $F:|\spaA|\to |\spaB|$, such that $(u,u')\hspace{-0.1em}\in \hspace{-0.1em}\Kupd_A$ implies $(F(u),F(u'))\hspace{-0.1em}\in\hspace{-0.1em}\Kupd_B$. We will denote model spaces and their carriers by the same symbol and often omit explicit mentioning of $\Kupd$.\qed  % (cf. Sect.\ref{sec:modelspaces}). 
\end{defin}
%\begin{defin}[Model Space] A {\em model space} is a category whose objects are called {\em models} and arrows are {\em deltas} or {\em updates}. We will write $\xupd{\spaA}(A,A')$ for the set of  arrows from $A$ to $A'$  to recall that they are deltas/updates. 
%\end{defin}

\zd{There was an essentially updated version of conditions above, but it was lost :()}	


==> sections/lensesFinal/modSpaces-new.tex <==
\subsection{Model Spaces, deltas and updates}% and Correspondences}
\label{sec:modelspaces}
Basically, a {\em model space} is a category, whose nodes are called {\em model states}, and arrows are {\em (directed) deltas}. % or {\em updates}. 
The latter are specifications of correspondences between model states: if model states are graphs, deltas are basically spans (binary relations) between graphs and their composition is the well-known span composition (which we  call {\em relational}). In this paper we follow an abstract seeting, in which we do not specify what deltas are: we only postulate that there may be different deltas between the same states, 
% from state $A$ to state $A'$; updates 
deltas are composable, and there are identity deltas which are the units of the composition. All these requirements are met by saying that a model space is a category.  
\input{sections/lensesFinal/piece-abstract2concrete}
	
%For an arrow \frar{u}{A}{A'}, we treat $A$ as the state of the model before update $u$, $A'$ as the state after the update, and $u$ as an update specification.  Structurally, it is a specification of correspondences between $A$ and $A'$. Operationally, it is an edit sequence (edit log) that changed $A$ to $A'$. The formalism does not prescribe what updates are, but assumes that they form a category, \ie, there may be different updates from state $A$ to state $A'$; updates are composable; and idle updates \frar{\id_A}{A}{A} (doing nothing) are the units of the composition. 


\subsubsection{Models as trajectories.}
Given a model space \spA, a {\em model} in \spA\ appears as a {\em trajectory tree} in the space \spA, \ie, as a graph mapping \frar{A}{T}{\spA}, where $T$ is a partially ordered set of version numbers considered as a graph. Objects of this graph will also be referred to as {\em (logical) time moments} and arrows are {\em (logical) updates}. Thus, an update \frar{u}{t}{t'} is mapped to a delta \frar{A(u)}{A(t)}{A(t')}, where $A(t)$ and $A(t')$ are the states of the model before and after the update, and $A(u)$ is the delta specifying the effect of the update. Let's assume for simplicity that $T$ has an initial element $t_0$ and is linearly ordered, $T=t_0<t_1<...$, and thus a model $A$ is a trajectory $A_0, A_1,...$ where $A_i=A(t_i)$. 

As a rule, we will follow the common terminological and notational tradition that ``hides'' the logical time and model-as-a-mapping constructs in the background  and thus does not carefully distinguish between models and states, \eg, we write $A$  and $A'$ for the states $A(t)$ and $A(t')$ and call them models, and thus use letter $A$ for two quite different notions. Similarly, we write \frar{u}{A}{A'} for the delta $A(u)$ and call it an {\em update delta} or often just an {\em update} so that both logical updates and their delta images are called updates. In order to stress that a delta is used without the trajectory context, we will refer to it as a {\em formal delta}. 
Usually, this ambiguous terminology and notation are easily interpreted in the right way based on the context, but sometimes we will need to be precise as described above. Specifically, we need the precise notation to formulate the following important property of model trajectories: for any model $A$ and (logical) update \frar{u}{t}{t'},
\begin{equation}\label{eq:loop=id}	
	% = loop=id law
			%\tag*{\lawnamebr{Identity}{\frar{u}{t}{t'}}}
			\tag{\lawname{Identity}} %{\frar{u}{t}{t'}}}
\mbox{$A(t)=A(t')$ implies $A(u)=\id_{A(t)}$}
\end{equation}	
That is, we state that if the model is not changed by an update, the update delta is an identity. As a rule, we will write $u^A$ for delta $A(u)$.

Logical updates can be sequentially associatively composed, which makes $T$ a category. It is argued in \cite{me-bx17} that it is reasonable to consider model  spaces as 2-categories with 2-deltas between deltas (think of the usual span morphisms), and models as (unitary) lax functors \frar{A}{T}{\spA} so that for any pair of consecutive updates \frar{u}{t}{t'}, \frar{v}{t'}{t''}, there is a 2-delta \drar{A(u,v)}{u^A;v^A}{(u;v)^A}.   	

\zd{Below is a piece to show how it can be used later}
\par
Now we need to distinguish between model state spaces \spA, \spB, etc, and model trajectory spaces $\spA^T$ etc.  Having a functor \flar{\get}{\spA}{\spB}, we obtain a functor \flar{\Get}{\spA^T}{\spB^T} by postcomposition -- it's a simple story. Getting \Put\ is more complex and needs induction. 

%First, we assume that $T$ has an initial object $t_0$ and all trajectories start at $t_0$. We will write $A_0$ for $A(t_0)$ etc. Objects in $T$ are reachable from $t_0$.
We  have a family of mappings $$\frar{\putl^B}{\spA(\get(X),\_)}{\spB(X,\_)}$$
 with $X$ ranging over \xob{\spB}. Now, given a state $B_0$ %$A_0=\get(B_0), B_0$ 
 and update \frar{u_0}{t_0}{t_1}, we define \frar{u_0^B}{B_0}{B_1} by 
$$
u_0^B = \putl^{B_0}(u_0^A),
$$
which gives us a new state $B_1$, %$A_1=\get(B_1), B_1$ 
and we can repeat the process for \frar{u_1}{t_1}{t_2} and so on. We thus obtain a mapping
$$
\frar{\Put}%
{(\spA^T\timm_{A_0=\get(X)}\xob{\spB})}%
{\spB^T_{B_0=X}}
$$
where the subscript near $\times$ indicates the pullback of \frar{t_0}{\spA^T}{\xob{\spA}} and \flar{\xob{\get}}{\xob{\spA}}{\xob{\spB}},  and    $\spB^T_{B_0=X}=\compr{B\in\spB^T}{B_0=X}$
%$$
%\frar{\Putl^B}{\spA^T_{A_0=\get(B)}}{\spB^T_{B_0=B}},
%$$ where we now need to assume an initial object $t_0$ in $T$, and $A_0=A(t_0)$, $B_0=B(t_0)$ \etc, and $\spA^T_{A_0=\get(B)}=\compr{A\in\spA^T}{A_0=\get(B)}$, similarly for $\spB^T_{B_0=B}$.  

The pairs of operations (\get, \putl) and (\Get, \Put) are different guys: the former is about formal delta processing, the latter is about updates. Particularly, to preserve Hipocraticness, we shouldn't  require $\get(l)=\id_{\get(B)}$ for any loop delta \frar{l}{B}{B}, $\get(\id)=\id$ will be sufficient due to the law \eqref{eq:loop=id}. Which does not mean that keeping Hippocr. is a must. 


\subsubsection{Compatibility relations between updates.}

We require every model space $\spA$ to be endowed with two additional constructs described in the two consecutive subsections below.  
%of update {\em merging}

\mysubsubsection{Sequential compatibility of updates} 
We assume a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
indexed by objects of \spaA, and 
specifying {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update %\frar{u}{\_}{A} 
$u$ into $A$ is compatible with update %\frar{u'}{A}{\_} 
$u'$ from $A$, if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$. For example, one could add Mary's employment at IBM ($\frar{u}{A_1}{A_1'}$) and subsequently add Ann ($\frar{u'}{A_1'}{A_1''}$) to $A'_1$ yielding a pair $(u,u')\in \Kupd_{A_1'}$ (see \cite{orejas-bx13} for a detailed discussion). Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for all $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$. 

\input{figures/diags/updMerge}
\mysubsubsection{Concurrent compatibility of updates and their merging} 
Intuitively, a pair of updates $u=(u_1, u_2)$ from a common source $A$ (\ie, a span) as shown in diagram \eqref{eq:mergeDef} is called {\em concurrently compatible}, if it can be performed in either order leading to the same result -- an update \frar{u_1+u_2}{A}{A''}. Formally, in the case of concurrent compatibility of $u_1$ and $u_2$, we require the existence of update \frar{u_1+ u_2}{A}{A''} %{A'_1{+}A'_2} 
and updates $\frar{\tilde{u_i}}{A_i'}{A''}$ such that $u_1;\tilde{u_1} = u_2;\tilde{u_2}=u_1+u_2$. Then we call updates $u_i$ {\em mergable}, \zdmodok{complement updates $\tilde{u_1},\tilde{u_2}$}{update $u_1+u_2$}{}  their {\em merge}, and
updates $\tilde{u_1},\tilde{u_2}$ {\em complements}, and write $(\tilde{u_1},\tilde{u_2})=\merge_A(u_1,u_2)$ or else $\tilde{u_i}=\merge_{A,i}(u_1,u_2)$. We will also denote the model $A''$ by $A'_1+_A A'_2$. For example, for model $A_1$ in Fig.\ref{fig:multimod-uml}, we can concurrently delete John's and add Mary's employments with IBM, or concurrently add two Mary's employments, say, with IBM and Google. But deleting Mary from the model and adding her employment with IBM are not concurrently compatible. Similarly, in $A_3$, updating addresses of different routes, or updating the \from\ and \toattr\ attributes of the same route are concurrently compatible, but deleting a route and changing its attribute are incompatible (we will also say, {\em in conflict}). %Mary's employment with Google. one could add Mary's employment at IBM ($u_1$) and concurrently add Ann ($u_2$) in $A_1$. These changes can be performed in either order, i.e.\ $\tilde{u_1}$ adds Mary's employment after Ann was added, $\tilde{u_2}$ adds Ann after Mary's employment was added yielding the merge update $\frar{u'}{A_1}{A''}$.

%A span of updates $u=(u_1...u_k)$ from a common source $A$ as shown in diagram \eqref{eq:mergeDef} is called {\em concurrently compatible} if they are entirely independent and can be performed in any interleaving order or concurrently leading to the same result--- an update \frar{u''}{A}{A''}. Then we call updates $u_i$ {\em mergable}, update $u''$ their {\em merge}, and write $u''=\merge_0(u)$, while each of the {\em complement} updates \frar{u'_i}{A'_i}{A''} such that $u_i;u'_i=u''$, $i=1..k$, is denoted by $\merge_i(u)$. For example, .......... \zd{to be completed .....}
%\hk{Let's omit the notation $\Span$ and only use \Kdisj{} (we also have no additional notation for all composable update pairs - the superset of $\Kupd$!)}
%\par
%\zd{Indeed!}
%\par

We denote the set of all mergable spans with apex $A$ by $\Kdisj{}_A$
%\subset\Span$ 
%(the black triangle aims to recall that the arity of the relation is a span). %\zd{WARNING: this now does not match notation in the new paper on ppg+} 
%\hk{I inactivated the redundant description of the merge-operation}\zd{ok}
%Thus, \merge\ is an operation that takes a mergable span of updates $u\in\Kdisj{}_A$ \subset\Span_A$ and returns an update \frar{\merge_0(u)}{A}{A''} and a cospan targeted at $A''$ whose feet are $u$'s feet. \zd{{\em it perhaps makes sense to introduce operations Feet  on spans and cospans).}}

%Suppose we have an $n$-ary span of updates as shown in the diagram \eqref{eq:updMerge}. Then we require there is an operation $\merge_n$, which produces an update \frar{u''}{A}{A''} and a cospan \frar{u'_i}{A'_i}{A''}, $i=1..n$ such that $u_i;u'_i=u''$ for all $i$. We write $(u'_1..u'_n)=\merge_n(u_1..u_n)$.

The definition of sequential and concurrent compatibility is a generalization of the notion of sequential and parallel independence of graph transformation rules \cite{gt-EEPT-2006} and below we will elaborate further on the interplay of sequentially and concurrently compatible pairs. Our definitions are, however, abstract enough to cover arbitrary conflict resolution policies (e.g.\ as described in the theory of amalagamated graph transformations \cite{DBLP:journals/jcss/BoehmFH87}) which, to a certain extent, allow merging also in case of conflicting parallel updates. \hk{I hope that this is more clear now??}  
\par
Now we define model spaces.
%In addition, we require a model space $\spA$ to be endowed with a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
%$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
%indexed by objects of \spaA, which specify {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update 
%$u$ into $A$ is {\em compatible} with update %\frar{u'}{A}{\_} 
%$u'$ from $A$ and write $(u,u')\in\Kupd_A$ or $u\Kupd_Au'$,  if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$ (see \cite{orejas-bx13} for a detailed discussion). Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for sets of all objects  in $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$. 
%%Now we define model spaces.
%\begin{defin}[Model spaces] \label{def:mspace}
%A {\em model space} is a pair 
%$\spaA=(|\spaA|, \Kupd)$ with $|\spaA|$ being a category (the {\em carrier}) of models and updates, and 
%
%$$\Kupd=\comprfam{\Kupd_A\subset |\spA|(\_,A)\timm|\spaA|(A,\_)}{A\inn\xob{|\spA|}}
%$$ 
%
%\noindent a family of {\em sequential compatibility} relations  for sequential update pairs as described above. We will often omit the bars $|$ and denote a space and its carrier category by the same symbol \spA.
%\end{defin}

\begin{defin}[Model Spaces] \label{def:mspace}
	A {\em model space} is a tuple 
	\[\spaA=(|\spaA|, \Kupd, \Kdisj{}, \merge)\]
	of the following four components. The first one is a category |\spaA| (the {\em carrier}) of {\em models} and {\em updates}. We adopt a notational convention to omit the bars $|$ and denote a space and its carrier category by the same symbol \spA. The second component is a family 
	\[\Kupd=\comprfam{\Kupd_A\subset \spA(\_,A)\timm\spaA(A,\_)}{A\inn\xob{\spA}}\]	
of {\em sequential compatibility} relations  for sequential update pairs as described above. The third and forth component are tightly coupled:
	\[\Kdisj{}=\comprfam{\Kdisj{}_A}{A\inn\xob{\spA}}\]
is a family of {\em concurrently compatible} or {\em mergable} spans of updates, and 
\[\merge =\comprfam{ \merge_A}
	%\frar{\merge^k_A}{\Kdisj{k}_A}{\spA(A,\_)\times\Cospan^k}}
	{A\inn\xob{\spA}}\]
is a family of merge operations as shown in \eqref{eq:mergeDef}. The domain of operation $\merge_A$ is exactly the set $\Kdisj{}_A$. 
We will denote the components of merge by $\merge_{A,i}$ with $i=1,2$ and omit index $A$ if they are clear from the context or not important. Writing $\merge_A(u,v)$ implicitely assumes $(u,v) \in \Kdisj{}_A$. \qed
\end{defin}
%
\begin{defin}[Well-behaved Model Spaces]\label{def:wbspace}
	\noindent A model space is well-behaved (wb) if the following conditions hold for all $A\in\xob{\spaA}$:
\begin{center}
\begin{tabular}{l@{\quad}l}
	\lawnamebr{\Kupd\ and~ Id}{} &	
	For all $u\inn{\spA}(\_,A)$, $u'\inn{\spaA}(A,\_)$: $(u,\id_A), (\id_A,u')\inn\Kupd_A$, 
	\\ [1ex]
		\lawnamebr{\Kdisj{}~and ~\Kupd}{} &
	For all $(u_1,u_2)\in\Kdisj{}_A$: $(u_i,\merge_{A,i}(u_1,u_2))\in\Kupd_{A'_i}$, $i=1..2$
	\\ [1ex]
	\lawnamebr{Merge\ and~ Id}{}& For all $\frar{u}{A}{A'}$: $\merge_A(u,\id_A) = (\id_{A'},u)$    
\end{tabular} 
\end{center} \qed
%A {\em model space functor} from $\spaA$ to $\spaB$ is a functor $F:|\spaA|\to |\spaB|$, such that $(u,u')\hspace{-0.1em}\in \hspace{-0.1em}\Kupd_A$ implies $(F(u),F(u'))\hspace{-0.1em}\in\hspace{-0.1em}\Kupd_B$. We will denote model spaces and their carriers by the same symbol and often omit explicit mentioning of $\Kupd$.\qed  % (cf. Sect.\ref{sec:modelspaces}). 
\end{defin}
Whereas the first condition is the already discussed natural property for sequential compatibility, the second requires complementing updates not to revert anything done by the other update. \footnote{
Note that we do not claim the converse, namely the existence of a concurrently compatible partner in a sequentially compatible pair.} The third requirement is again self-evident.   
%\input{figures/diags/mergeDef}


==> sections/lensesFinal/modSpaces-withTraject.tex <==
\subsection{Model Spaces, deltas and updates}% and Correspondences}
\label{sec:modelspaces}
Basically, a {\em model space} is a category, whose nodes are called {\em model states}, and arrows are {\em (directed) deltas}. % or {\em updates}. 
The latter are specifications of correspondences between model states: if model states are graphs, deltas are basically spans (binary relations) between graphs and their composition is the well-known span composition (which we  call {\em relational}). In this paper we follow an abstract seeting, in which we do not specify what deltas are: we only postulate that there may be different deltas between the same states, 
% from state $A$ to state $A'$; updates 
deltas are composable, and there are identity deltas which are the units of the composition. All these requirements are met by saying that a model space is a category.  
\input{sections/lensesFinal/piece-abstract2concrete}
	
%For an arrow \frar{u}{A}{A'}, we treat $A$ as the state of the model before update $u$, $A'$ as the state after the update, and $u$ as an update specification.  Structurally, it is a specification of correspondences between $A$ and $A'$. Operationally, it is an edit sequence (edit log) that changed $A$ to $A'$. The formalism does not prescribe what updates are, but assumes that they form a category, \ie, there may be different updates from state $A$ to state $A'$; updates are composable; and idle updates \frar{\id_A}{A}{A} (doing nothing) are the units of the composition. 


\subsubsection{Models as trajectories.}
Given a model space \spA, a {\em model} in \spA\ appears as a {\em trajectory tree} in the space \spA, \ie, as a graph mapping \frar{A}{T}{\spA}, where $T$ is a partially ordered set of version numbers considered as a graph. Objects of this graph will also be referred to as {\em (logical) time moments} and arrows are {\em (logical) updates}. Thus, an update \frar{u}{t}{t'} is mapped to a delta \frar{A(u)}{A(t)}{A(t')}, where $A(t)$ and $A(t')$ are the states of the model before and after the update, and $A(u)$ is the delta specifying the effect of the update. Let's assume for simplicity that $T$ has an initial element $t_0$ and is linearly ordered, $T=t_0<t_1<...$, and thus a model $A$ is a trajectory $A_0, A_1,...$ where $A_i=A(t_i)$. 

As a rule, we will follow the common terminological and notational tradition that ``hides'' the logical time and model-as-a-mapping constructs in the background  and thus does not carefully distinguish between models and states, \eg, we write $A$  and $A'$ for the states $A(t)$ and $A(t')$ and call them models, and thus use letter $A$ for two quite different notions. Similarly, we write \frar{u}{A}{A'} for the delta $A(u)$ and call it an {\em update delta} or often just an {\em update} so that both logical updates and their delta images are called updates. In order to stress that a delta is used without the trajectory context, we will refer to it as a {\em formal delta}. 
Usually, this ambiguous terminology and notation are easily interpreted in the right way based on the context, but sometimes we will need to be precise as described above. Specifically, we need the precise notation to formulate the following important property of model trajectories: for any model $A$ and (logical) update \frar{u}{t}{t'},
\begin{equation}\label{eq:loop=id}	
	% = loop=id law
			%\tag*{\lawnamebr{Identity}{\frar{u}{t}{t'}}}
			\tag{\lawname{Identity}} %{\frar{u}{t}{t'}}}
\mbox{$A(t)=A(t')$ implies $A(u)=\id_{A(t)}$}
\end{equation}	
That is, we state that if the model is not changed by an update, the update delta is an identity. As a rule, we will write $u^A$ for delta $A(u)$.

Logical updates can be sequentially associatively composed, which makes $T$ a category. It is argued in \cite{me-bx17} that it is reasonable to consider model  spaces as 2-categories with 2-deltas between deltas (think of the usual span morphisms), and models as (unitary) lax functors \frar{A}{T}{\spA} so that for any pair of consecutive updates \frar{u}{t}{t'}, \frar{v}{t'}{t''}, there is a 2-delta \drar{A(u,v)}{u^A;v^A}{(u;v)^A}.   	

\zd{Below is a piece to show how it can be used later}
\par
Now we need to distinguish between model state spaces \spA, \spB, etc, and model trajectory spaces $\spA^T$ etc.  Having a functor \flar{\get}{\spA}{\spB}, we obtain a functor \flar{\Get}{\spA^T}{\spB^T} by postcomposition -- it's a simple story. Getting \Put\ is more complex and needs induction. 

%First, we assume that $T$ has an initial object $t_0$ and all trajectories start at $t_0$. We will write $A_0$ for $A(t_0)$ etc. Objects in $T$ are reachable from $t_0$.
We  have a family of mappings $$\frar{\putl^B}{\spA(\get(X),\_)}{\spB(X,\_)}$$
 with $X$ ranging over \xob{\spB}. Now, given a state $B_0$ %$A_0=\get(B_0), B_0$ 
 and update \frar{u_0}{t_0}{t_1}, we define \frar{u_0^B}{B_0}{B_1} by 
$$
u_0^B = \putl^{B_0}(u_0^A),
$$
which gives us a new state $B_1$, %$A_1=\get(B_1), B_1$ 
and we can repeat the process for \frar{u_1}{t_1}{t_2} and so on. We thus obtain a mapping
$$
\frar{\Put}%
{(\spA^T\timm_{A_0=\get(X)}\xob{\spB})}%
{\spB^T_{B_0=X}}
$$
where the subscript near $\times$ indicates the pullback of \frar{t_0}{\spA^T}{\xob{\spA}} and \flar{\xob{\get}}{\xob{\spA}}{\xob{\spB}},  and    $\spB^T_{B_0=X}=\compr{B\in\spB^T}{B_0=X}$
%$$
%\frar{\Putl^B}{\spA^T_{A_0=\get(B)}}{\spB^T_{B_0=B}},
%$$ where we now need to assume an initial object $t_0$ in $T$, and $A_0=A(t_0)$, $B_0=B(t_0)$ \etc, and $\spA^T_{A_0=\get(B)}=\compr{A\in\spA^T}{A_0=\get(B)}$, similarly for $\spB^T_{B_0=B}$.  

The pairs of operations (\get, \putl) and (\Get, \Put) are different guys: the former is about formal delta processing, the latter is about updates. Particularly, to preserve Hipocraticness, we shouldn't  require $\get(l)=\id_{\get(B)}$ for any loop delta \frar{l}{B}{B}, $\get(\id)=\id$ will be sufficient due to the law \eqref{eq:loop=id}. Which does not mean that keeping Hippocr. is a must. 


\subsubsection{Compatibility relations between updates.}

We require every model space $\spA$ to be endowed with two additional constructs described in the two consecutive subsections below.  
%of update {\em merging}

\mysubsubsection{Sequential compatibility of updates} 
We assume a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
indexed by objects of \spaA, and 
specifying {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update %\frar{u}{\_}{A} 
$u$ into $A$ is compatible with update %\frar{u'}{A}{\_} 
$u'$ from $A$, if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$. For example, one could add Mary's employment at IBM ($\frar{u}{A_1}{A_1'}$) and subsequently add Ann ($\frar{u'}{A_1'}{A_1''}$) to $A'_1$ yielding a pair $(u,u')\in \Kupd_{A_1'}$ (see \cite{orejas-bx13} for a detailed discussion). Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for all $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$. 

\input{figures/diags/updMerge}
\mysubsubsection{Concurrent compatibility of updates and their merging} 
Intuitively, a pair of updates $u=(u_1, u_2)$ from a common source $A$ (\ie, a span) as shown in diagram \eqref{eq:mergeDef} is called {\em concurrently compatible}, if it can be performed in either order leading to the same result -- an update \frar{u_1+u_2}{A}{A''}. Formally, in the case of concurrent compatibility of $u_1$ and $u_2$, we require the existence of update \frar{u_1+ u_2}{A}{A''} %{A'_1{+}A'_2} 
and updates $\frar{\tilde{u_i}}{A_i'}{A''}$ such that $u_1;\tilde{u_1} = u_2;\tilde{u_2}=u_1+u_2$. Then we call updates $u_i$ {\em mergable}, \zdmodok{complement updates $\tilde{u_1},\tilde{u_2}$}{update $u_1+u_2$}{}  their {\em merge}, and
updates $\tilde{u_1},\tilde{u_2}$ {\em complements}, and write $(\tilde{u_1},\tilde{u_2})=\merge_A(u_1,u_2)$ or else $\tilde{u_i}=\merge_{A,i}(u_1,u_2)$. We will also denote the model $A''$ by $A'_1+_A A'_2$. For example, for model $A_1$ in Fig.\ref{fig:multimod-uml}, we can concurrently delete John's and add Mary's employments with IBM, or concurrently add two Mary's employments, say, with IBM and Google. But deleting Mary from the model and adding her employment with IBM are not concurrently compatible. Similarly, in $A_3$, updating addresses of different routes, or updating the \from\ and \toattr\ attributes of the same route are concurrently compatible, but deleting a route and changing its attribute are incompatible (we will also say, {\em in conflict}). %Mary's employment with Google. one could add Mary's employment at IBM ($u_1$) and concurrently add Ann ($u_2$) in $A_1$. These changes can be performed in either order, i.e.\ $\tilde{u_1}$ adds Mary's employment after Ann was added, $\tilde{u_2}$ adds Ann after Mary's employment was added yielding the merge update $\frar{u'}{A_1}{A''}$.

%A span of updates $u=(u_1...u_k)$ from a common source $A$ as shown in diagram \eqref{eq:mergeDef} is called {\em concurrently compatible} if they are entirely independent and can be performed in any interleaving order or concurrently leading to the same result--- an update \frar{u''}{A}{A''}. Then we call updates $u_i$ {\em mergable}, update $u''$ their {\em merge}, and write $u''=\merge_0(u)$, while each of the {\em complement} updates \frar{u'_i}{A'_i}{A''} such that $u_i;u'_i=u''$, $i=1..k$, is denoted by $\merge_i(u)$. For example, .......... \zd{to be completed .....}
%\hk{Let's omit the notation $\Span$ and only use \Kdisj{} (we also have no additional notation for all composable update pairs - the superset of $\Kupd$!)}
%\par
%\zd{Indeed!}
%\par

We denote the set of all mergable spans with apex $A$ by $\Kdisj{}_A$
%\subset\Span$ 
%(the black triangle aims to recall that the arity of the relation is a span). %\zd{WARNING: this now does not match notation in the new paper on ppg+} 
%\hk{I inactivated the redundant description of the merge-operation}\zd{ok}
%Thus, \merge\ is an operation that takes a mergable span of updates $u\in\Kdisj{}_A$ \subset\Span_A$ and returns an update \frar{\merge_0(u)}{A}{A''} and a cospan targeted at $A''$ whose feet are $u$'s feet. \zd{{\em it perhaps makes sense to introduce operations Feet  on spans and cospans).}}

%Suppose we have an $n$-ary span of updates as shown in the diagram \eqref{eq:updMerge}. Then we require there is an operation $\merge_n$, which produces an update \frar{u''}{A}{A''} and a cospan \frar{u'_i}{A'_i}{A''}, $i=1..n$ such that $u_i;u'_i=u''$ for all $i$. We write $(u'_1..u'_n)=\merge_n(u_1..u_n)$.

The definition of sequential and concurrent compatibility is a generalization of the notion of sequential and parallel independence of graph transformation rules \cite{gt-EEPT-2006} and below we will elaborate further on the interplay of sequentially and concurrently compatible pairs. Our definitions are, however, abstract enough to cover arbitrary conflict resolution policies (e.g.\ as described in the theory of amalagamated graph transformations \cite{DBLP:journals/jcss/BoehmFH87}) which, to a certain extent, allow merging also in case of conflicting parallel updates. \hk{I hope that this is more clear now??}  
\par
Now we define model spaces.
%In addition, we require a model space $\spA$ to be endowed with a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
%$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
%indexed by objects of \spaA, which specify {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update 
%$u$ into $A$ is {\em compatible} with update %\frar{u'}{A}{\_} 
%$u'$ from $A$ and write $(u,u')\in\Kupd_A$ or $u\Kupd_Au'$,  if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$ (see \cite{orejas-bx13} for a detailed discussion). Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for sets of all objects  in $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$. 
%%Now we define model spaces.
%\begin{defin}[Model spaces] \label{def:mspace}
%A {\em model space} is a pair 
%$\spaA=(|\spaA|, \Kupd)$ with $|\spaA|$ being a category (the {\em carrier}) of models and updates, and 
%
%$$\Kupd=\comprfam{\Kupd_A\subset |\spA|(\_,A)\timm|\spaA|(A,\_)}{A\inn\xob{|\spA|}}
%$$ 
%
%\noindent a family of {\em sequential compatibility} relations  for sequential update pairs as described above. We will often omit the bars $|$ and denote a space and its carrier category by the same symbol \spA.
%\end{defin}

\begin{defin}[Model Spaces] \label{def:mspace}
	A {\em model space} is a tuple 
	\[\spaA=(|\spaA|, \Kupd, \Kdisj{}, \merge)\]
	of the following four components. The first one is a category |\spaA| (the {\em carrier}) of {\em models} and {\em updates}. We adopt a notational convention to omit the bars $|$ and denote a space and its carrier category by the same symbol \spA. The second component is a family 
	\[\Kupd=\comprfam{\Kupd_A\subset \spA(\_,A)\timm\spaA(A,\_)}{A\inn\xob{\spA}}\]	
of {\em sequential compatibility} relations  for sequential update pairs as described above. The third and forth component are tightly coupled:
	\[\Kdisj{}=\comprfam{\Kdisj{}_A}{A\inn\xob{\spA}}\]
is a family of {\em concurrently compatible} or {\em mergable} spans of updates, and 
\[\merge =\comprfam{ \merge_A}
	%\frar{\merge^k_A}{\Kdisj{k}_A}{\spA(A,\_)\times\Cospan^k}}
	{A\inn\xob{\spA}}\]
is a family of merge operations as shown in \eqref{eq:mergeDef}. The domain of operation $\merge_A$ is exactly the set $\Kdisj{}_A$. 
We will denote the components of merge by $\merge_{A,i}$ with $i=1,2$ and omit index $A$ if they are clear from the context or not important. Writing $\merge_A(u,v)$ implicitely assumes $(u,v) \in \Kdisj{}_A$. \qed
\end{defin}
%
\begin{defin}[Well-behaved Model Spaces]\label{def:wbspace}
	\noindent A model space is well-behaved (wb) if the following conditions hold for all $A\in\xob{\spaA}$:
\begin{center}
\begin{tabular}{l@{\quad}l}
	\lawnamebr{\Kupd\ and~ Id}{} &	
	For all $u\inn{\spA}(\_,A)$, $u'\inn{\spaA}(A,\_)$: $(u,\id_A), (\id_A,u')\inn\Kupd_A$, 
	\\ [1ex]
		\lawnamebr{\Kdisj{}~and ~\Kupd}{} &
	For all $(u_1,u_2)\in\Kdisj{}_A$: $(u_i,\merge_{A,i}(u_1,u_2))\in\Kupd_{A'_i}$, $i=1..2$
	\\ [1ex]
	\lawnamebr{Merge\ and~ Id}{}& For all $\frar{u}{A}{A'}$: $\merge_A(u,\id_A) = (\id_{A'},u)$    
\end{tabular} 
\end{center} \qed
%A {\em model space functor} from $\spaA$ to $\spaB$ is a functor $F:|\spaA|\to |\spaB|$, such that $(u,u')\hspace{-0.1em}\in \hspace{-0.1em}\Kupd_A$ implies $(F(u),F(u'))\hspace{-0.1em}\in\hspace{-0.1em}\Kupd_B$. We will denote model spaces and their carriers by the same symbol and often omit explicit mentioning of $\Kupd$.\qed  % (cf. Sect.\ref{sec:modelspaces}). 
\end{defin}
Whereas the first condition is the already discussed natural property for sequential compatibility, the second requires complementing updates not to revert anything done by the other update. \footnote{
Note that we do not claim the converse, namely the existence of a concurrently compatible partner in a sequentially compatible pair.} The third requirement is again self-evident.   
%\input{figures/diags/mergeDef}


==> sections/lensesFinal/modSpaces.tex <==
\subsection{Model Spaces and updates}% and Correspondences}
\label{sec:modelspaces}
Basically, a {\em model space} is a category, whose nodes are called {\em model states} or just {\em models}, and arrows are {\em (directed) deltas} or {\em updates}. For an arrow \frar{u}{A}{A'}, we treat $A$ as the state of the model before update $u$, $A'$ as the state after the update, and $u$ as an update specification.  Structurally, it is a specification of correspondences between $A$ and $A'$. Operationally, it is an edit sequence (edit log) that changed $A$ to $A'$. The formalism does not prescribe what updates are, but assumes that they form a category, \ie, there may be different updates from state $A$ to state $A'$; updates are composable; and idle updates \frar{\id_A}{A}{A} (doing nothing) are the units of the composition. 
\hkmodok{
It is also useful to have a more concrete notion of a model space as based on a category \spE\ of models and model embeddings, and then define an update \frar{u}{A}{A'} as a span of embeddings \flar{u_l}{A}{K}  and \frar{u_r}{K}{A'} where $K$ is a submodel of $A$ consisting of all elements preserved by $u$ so that embeddings $u_l$ and $u_r$ specify the deleted and the inserted elements resp. Then a model space \spA\ appears as the category $\Span(\spE)$ for some given \spE. Two ``extreme'' cases for the latter are a) the category of graphs and their inclusions, $\gracat_\subset$, which does not distinguish between objects/references and primitive values/attributes, and b) the Object-Slot-Value model developed in \cite[Sect.3]{me-gttse09} , which does make the distinction between objects and values but does not consider references/links between objects. Integrating a) and b) gives us the category of attributed graphs \cite{gtbook06}. Some of the notions that we axiomatically define below can be given formal definitions for a concrete choice of the category \spE, and we refer to paper \cite{orejas-bx13}, in which some of these definitions can be found for $\spE=\gracat_\subset$.
}{A prominent example of model spaces is the category of graphs where updates are encoded as (certain equivalence classes of) binary spans between them. They are heaviliy used in the theory of Graph Transformations \cite{gtbook06}. In this way an update $u:A\to A'$ can be a deletion or an addition or a combination of both.}{Thus updates as spans are at least mentioned informally. The formal treatment of the span cat with equivalences and so on is too much here! }
%\zd{In general, I agree, but let's keep this piece for some and finally decide later -- I mean that a systematic use of viewing \spA\ as \Span(\spE) is not assumed but maybe there will be a place where having it will be a useful thing.}
\par
We require every model space $\spA$ to be endowed with two additional constructs described in the two consecutive subsections below.  
%of update {\em merging}

\mysubsubsection{Sequential compatibility of updates} 
We assume a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
indexed by objects of \spaA, and 
specifying {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update %\frar{u}{\_}{A} 
$u$ into $A$ is compatible with update %\frar{u'}{A}{\_} 
$u'$ from $A$, if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$. For example, one could add Mary's employment at IBM ($\frar{u}{A_1}{A_1'}$) and subsequently add Ann ($\frar{u'}{A_1'}{A_1''}$) to $A'_1$ yielding a pair $(u,u')\in \Kupd_{A_1'}$ (see \cite{orejas-bx13} for a detailed discussion). Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for all $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$. 

\input{figures/diags/updMerge}
\mysubsubsection{Concurrent compatibility of updates and their merging} 
Intuitively, a pair of updates $u=(u_1, u_2)$ from a common source $A$ (\ie, a span) as shown in diagram \eqref{eq:mergeDef} is called {\em concurrently compatible}, if it can be performed in either order leading to the same result -- an update \frar{u_1+u_2}{A}{A''}. Formally, in the case of concurrent compatibility of $u_1$ and $u_2$, we require the existence of update \frar{u_1+ u_2}{A}{A''} %{A'_1{+}A'_2} 
and updates $\frar{\tilde{u_i}}{A_i'}{A''}$ such that $u_1;\tilde{u_1} = u_2;\tilde{u_2}=u_1+u_2$. Then we call updates $u_i$ {\em mergable}, \zdmodok{complement updates $\tilde{u_1},\tilde{u_2}$}{update $u_1+u_2$}{}  their {\em merge}, and
updates $\tilde{u_1},\tilde{u_2}$ {\em complements}, and write $(\tilde{u_1},\tilde{u_2})=\merge_A(u_1,u_2)$ or else $\tilde{u_i}=\merge_{A,i}(u_1,u_2)$. We will also denote the model $A''$ by $A'_1+_A A'_2$. For example, for model $A_1$ in Fig.\ref{fig:multimod-uml}, we can concurrently delete John's and add Mary's employments with IBM, or concurrently add two Mary's employments, say, with IBM and Google. But deleting Mary from the model and adding her employment with IBM are not concurrently compatible. Similarly, in $A_3$, updating addresses of different routes, or updating the \from\ and \toattr\ attributes of the same route are concurrently compatible, but deleting a route and changing its attribute are incompatible (we will also say, {\em in conflict}). %Mary's employment with Google. one could add Mary's employment at IBM ($u_1$) and concurrently add Ann ($u_2$) in $A_1$. These changes can be performed in either order, i.e.\ $\tilde{u_1}$ adds Mary's employment after Ann was added, $\tilde{u_2}$ adds Ann after Mary's employment was added yielding the merge update $\frar{u'}{A_1}{A''}$.

%A span of updates $u=(u_1...u_k)$ from a common source $A$ as shown in diagram \eqref{eq:mergeDef} is called {\em concurrently compatible} if they are entirely independent and can be performed in any interleaving order or concurrently leading to the same result--- an update \frar{u''}{A}{A''}. Then we call updates $u_i$ {\em mergable}, update $u''$ their {\em merge}, and write $u''=\merge_0(u)$, while each of the {\em complement} updates \frar{u'_i}{A'_i}{A''} such that $u_i;u'_i=u''$, $i=1..k$, is denoted by $\merge_i(u)$. For example, .......... \zd{to be completed .....}
%\hk{Let's omit the notation $\Span$ and only use \Kdisj{} (we also have no additional notation for all composable update pairs - the superset of $\Kupd$!)}
%\par
%\zd{Indeed!}
%\par

We denote the set of all mergable spans with apex $A$ by $\Kdisj{}_A$
%\subset\Span$ 
%(the black triangle aims to recall that the arity of the relation is a span). %\zd{WARNING: this now does not match notation in the new paper on ppg+} 
%\hk{I inactivated the redundant description of the merge-operation}\zd{ok}
%Thus, \merge\ is an operation that takes a mergable span of updates $u\in\Kdisj{}_A$ \subset\Span_A$ and returns an update \frar{\merge_0(u)}{A}{A''} and a cospan targeted at $A''$ whose feet are $u$'s feet. \zd{{\em it perhaps makes sense to introduce operations Feet  on spans and cospans).}}

%Suppose we have an $n$-ary span of updates as shown in the diagram \eqref{eq:updMerge}. Then we require there is an operation $\merge_n$, which produces an update \frar{u''}{A}{A''} and a cospan \frar{u'_i}{A'_i}{A''}, $i=1..n$ such that $u_i;u'_i=u''$ for all $i$. We write $(u'_1..u'_n)=\merge_n(u_1..u_n)$.

The definition of sequential and concurrent compatibility is a generalization of the notion of sequential and parallel independence of graph transformation rules \cite{gt-EEPT-2006} and below we will elaborate further on the interplay of sequentially and concurrently compatible pairs. Our definitions are, however, abstract enough to cover arbitrary conflict resolution policies (e.g.\ as described in the theory of amalgamated graph transformations \cite{DBLP:journals/jcss/BoehmFH87}) which, to a certain extent, allow merging also in case of conflicting parallel updates. \hk{I hope that this is more clear now??}\zd{hm, understanding of this probably needs having a notion of amalgamated GTs, which is not my case, so, let's ignore my questions}  
\par
Now we define model spaces.
%In addition, we require a model space $\spA$ to be endowed with a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
%$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
%indexed by objects of \spaA, which specify {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update 
%$u$ into $A$ is {\em compatible} with update %\frar{u'}{A}{\_} 
%$u'$ from $A$ and write $(u,u')\in\Kupd_A$ or $u\Kupd_Au'$,  if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$ (see \cite{orejas-bx13} for a detailed discussion). Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for sets of all objects  in $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$. 
%%Now we define model spaces.
%\begin{defin}[Model spaces] \label{def:mspace}
%A {\em model space} is a pair 
%$\spaA=(|\spaA|, \Kupd)$ with $|\spaA|$ being a category (the {\em carrier}) of models and updates, and 
%
%$$\Kupd=\comprfam{\Kupd_A\subset |\spA|(\_,A)\timm|\spaA|(A,\_)}{A\inn\xob{|\spA|}}
%$$ 
%
%\noindent a family of {\em sequential compatibility} relations  for sequential update pairs as described above. We will often omit the bars $|$ and denote a space and its carrier category by the same symbol \spA.
%\end{defin}

\begin{defin}[Model Spaces] \label{def:mspace}
	A {\em model space} is a tuple 
	\[\spaA=(|\spaA|, \Kupd, \Kdisj{}, \merge)\]
	of the following four components. The first one is a category |\spaA| (the {\em carrier}) of {\em models} and {\em updates}. We adopt a notational convention to omit the bars $|$ and denote a space and its carrier category by the same symbol \spA. The second component is a family 
	\[\Kupd=\comprfam{\Kupd_A\subset \spA(\_,A)\timm\spaA(A,\_)}{A\inn\xob{\spA}}\]	
of {\em sequential compatibility} relations  for sequential update pairs as described above. The third and forth component are tightly coupled:
	\[\Kdisj{}=\comprfam{\Kdisj{}_A}{A\inn\xob{\spA}}\]
is a family of {\em concurrently compatible} or {\em mergable} spans of updates, and 
\[\merge =\comprfam{ \merge_A}
	%\frar{\merge^k_A}{\Kdisj{k}_A}{\spA(A,\_)\times\Cospan^k}}
	{A\inn\xob{\spA}}\]
is a family of merge operations as shown in \eqref{eq:mergeDef}. The domain of operation $\merge_A$ is exactly the set $\Kdisj{}_A$. 
We will denote the components of merge by $\merge_{A,i}$ with $i=1,2$ and omit index $A$ if they are clear from the context or not important. Writing $\merge_A(u,v)$ implicitely assumes $(u,v) \in \Kdisj{}_A$. \qed
\end{defin}
%
\begin{defin}[Well-behaved Model Spaces]\label{def:wbspace}
	\noindent A model space is well-behaved (wb) if the following conditions hold for all $A\in\xob{\spaA}$:
\begin{center}
\begin{tabular}{l@{\quad}l}
	\lawnamebr{\Kupd\ and~ Id}{} &	
	For all $u\inn{\spA}(\_,A)$, $u'\inn{\spaA}(A,\_)$: $(u,\id_A), (\id_A,u')\inn\Kupd_A$, 
	\\ [1ex]
		\lawnamebr{\Kdisj{}~and ~\Kupd}{} &
	For all $(u_1,u_2)\in\Kdisj{}_A$: $(u_i,\merge_{A,i}(u_1,u_2))\in\Kupd_{A'_i}$, $i=1..2$
	\\ [1ex]
	\lawnamebr{Merge\ and~ Id}{}& For all $\frar{u}{A}{A'}$: $\merge_A(u,\id_A) = (\id_{A'},u)$    
\end{tabular} 
\end{center} \qed
%A {\em model space functor} from $\spaA$ to $\spaB$ is a functor $F:|\spaA|\to |\spaB|$, such that $(u,u')\hspace{-0.1em}\in \hspace{-0.1em}\Kupd_A$ implies $(F(u),F(u'))\hspace{-0.1em}\in\hspace{-0.1em}\Kupd_B$. We will denote model spaces and their carriers by the same symbol and often omit explicit mentioning of $\Kupd$.\qed  % (cf. Sect.\ref{sec:modelspaces}). 
\end{defin}
Whereas the first condition is the already discussed natural property for sequential compatibility, the second requires complementing updates not to revert anything done by the other update. \footnote{
Note that we do not claim the converse, namely the existence of a concurrently compatible partner in a sequentially compatible pair.} The third requirement is again self-evident.   
%\input{figures/diags/mergeDef}


==> sections/lensesFinal/modelSpaces-currentTexSt.tex <==
\mysubsection{Model spaces and correspondences.}


Basically, a {\em model space} is a directed graph, whose objects are called {\em model states} or just {\em models}, and arrows are {\em (directed) deltas} or  {\em updates}. For an arrow \frar{u}{A}{A'}, we treat $A$ as the state of some model before update $u$, $A'$ as the state after the update, and $u$ as an update specification.  Structurally, it is a specification of correspondences between $A$ and $A'$. Operationally, it is an edit sequence (edit log) that changed $A$ to $A'$. There are also special {\em idle} loop updates  \frar{\id_A}{A}{A} that do nothing. The formalism does not prescribe what updates are, but assumes that  
(a) normally there may be different updates from state $A$ to state $A'$, (b) updates are composable, and (c) idle updates are the units of the composition. These three conditions mean that we require a model space to be a category (see Sect. A.1)
\begin{mydefin}[Model Space] A {\em model space} is a category whose objects are called {\em models} and arrows are {\em deltas} or {\em updates}. %Objects of a model space \spaA\ will be denoted by \xob{\spaA} and 
	We will write $\xupd{\spaA}(A,A')$ for the set of  arrows from $A$ to $A'$  to recall that they are deltas/updates. 
\end{mydefin}
In the sequel, we will work with families of model spaces indexed by a finite set $I$, whose elements can be seen as space {\em names}. To simplify notation, we will assume that $I=\{1,..,n\}$ although ordering will not play any role in our \fwk. \zdmodok{ It is, however, no loss of generality, if we assume the spaces to be numbered, i.e.\ we can work with the cartesian product $\spA_1\times \cdots \times \spA_n$, if $I$ contains $n$ elements for some arity $n\ge 2$.}{}{} 
Given a tuple of model spaces $\spaA_1...\spaA_n$, we will refer to objects and arrows of the product category $\spaA_1\timm...\timm\spaA_n$ (see Appendix)  as {\em model} and {\em update tuples}
; sometimes,  as {\em discrete multimodels  {\em and} multiupdates}.  
%\begin{mydefin}[Model and Update Tuples]\label{def:modelTupleUpdTuple}
%A family $(A_1, \ldots, A_n) \in \xob{\spA_1}\times \cdots \times \xob{\spA_n}$ is called a {\em model tuple} (or sometimes a {\em discrete} multimodel). Given two tuples $(A_1, \ldots, A_n)$ and $(A_1', \ldots, A_n')$ and updates \frar{u_i}{A_i}{A_i'} of $\xupd{\spaA_i}$, resp., $(u_1, \ldots, u_n)$ is called an {\em update tuple}\footnote{
%By the definition of cartesian product of categories, the collection of all update tuple is the same as $\xupd{\spaA_1\times \cdots\times \spaA_n}$.
%}.\qed
%\end{mydefin}
%
%{\color{blue}Next para may be moved}\\ 
%Assume $n=2$ for the moment, \ie, there are two model spaces \spaA\ and \spaB. E.g., \spaA\ may encompass all possible object structures that conform to a fixed class diagram and \spaB\ contains all object structures that conform to a second fixed class diagram. A different example is, if \spaA\ is a set of UML class diagrams and \spaB\ is a set of relational schemas. A pair $(A,B)$ of interrelated models normally comes with a traceability mapping so that our typical situation to consider is a triple $(A,R,B)$ with $A$ a model from \spaA, $B$ a model from \spaB, and $R$ some specification of correspondences between them. There may be many different correspondences between the same $A$ and $B$, but not all of them satisfy some a priori given notion of consistency. Hence, in order to describe exactly legal triples $(A,R,B)$ one has to specify the admissible set $\R$ of consistent correspondence specification together with the respective model pairs that they coordinate, \ie one must specify two mappings $\partial_\spaA:\R\to \xob{\spaA}$ and $\partial_\spaB:\R\to \xob{\spaB}$.
%
%We can now provide the corresponding generalization for arbitrary $n$:
\begin{mydefin}[Multispace and Multimodels]\label{def:multispace}
A {\em multimodel space} or just a {\em multispace} \mspaA\ is given by (a) a  finite family of model spaces $\partial\mspaA=(\spaA_1, \ldots, \spaA_n)$ called the {\em boundary} of \mspaA, and (b) a family of disjoint sets $\R(A_1...A_n)$ indexed by model tuples over $\partial\mspA$. Elements of set $\R(A_1...A_n)$ are called {\em (consistent) corrs} and understood as consistent correspondence specifications interrelating models $A_i$. 
Spaces $\spaA_i$ are called {\em feet} of \mspaA\ and denoted by $\partial_i(\mspaA)$.

%Given a corr $\acorr\in \R(A_1...A_n)$, we refer to model $A_i$ as the $i$'s {\em boundary} of \acorr\ and write $A_i=\partial_i(\acorr)$ and $\partial\R$ for the tuple $A_i$, $i\inn I$. Thus $\partial\acorr=A$ iff $\acorr\in\R(A)$.  An {\em (aligned consistent) multimodel} over a multispace \mspaA\ is a pair $\nia=(\famA, \acorr)$ with $\famA\in\xob{\spaA}$ a model tuple over \mspaA, and $\acorr\in \K(\fmaA)$ some (consistent) corr between the members of \famA. We then write $\nia\in\xstar{\mspaA}$.  \shortlong{(Thus, in this paper we do not consider inconsistent multimodels.)}{We call \nia\ {\em consistent} if the corr is consistent, $r\in\Kcorr(\famA)$.}
%

An {\em (aligned consistent) multimodel} over a multispace \mspaA\ is a pair $(\bar{A},R)$ with $\bar{A}=(A_1, \ldots, A_n)$ a model tuple over $\partial\mspA$, and $R\in \R(\bar{A})$ a corr relating $\bar{A}$-members. We write $\partial_i(R)$ for $A_i$ and call them {\em feet} of $R$; the entire tuple $\bar{A}$ is the {\em boundary} $\partial R$ of $R$.  The class of all multimodels over \mspaA\ is denoted by \xstar{\mspA} (note the difference with $\xob{\mspaA}\eqdef \xob{\spaA_1}\timm...\timm\xob{\spaA_n}$ denoting the class of discrete/non-aligned multimodels). 
%$A_i\in \xob{\spaA_i}$ and $\partial_i(R) = A_i$ for all $i$. 
A {\em multimodel update} \frar{u}{(A_1, \ldots, A_n, R)}{(A_1', \ldots, A_n', R')} is an update tuple (\frar{u_1}{A_1}{A'_1}, \ldots, \frar{u_n}{A_n}{A'_n}). %(Note that we require the source and the target of the update to be aligned rather than discrete multimodels.)      
%\end{enumerate}
%Note that each corr $R\in\R$ comes equipped with boundary mappings (by \ref{enum2} and \ref{enum3}). Accordingly, models $\partial_i(R)$ are called the {\em boundary} of $R$. Thus $R$ is actually an  $n$-ary ``star''-link connecting models $A_1\eqdef\partial_1(R), \ldots, A_n\eqdef\partial_n(R)$. See Fig.\ \ref{fig:alignedMultimod}, where the corresponding spaces are depicted. It is deliberate that this {\em completely} determines a multimodel as defined in \ref{enum4}, because we want to emphasize the fact that, in this paper, we do not consider inconsistent multimodels.\qed
%\shortlong{}
{These data make a multispace \mspaA\ a category different from $\spaA_1\timm...\timm\spaA_n$.} \qed
\end{mydefin}
%
%To assign to a model tuple $(A_1, \ldots, A_n)$ its admissible correspondence specifications, we introduce the following notation: 
%\[\R(A_1, \ldots, A_n)\eqdef \{R\in\R \mid \forall i: \partial_i(R) = A_i\}\]
%Finally, it is important to 
We will also need to identify the set of all corrs  for some  fixed $A_i\in \xob{\spaA_i}$ (for a given $i$). We define 
$\R(A_i,\_)=\compr{R\in\R(\bar{A})}{\bar{A}_i=A_i}$.


\zdmod{$\R_i(A_i, \_)\eqdef \{(\partial_1(R), \ldots, \partial_n(R)) \mid R\in \R, \partial_i(R) = A_i\}$}{???}{is it what we need?}


% \mbox{ and } \partial_i(R)=A_i}$


%\begin{example}
%Running
%\end{example}




==> sections/lensesFinal/modelSpaces.tex <==

%\endinput 
\subsection{Model Spaces and Correspondences}\label{sec:modelspaces}
Basically, a {\em model space} is a category, whose nodes are called {\em model states} or just {\em models}, and arrows are {\em (directed) deltas} or {\em updates}. For an arrow \frar{u}{A}{A'}, we treat $A$ as the state of the model before update $u$, $A'$ as the state after the update, and $u$ as an update specification.  Structurally, it is a specification of correspondences between $A$ and $A'$. Operationally, it is an edit sequence (edit log) that changed $A$ to $A'$. The formalism does not prescribe what updates are, but assumes that they form a category, \ie, there may be different updates from state $A$ to state $A'$; updates are composable; and idle updates \frar{\id_A}{A}{A} (doing nothing) are the units of the composition. 
	
In addition, we require every model space $\spaA$ to be endowed with a family $(\Kupd_A)_{A\inn\xob{\spaA}}$ of binary relations %$\comprfam{\Kupd_{A}\subset\spaA(\_,A)\timm\spaA(A,\_)}{A\in\xob{\spaA}}$,
	$\Kupd_{A}\subset\xarr{\spaA}(\_,A)\timm\xarr{\spaA}(A,\_) $
	indexed by objects of \spaA, and 
	specifying {\em non-conflicting} or {\em compatible} consecutive updates. Intuitively, an update %\frar{u}{\_}{A} 
	$u$ into $A$ is compatible with update %\frar{u'}{A}{\_} 
	$u'$ from $A$, if $u'$ does not revert/undo anything done by $u$, \eg, it does not delete/create objects created/deleted by $u$, or re-modify attributes modified by $u$ (see \cite{orejas-bx13} for a detailed discussion). Formally, we only require $(u,\id_A)\inn\Kupd_A$ and  $(\id_A,u')\inn\Kupd_A$ for all $A\in\xob{\spaA}$, $u\inn\xarr{\spaA}(\_,A)$ and $u'\inn\xarr{\spaA}(A,\_)$.  
	\begin{definition}[Model spaces] A {\em model space} is a pair $\spaA=(|\spaA|,\Kupd_A)$ with $|\spaA|$ a category (the {\em carrier}) of models and updates and $\Kupd_A$ a family as specified above. A {\em model space functor} from $\spaA$ to $\spaB$ is a functor $F:|\spaA|\to |\spaB|$, such that $(u,u')\hspace{-0.1em}\in \hspace{-0.1em}\Kupd_A$ implies $(F(u),F(u'))\hspace{-0.1em}\in\hspace{-0.1em}\Kupd_B$. We will denote model spaces and their carriers by the same symbol and often omit explicit mentioning of $\Kupd$.\qed  % (cf. Sect.\ref{sec:modelspaces}). 
	\end{definition}
%\begin{defin}[Model Space] A {\em model space} is a category whose objects are called {\em models} and arrows are {\em deltas} or {\em updates}. We will write $\xupd{\spaA}(A,A')$ for the set of  arrows from $A$ to $A'$  to recall that they are deltas/updates. 
%\end{defin}
In the sequel, we will work with families of model spaces indexed by a finite set $I$, whose elements can be seen as space {\em names}. To simplify notation, we will assume that $I=\{1,\ldots,n\}$ although ordering will not play any role in our \fwk. Given a tuple of model spaces $\spaA_1, \ldots, \spaA_n$, we will refer to objects and arrows of the product category $\prod\spA=\spaA_1\timm\cdots\timm\spaA_n$ as {\em model tuples} and {\em update tuples} or, sometimes, as {\em discrete multimodels  / multiupdates}.  

%\input{sections/lensesFinal/multispace-old}
\input{sections/lensesFinal/multispace-total} 


==> sections/lensesFinal/multiLenses-new-withTraj.tex <==
\section{%Multidirectional Update Propagation and Delta Lenses
Multimodel spaces
}
\label{sec:mmod}
%\label{sect:multiaryDeltaLenses}
 

A delta-based mathematical model for bx  is well-known under the name of delta lenses; below we will say just {\em lens}. There are two main variants: asymmetric lenses, when one model is a view of the other and hence does not have any private information, and symmetric lenses, when both sides have their private data not visible on the other side \cite{me-jot11,me-models11,bpierce-popl11}. In the next sections we will develop a \fwk\ for generalizing the idea for any $n\ge 2$ and including reflective updates. %: we present basic definitions and several easy results. %, but the very equivalence result is left for future work. 

\subsection{Background: Graphs, (co)Spans, and Categories}
\input{sections/app/graphs-cats-total}

%%\input{sections/lensesFinal/modSpaces-big}
%\input{sections/lensesFinal/modSpaces}
%\input{sections/lensesFinal/multimodSpaces}
%\input{sections/lensesFinal/multiPpg}
%\input{sections/lensesFinal/lego}
%%\input{sections/lensesFinal/asym2sym}
%=== a major update: models are lax trajectories
\input{sections/lensesFinal/modSpaces-new}
%\clearpage
%\input{sections/lensesFinal/multimodSpaces-new} actually old
\clearpage
\input{sections/lensesFinal/multimodSpaces-last}
%\input{sections/lensesFinal/multimodSpaces-Newest} % outdated
%\input{sections/lensesFinal/multiPpg}
\input{sections/lensesFinal/multiPpg-last}
%\clearpage
%\zd{the old version}
%\input{sections/lensesFinal/lego-new} % actually old
\clearpage
\zd{the last version} 
\input{sections/lensesFinal/lego-last}






==> sections/lensesFinal/multiLenses-new.tex <==
\section{%Multidirectional Update Propagation and Delta Lenses
Multimodel spaces
}
\label{sec:mmod}
%\label{sect:multiaryDeltaLenses}
 

A delta-based mathematical model for bx  is well-known under the name of delta lenses; below we will say just {\em lens}. There are two main variants: asymmetric lenses, when one model is a view of the other and hence does not have any private information, and symmetric lenses, when both sides have their private data not visible on the other side \cite{me-jot11,me-models11,bpierce-popl11}. In the next sections we will develop a \fwk\ for generalizing the idea for any $n\ge 2$ and including reflective updates. %: we present basic definitions and several easy results. %, but the very equivalence result is left for future work. 

\subsection{Background: Graphs, (co)Spans, and Categories}
\input{sections/app/graphs-cats-total}

%%\input{sections/lensesFinal/modSpaces-big}
%\input{sections/lensesFinal/modSpaces}
%\input{sections/lensesFinal/multimodSpaces}
%\input{sections/lensesFinal/multiPpg}
%\input{sections/lensesFinal/lego}
%%\input{sections/lensesFinal/asym2sym}

%=== a major update: models are lax trajectories
\input{sections/lensesFinal/modSpaces-new}
%\input{sections/lensesFinal/modSpaces-last}

%\input{sections/lensesFinal/multimodSpaces-new} actually old
\input{sections/lensesFinal/multimodSpaces-last}
%\input{sections/lensesFinal/multimodSpaces-Newest} % outdated

%\input{sections/lensesFinal/multiPpg-new} %actually old?
\input{sections/lensesFinal/multiPpg-last}
%\input{sections/lensesFinal/lego-new} % actually old
\input{sections/lensesFinal/lego-last}






==> sections/lensesFinal/multiLenses.tex <==
\section{%Multidirectional Update Propagation and Delta Lenses
Multimodel spaces
}
\label{sec:mmod}
%\label{sect:multiaryDeltaLenses}
 

A delta-based mathematical model for bx  is well-known under the name of delta lenses; below we will say just {\em lens}. There are two main variants: asymmetric lenses, when one model is a view of the other and hence does not have any private information, and symmetric lenses, when both sides have their private data not visible on the other side \cite{me-jot11,me-models11,bpierce-popl11}. In the next sections we will develop a \fwk\ for generalizing the idea for any $n\ge 2$ and including reflective updates. %: we present basic definitions and several easy results. %, but the very equivalence result is left for future work. 
\subsection{Background: Graphs, (co)Spans, and Categories}
\input{sections/app/graphs-cats-total}

%\input{sections/lensesFinal/modSpaces-big}
%\newpage
\input{sections/lensesFinal/modSpaces}
\input{sections/lensesFinal/multimodSpaces-Newest}
\input{sections/lensesFinal/multiPpg}
\input{sections/lensesFinal/lego}
%\input{sections/lensesFinal/asym2sym}







==> sections/lensesFinal/multiPpg-new.tex <==
\section{Update Propagation and Multiary (Delta) Lenses}
%\subsection{Update Propagation and Multiary (Delta) Lenses}

Update policies described in \sectref{sec:example} can be extended to cover propagation of all updates $u_i$, $i\in 1...3$ according to the pattern  in \figref{fig:ppgPatterns-reflect}. \zdneww{This is a non-trivial task, but after it is accomplished, we obtain a \syncon\ \fwk, which we algebraically model as an algebraic structure called a {\em well-behaved lens}. In this term,  {\em lens} refers to a collection of diagram operations defined over a multispace of models, which take a configuration of models, corrs and updates and {\em propagate} them, \ie, return another configuration of models, corrs and updates. A lens is called {\em well-behaved}, if propagation operations satisfy a set of algebraic laws specified by equations. This terminological discipline goes back to the first papers, in which lenses were introduced \cite{bpierce-popl05}. We define and discuss well-behaved lenses in the next \sectref{sec:wblens}. In \sectref{sec:vwblens}, we discuss an important special property of lenses: compatibility of update propagation with update composition, which is regulated by the most controversial amongst the lens laws -- the (in) famous PutPut law.}{}{-2em} 

\subsection{Well-behaved lenses}\label{sec:wblens}	

\begin{defin}[Symmetric lenses]\label{def:multi-lenses}
	An $n$-ary {\em symmetric lens} is a pair $\ell=(\mspaA, \ppg)$ with \mspaA\ an $n$-ary multispace called the {\em carrier} of $\ell$, and  $(\ppg_i)_{i\le n}$ an $n$-tuple of operations of the following arities. Operation $\ppg_i$ takes a consistent corr $R$ with boundary $\prt R=\tupleA$,
	and a foot update \frar{u_i}{A_i}{A'_i} as its input, and returns 
	
	%\noindent 
	(a) an $(n-1)$-tuple of updates \frar{u'_j}{A_j}{A''_j} with $1\le j\not= i\le n$; 
	
	%\noindent 
	(b) a {\em reflective} update \frar{u'_i}{A'_i}{A''_i} also called an {\em amendment} of $u_i$, 
	
	%\noindent 
	(c) a new consistent corr $\acorr''\in \tupleAii^\bigstar$. 
	
	\noindent In fact, operation $\ppg_i$ completes a (local) foot update $u_i$ to a (global) tuple update of the entire multimodel, whose  components are $(u_j')_{j\ne i}$ and $u_i;u'_i$ (see \figref{fig:ppgPatterns-reflect}). 
	\qed
\end{defin}
Note that all \ppg\ operations are only defined for consistent corrs and return consistent corrs.
%\begin{mydefin}[Symmetric Lens]
%	A {\em symmetric lens} is a pair $\ell=(\mspaA, \ppg)$ with \mspaA\ a multispace (called the carrier of $\ell$) with model spaces $\spaA_1, \ldots, \spaA_n$, corr set $\R$, and $\ppg = (\ppg_1, \ldots, \ppg_n)$ an $n$-tuple of operations with 
%\[
%\ppg_i: \left\{
%\begin{array}{rcl}
%\xupd{\spaA_i} \times_i \R & \to & \xupd{\spaA_1\times \cdots \times \spaA_n}\times \R \\
%(u_i, R) &\mapsto & (u_1', \ldots, u_n', R'')\\
%\end{array}\right.
%\]	
%for all $i$. $n$ is called the {\em arity} of $\ell$ or, equivalently, $\ell$ is an $n$-ary lens.

%\input{figures/pdfs/alignedMultimodel.tex}
%The notation $\xupd{\spaA_i} \times_i \R$ depicts those pairs $(u_i: A_i\to A_i', R)$ for which $\partial_i(R) = A_i$, or, equivalently, $R\in \R_i(A_i,\_)$, i.e.\ (in the same way as in the binary example) $\ppg_i$ takes as input $R\in \R_i(A_i,\_)$ and an update of $A_i$. For $j\ne i$ it returns (a) updates \frar{u'_j}{A_j}{A''_j} and (b) a {\em reflective} update \frar{u'_i}{A'_i}{A''_i} (also called an {\em amendment} of $u_i$), and (c) a new consistent corr $R''\in \R(A_1'', \ldots, A_n'')$. In fact, operation $\ppg_i$ completes update $u_i$ to a multiupdate 
%
%\[(u_1', \ldots, u_{i-1}', (u_i;u_i'), u_{i+1}', \ldots, u_n')\]
%
%(see \figref{fig:ppgPatterns-reflect})
%\end{mydefin}
%We will employ the following notational conventions. 
{\bf Notation.} If the first argument \acorr\ of operation \ppg$_i$ is fixed, the corresponding family of unary operations (whose only argument is $u_i$) will be denoted by $\ppgr_i$. By taking the $j$th component of the multi-element result, we obtain single-valued unary operations $\ppgr_{ij}$ producing, resp. updates $\frar{u'_j=\ppgr_{ij}(u_i)}{A'_j}{A''_j}$, where $A'_j=A_j$ for all $j\not=i$ (see clause (a) of the definition) while $\ppgr_{ii}$ is the reflective update (b). We also have operation $\ppgr_{i\star}$ returning a new consistent corr $R''=\ppgr_{i\star}(u_i)$ according to (c).
\begin{defin}[Closed updates]
	Given a lens $\ell=(\mspaA,\ppg)$ and a corr $R\in \tupleA^\bigstar$, we call an update \frar{u_i}{A_i}{A'_i} $R$-{\em closed}, if $\ppgr_{ii}(u_i)=\id_{A_i'}$. An update is $\ell$-{\em closed} if it is $R$-closed for all $R$. Lens $\ell$ is called {\em non-reflective} at foot $\spaA_i$, if all updates in $\spA_i$ \ %\xupd{\spA_i} 
	are $\ell$-closed. \qed
\end{defin} 
\zd{Below is an important piece which is not easy to write b/c we don't have really strong arguments. It needs completion.}
\\
\hk{I'm not sure whether you want it to be placed here or better in the introduction. Please decide!}
\par
\zdneww{Update propagation policies discussed in Sect.2 give rise to a 3-ary lens. 
\\
	....
\\
	Consistency restoration is not unique, there are different policies. ....Based on heuristics etc ...
\\
We will not actually define the lens -- it can be done along the lines of how binary symmetric lens are defined with, \eg, triple graph grammars \cite{?}. Our goal in the paper is to describe general laws, and show their consistency with simple mathematical examples described below. 
For the \exIntro, update propagation policies described in \sectref{sec:example} give rise to a lens non-reflective at space $\spA_3$.}{important piece which is not easy to write}{-8em}

\begin{defin}[Well-behaved lenses]\label{def:wblens}
	A lens $\ell=(\mspaA,\ppg)$ is called {\em well-behaved (wb)} if the following laws hold for all $i\le n$, $A_i\in\xob{\spaA_i}$, 
	$R\in \Kcorr _{A_i}\subset A_i^\bigstar$ and \frar{u_i}{A_i}{A'_i}, cf. \figref{fig:ppgPatterns-reflect}
	
	\lawgap=1ex
	%\newcommand\lawind{\ensuremath{$_i$}}

	\smallskip\noindent
	\begin{tabular}{l@{\quad}l}
% = stability law
		\lawnamebr{Stability}{i}&
		$\forall j\in\{1...n\}: \ppgr_{ij}(\id_{A_i})=\id_{A_j}$\mbox{ and } $\ppg^R_{i\star}(id_{A_i}) = R$
%		\\  [\lawgap] &
%		 \lawnamebr{Hippocr}{i} &
%		 Let $A_j=\prt_jR$ for $j\le n$ (and hence $\prt_iR=A_i$).
%		 %\noteq i$, $\ovr{u_i}=(\id_{A_1}...u_i...\id_{A_n})$ and $A'=(A_1...A'_i...A_n)$. 
%		 \\ [0.5ex] &
%		  	If  $R'=u_i^\bigstar(R) \in \Kcorr_{A_i'}$, \ie, realignment returns a consistent corr, 
%		\\ & 
%		then $\ppgr_{ij}(u_i)=\id_{A'_j}$ for all $j\le n$, and $\ppgr_{i\star}(u_i)=R'$.
		\\[\lawgap]
		 \lawnamebr{Reflect1}{i} &	
		$(u_i, \ppgr_{ii}(u_i))\in \Kupd_{A_i'}$ %for all $u_i$ 
		\\[\lawgap]
		\lawnamebr{Reflect2}{i} &
		$\ppgr_{ij}(u_i;\ppgr_{ii}(u_i)) = \ppgr_{ij} (u_i)$ for all $j\noteq i$
		\\  [\lawgap]  
		\lawnamebr{Reflect3}{i} &
			$\ppgr_{ii}(u_i;\ppgr_{ii}(u_i))=\id_{A''_i}$ 
			where $A''_i$ is the target model of $\ppgr_{ii}$.
			% $u_i' =  \ppgr_{ii}(u_i)$ as in Def.~\ref{def:multi-lenses} 
		%	\\  [\lawgap] \lawnamebr{PutPut}$\forall w_i\inn\Kupd_{A''}(u''_i,\_),$ 
		%	& \pputi
		%	\\	[-0.1\lawgap] $\hphantom{\lawnamebr{PutPu}}$
		%	$\forall  j\noteq i$ 
		%	&  \pputii
		%	%	$\ppgr_{ij}(u''_i~; w_i)=\ppgr_{ij}(u''_i) ; \ppg^{\acorr''}_{ij}(w_i)$,  
		%	%	\\ [0.5\lawgap] & 
		%	%	 and $(\ppgr_{ij}(u''_i),~\ppg^{\acorr''}_{ij}(w_i))\in \Kupd_{A''_j}$
	\end{tabular}\\
\end{defin}
\zdmodd{\lawname{Hippocr} law says that if realignment returns a consistent corr, nothing should be done.}{\lawname{Stability} says that lenses do nothing voluntarily}{HIPPO}{-1em}
 \lawname{Reflect1} says that amendment works towards ``completion'' rather than ``undoing'', and  \lawname{Reflect2-3} are idempotency conditions to ensure the completion indeed done. 

\zd{Hippocr implies Stability is commented}
%Because alignment $\mspA^\bigstar$ is a functor, it preserves identities. This together with \lawname{Hippocr} implies \lawname{Stability}, which says that lenses do nothing voluntarily:
%\begin{corollary}[{\sf Stability}]\label{cor:1} 
%%\smallskip\noindent
%%		\begin{tabular}{l@{\qquad}l}
%%				&
%			{\em	If $\ell$ is wb, then for all consistent corrs $R$ and all $i,j\le n$: $\ppgr_{ij}(\id_{A_i})=\id_{A_j}$\mbox{ and } $\ppg^R_{i\star}(\id_{A_i}) = R$}
%%				\\  [1ex]
%%	\end{tabular} 
%\qed
%\end{corollary}
%The last law (called \lawname{PutPut} by the same traditional lens style) says that propagation of compatible updates preserves the composition and thus ignores the intermediate history of the updating path if updates do not conflict.
\begin{defin}[{\sf Invertibility}] \label{def:invert}
	A wb lens is called {\em (weakly) invertible}, if it satisfies the following law for any $i$, update \frar{u_i}{A_i}{A'_i} and $R\in A_i^\bigstar$:
	
	\noindent \begin{tabular}{l@{\quad}l}
		\lawnamebr{Invert}{i}%$_{j\noteq i}$
		& for all $j\noteq i$: 
		$\ppgr_{ij}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ij}(u_i)$	
	\end{tabular}
	\qed 	
\end{defin}
This law deals with ''round-tripping'': operation $\ppgr_{ji}$ applied to 
update $u_j=\ppgr_{ij}(u_i)$ results in update $\hat{u_i}$ equivalent to $u_i$ in the sense that $\ppgr_{ij}(\hat{u_i})=\ppgr_{ij}(u_i)$  (see \cite{me-models11} for a motivating discussion). %it was made apparent that it is a good compromise between proper prevention of unwanted effects on the one hand and leaving enough freedom for the framework on the other hand.
\zdmodno{}{Hmm, \\
	\noindent \begin{tabular}{l@{\quad}l}
		\lawnamebr{Invert{-}strong}{i}%$_{j\noteq i}$
		& for all $j\noteq i$ and all $k$: 
		$\ppgr_{ik}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ik}(u_i)$	
	\end{tabular}
}{I just recognized that the much stronger version on the left would perhaps be more reasonable: to think about }
%<<<<<<< HEAD
%\exIntro\ A natural update propagation policy in the example of Sect.\ref{sec:example} is the following: If a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case, already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id_{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%=======
%\exIntro\ A reasonable update propagation policy would be is if a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%>>>>>>> edits thru the whole paper
%The next two (simple) examples will be used in the forthcoming theorems. 	 
\begin{example}[Trivial lenses \trivlensna]\label{ex:TerminalLens} 
	%\subsection{Terminal categories and lenses.} 
	A category consisting of one object and one (necessary identity) arrow is called {\em terminal}. All terminal categories are isomorphic; we fix one, whose object is denoted by $1$ while the category is denoted by \trmcat\ (bold 1). The terminal category \trmcat\ gives rise to a unique {\em terminal space} with  $\Kupd_1 = \{(id_1,id_1)\}$.
	%\begin{example}[Terminal lens \trmlens]
	
	Any model space \spA\ gives rise to the following {\em trivial} $n$-ary lens \trivlensna. The first foot space $\spA_1=\spA$ while for all $j=2..n$, $\spA_j=\trmcat$.   %\footnote{
	Tuple models are uniquely determined by their first foot, and given such a model $(A,1...1)$, the set of corrs is the singleton $\{\etosing{A}\}$ with $\prt_1\etosing{A}=A$ and $\prt_{2..n}\etosing{A}=1$, and this only corr is considered consistent. Hence, all mutlimodels are consistent and update propagation is not actually needed. For any \spA, lens $\trivl_n(\spA)$ is a wb, invertible lens non-reflective at all its feet in a entirely trivial way.\qed  
\end{example}
%\zd{still I decided to distinguish an element $x$ and a corr made from that element as \etosing{x}. The latex macros is} \verb|\etosing| \zd{(read "element to a singleton") in the file macros/thisPaper. This will be used many times below}

The next example is more interesting.
\begin{example}[Identity Lenses \idlensna]\label{ex:idLens} 
	Let $\spaA$ be an arbitrary model space. It generates an $n$-ary lens \idlensna\ as follows. The carrier $\mspaA$ has $n$ identical feet spaces: $\prtbf_i\mspaA=\spaA$ for all $i=1..n$. The corr set for a tuple model $ A\!\!A=(A_1..A_n)$, \ie, set $A\!\!A^\bigstar$, is the singleton $\{\etosing{A\!\!A }\}$ with $\prt_i\etosing{A\!\!A}=A_i$, and this corr is consistent iff all $A_i=A$ for some model $A\in\xob{\spA}$.  All updates are propagated to themselves (hence the name of \idlensna). Obviously, \idlensna\ is a wb, invertible lens non-reflective at all its feet. \qed 
\end{example}

\subsection{Very well-behaved lenses}\label{sec:vwblens}	


We consider an important property of update propagation---its compatibility with update composition. A simple compositionality law would require that the composition $u_i;v_i$ of two consecutive foot updates \frar{u_i}{A_i}{A'_i}, \frar{v_i}{A'_i}{B_i}, is propagated into the composition of propagations: 
$\ppgr_{ij}(u_i;v_i)=\ppgr_{ij}(u_i);\ppgrx{R''}_{ij}(v_i)$ with $R''$ being the corr provided by the first propagation, $R''=\ppgr_{i\star}(u_i)$. It is however well known that such a simple law (called PutPut) often does not hold. 

\input{figures/pdfs/ex-putput1.tex}
Figure~\ref{fig:ex-putput1} presents a simple example (we use a more compact notations, in which \name-attributes are placed at the OID boxes).  At the initial moment, the binary multimodel $(\ai, \aii)$ with the (implicit) corr given by name matching is consistent: the only intermodel constraint (C1) is satisfied. Update $u_1$ adds a new employment record to model \ai, constraint (C1) is violated, and to restore consistency, a new employment is added to \aii\ by update $u_2=\ppgr_{12}(u_1)$ (the new propagated model and update are shown with blue lines and blank).  Then  update $v_1$ deletes the record added by $u_1$, but as the resulting multimodel $(A''_1, A'_2)$  remains consistent, nothing should be done (the law of (Stability)) and thus $v_1$ is propagated to identity, $v_2=\ppgrx{R''}_{12}(v_1) =\id_{A'_2}$. Now we notice that the composition $(u_1;v_1)$ is identity and hence to be propagated to identity, \ie, $\ppgr_{12}(u_1;v_1) = \id_{A_2}$, while $\ppgr_{12}(u_1);\ppgrx{R''}_{12}(v_1) =u_2;v_2=u_2 \noteq \id_{A_2}$, and $A''_1\noteq A''_2$.  Obviously, the violation story will still hold if models \ai\ and \aii\ are much bigger and updates $u_1$ and $v_1$ are parts of bigger updates (but Mary should not appear in \ai).  

\input{figures/pdfs/ex-putput2.tex}
Figure~\ref{fig:ex-putput2} presents a more interesting ternary example. Multi-model $\nia$ is consistent, but update $u_3$ deletes route \#1 and violates constraint (C2). In this case, the most direct propagation policy would delete all employment records related to \#1\ but, to keep changes minimal, would keep people in $A_1$ and companies in $A_2$ as specified by model $\nia'$ in the figure. Then a new route is inserted by update $v_3$  (note the new OID), which has the same \from\ and \toattr\ attributes as route \#1. There are multiple ways to propagate such an insertion. The simplest is to do nothing as the multimodel $(A'_1.A'_2,A''_3, R'=\varnothing)$ is consistent (recall that mapping \etor\ is not necessarily surjective).  However, we can assume a more intelligent policy that looks for people with address a1 in the first database (and finds John and Mary), then checks somehow (\eg, by other attributes in the database schema $M_1$ which we did not show) if some of them are recent graduates in IT (and, for example, finds that Mary is such) and thus could work for a company at the address a10 (Google). Then such a policy would propagate update $v_3$ to $v_1$ and $v_2$ as shown in the figure. The composition of updates $u_3$ and $v_3$  is, in fact, an identity as object identifiers are normally invisible, and thus $u_3;v_3$ would be propagated to the identity on the multimodel \nia. However, $\nia''\noteq\nia$ and Putput again fails.

Note that a common feature of the two examples is that the second update $v$ fully reverts the effect of the first one, $u$, while their propagations do not fully enjoy such a property due to some ``side effects''. In fact, Putput is violated if update $v$ would just partially revert update $u$. Several other examples and a more general discussion of this phenomenon that forces Putput to fail can be found in \cite{me-bx17}. However, it makes sense to require compositional update propagation for two {\em sequentially compatible} updates in the sense of \defref{def:mspace}; we call the respective version of the law \kputput\ with 'k' recalling the sequential compatibility relation \Kupd. To manage update amendments, we will also need to use update merging operator \merge\ as shown in \figref{fig:putput}  


\begin{defin}[Very well-behaved lenses] \label{def:putput}
	A wb lens is called {\em very well behaved (vwb)}, if it satisfies the following \kputputlaw\ for any $i$, corr $R\in A_i^\bigstar$, and updates \frar{u_i}{A_i}{A'_i}, \frar{v_i}{A'_i}{B_i} (see \figref{fig:putput}).
	
	Let $u'_i:=\ppgr_{ii}(u_i)$. If $(u_i,v_i)\in\Kupd_{A_i'}$  and  $(v_i,u'_i)\in\Kdisj{}_{A_i'}$, 
	then $(\tilde v_i, \tilde u'_i):=\merge(v_i, u'_i)$ is defined (see \figref{fig:putput}) and the following equalities hold:
	
	\smallskip
	\noindent \begin{tabular}{l@{\quad}ll}
		\multirow{2}{*}{\lawnamebr{\kputput}{j\noteq i}}  & % row 1
			$\ppgr_{ij}(u_i;v_i)=
		\ppgr_{ij}(u_i);\ppg^{R''}_{ij}(\widetilde{u'_i})$, 
		\\ [0.5ex]	& % row 2
		and $(\ppgr_{ij}(u_i),\ppg^{R''}_{ij}(\widetilde{u'_i}))\in \Kupd_{A_j''}$,
				\\ [0.5ex] 
			\lawnamebr{\kputput}{ii}	&
		and $\ppgr_{ii}(u_i;v_i) = \widetilde{v_i};\ppg^{R''}_{ii}(\widetilde{u_i'})$,
	\end{tabular}\\
see the dashed arrows in \figref{fig:putput}, which depict the propagation of the composed updates. \qed 	
\end{defin}
\input{figures/diags/putput.tex}


\endinput

Update policies described in \sectref{sec:example} can be extended to cover propagation of all updates $u_i$, $i\in 1...3$ according to the pattern  in \figref{fig:ppgPatterns-reflect}. This is a non-trivial task, but after it is accomplished, we have the following \syncon\ structure. 

\noindent 
\begin{minipage}[t]{0.675\textwidth}
\begin{defin}[Symmetric lenses]\label{def:mlens}
	An $n$-ary {\em symmetric lens} is a pair $\ell=(\mspaA, \ppg)$ with \mspaA\ an $n$-ary multispace called the {\em carrier} of $\ell$, and  \ppg\ the following {\em propagation} operation. It takes a corr $R$ (in fact, a multimodel) with boundary $\prt R=\tupA=\tupleA$,
	and an update \frar{\tupu}{\tupA}{\tupA'} as its input, and returns  a multimodel with corr $R''$ and boundary $\tupA''=\prt R''$ produced by an amendment update \frar{u'}{\tupA'}{\tupA''} as shown in the diagram on the right, in which$\tupu''=\tupu;\tupu'$ (recall that given elements are framed and solid, derived ones are non-framed and dashed). \qed
\end{defin}
\end{minipage}\qquad
\begin{minipage}[t]{0.245\textwidth}
	%\vspace{-2ex}
	\input{figures/diags/lensDef}
\end{minipage}

Note that the tuple model $\tupA'$ is not necessary the boundary of some (consistent) corr $R'$. If it is, then amendment $\tupu$ would be an identity,  $R''=R'$, and $\tupu''=\tupu$.    

\begin{defin}[Notation.]
As operation \ppg\ produces several component, it actually gives rise to several operations \corring\ to the parts of the output: we write
\begin{equation}
\begin{tabular}{l}
$(R'',\tupu')=\ppg(R,\tupu)$,  \\
$R''=\ppg_\star(R, \tupu)$, \\ 
$u'_i=\ppg_i(R,\tupu)$, \\ 
$\tupu'=\ppg_{1..n}(R,\tupu)$ \\
$\tupu''= \tupu;\tupu' = \ppg'_{1..n}(R,\tupu)$. 
\end{tabular}
\end{equation}

If the first argument \acorr\ of operation \ppg\ is fixed, the corresponding family of tuple-valued unary operations (whose only argument is \tupu) will be denoted by $\ppgr$. By taking the $i$th component of the multi-element result, we obtain element-valued unary operations $\ppgr_i$ producing, resp. updates $\frar{u'_i=\ppgr_{i}(\tupu)}{A'_i}{A''_i}$. We write $\ppgr_{1..n}(\tupu)$ for the tuple $(\ppgr_1(\tupu)...\ppgr_n(\tupu))$.
%Note that $A'_j=A_j$ for all $j\not=i$ (see clause (a) of the definition) while $\ppgr_{ii}$ is the reflective update (b). 
We also have operation $\ppgr_{\star}$ returning a new consistent corr $R''=\ppgr_{\star}(u_i)$ according to \defref{def:mlens}
\end{defin}
\begin{defin}[Closed updates]
	Given a lens $\ell=(\mspaA,\ppg)$, a corr $R\in \R{}\tupleA$ and an update \frar{\tupu}{\tupA}{\tupA'}, we call its component  \frar{u_i}{A_i}{A'_i} $R$-{\em closed}, if the \corring\ amendment  is an identity: $\ppgr_{i}(\tupu)=\id_{A_i'}$. A subtuple update $\tupv < \tupu$ is $R$-closed if all its components are $R$-closed. If the entire \tupu\ is $R$-closed, we call it {\em consistency preserving}.
	
	An subtuple update is $\ell$-{\em closed} if it is $R$-closed for all $R$. Lens $\ell$ is called {\em non-reflective} at foot $\spaA_i$, if all updates in \xupd{\spaA_i} are $\ell$-closed. \qed
\end{defin} 
\zdhl{For the \exIntro, update propagation policies described in \sectref{sec:example} give rise to a lens non-reflective at space $\spA_3$.}{TO BE CHECKED} 
%\endinput
%\vspace{-2ex}
\begin{defin}[Well-behavedness]\label{def:wblens}
A lens $\ell=(\mspaA,\ppg)$ is called {\em well-behaved (wb)} if the following laws hold for all \tupA, $R\in\R{}(\tupA)$ and 
 \frar{\tupu}{\tupA}{\tupA'}, cf. \figref{fig:ppgPatterns-reflect}

%\newcommand\lawind{\ensuremath{$_i$}}
\smallskip\noindent
\begin{tabular}{l@{\qquad}l}
	\lawnamebr{Stability}{}&
	 $\ppg(R,\id)=(R, \id)$  %\mbox{ and } $\ppg^R_{\star}(id) = R$
	\\ [1ex] 
	\lawnamebr{Hippocr1}{} &	
	if $ R\in \consK$ and $R'=\tupu^\bigstar(R)\in\consK$, then $\ppg(R,\tupu)=(R', \id_{\tupA'})$
	\\ [1ex]
	\lawnamebr{Idempotency}{i} &
	$\ppg(R, \ppg'_{1..n}(R,u)) = (\ppg_{\star}(R, \tupu), \id_{\tupA''})$
	\\ [1ex]
		\lawnamebr{Hippocr2}{} &	
	$ \tupu \in \Kspan{}$ implies $(\tupu,\ppg_{1..n}(R, \tupu)) \in \Kupd_{\tupA'}$ 
\end{tabular}\\
%where $u_i' =  \ppgr_{ii}(u_i)$ as in Def.~\ref{def:multi-lenses}.\qed
\end{defin}
\lawname{Stability} says that lenses do nothing voluntarily. \lawname{Idempotecny} says .... 
\zd{To be completed. And I am not sure we need hippo1-2 in this paper.}
 %\lawname{Reflect1} says that amendment works towards ``completion'' rather than ``undoing'', and  \lawname{Reflect2-3} are idempotency conditions to ensure the completion indeed done. %(a sort of \lawname{PutGetPut} law in the lens terminological tradition).
%\footnote{In the lens terminological tradition,
%a sort of \lawname{PutGetPut} law in the lens terminological tradition, \lawname{Reflect1} could be called {\em self-Hippocraticness}, while \lawname{Reflect2} is a sort of \lawname{PutGetPut} law.}  
%%%The converse implication is ensured by the existence of $\acorr''\inn \K(A''_i,\_)$. Law \lawname{Idempt} says that amendment just adjust different  granularities of changes in the feet of the lens.  
%The last law (called \lawname{PutPut} by the same traditional lens style) says that propagation of compatible updates preserves the composition and thus ignores the intermediate history of the updating path if updates do not conflict.
%\exIntro. \lawname{Reflect1} means that an update $u_1$: Add Mary to $A_1$, and its amendment $u'_1$: Add employment (Mary, IBM) to $A'_1$, are considered non-conflicting. \lawname{Reflect2} ensures resulting updates in $A_2$ and $A_3$ to be the same irrespective to whether we propagate $u_1$ or $u_1;u'_1$, and  \lawname{Reflect3} says that no amendment is necessary for propagating $u_1;u'_1$. % the results of propagation if we want to propagate them back (from $A_{2,3}$ to $A_1$) or again (no amendment to $u_1;u'_1$). 
	
	\zd{HERE I STOPPED FOR TODAY. INVERTIBILITY SEEMS TO BE A TOUGH ISSUE}
	
	\begin{definition}[Invertibility] \label{def:invert}
		A wb lens is called {\em (weakly) invertible}, if it satisfies the following law for any $i$, update \frar{u_i}{A_i}{A'_i} and $R\in\R{i}(A_i,\_)$:
		
		\noindent \begin{tabular}{l@{\quad}l}
			\lawnamebr{Invert}{i}%$_{j\noteq i}$
			& for all $j\noteq i$: 
			$\ppgr_{ij}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ij}(u_i)$	
		\end{tabular}
		\qed 	
	\end{definition}
This law deals with ''round-tripping'': operation $\ppgr_{ji}$ applied to 
update $u_j=\ppgr_{ij}(u_i)$ results in update $\hat{u_i}$ equivalent to $u_i$ in the sense that $\ppgr_{ij}(\hat{u_i})=\ppgr_{ij}(u_i)$  (see \cite{me-models11} for a motivating discussion). %it was made apparent that it is a good compromise between proper prevention of unwanted effects on the one hand and leaving enough freedom for the framework on the other hand.
\zdmodno{}{Hmm, \\
	\noindent \begin{tabular}{l@{\quad}l}
	\lawnamebr{Invert{-}strong}{i}%$_{j\noteq i}$
	& for all $j\noteq i$ and all $k$: 
	$\ppgr_{ik}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ik}(u_i)$	
\end{tabular}
}{I just recognized that the much stronger version on the left would perhaps be more reasonable: to think about }
%<<<<<<< HEAD
%\exIntro\ A natural update propagation policy in the example of Sect.\ref{sec:example} is the following: If a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case, already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id_{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%=======
%\exIntro\ A reasonable update propagation policy would be is if a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%>>>>>>> edits thru the whole paper
%The next two (simple) examples will be used in the forthcoming theorems. 	 
\begin{example}[Identity Lens \idlensna]\label{ex:idLens} 
Let $\spaA$ be an arbitrary model space. It generates an $n$-ary lens \idlensna\ as follows: The carrier $\mspaA$ has $n$ identical model spaces: $\spaA_i=\spaA$ for all $i\in\{1,..,n\}$, it has $\R{} = \xob{\spaA}$, and boundary functions are identities. All updates are propagated to themselves (hence the name of \idlensna). Obviously, \idlensna\ is a wb, invertible lens non-reflective at all its feet. \qed 
\end{example}

==> sections/lensesFinal/multiPpg.tex <==
\section{Update Propagation and Multiary (Delta) Lenses}
%\subsection{Update Propagation and Multiary (Delta) Lenses}

Update policies described in \sectref{sec:example} can be extended to cover propagation of all updates $u_i$, $i\in 1...3$ according to the pattern  in \figref{fig:ppgPatterns-reflect}. \zdneww{This is a non-trivial task, but after it is accomplished, we obtain a \syncon\ \fwk, which we algebraically model as an algebraic structure called a {\em well-behaved lens}. In this term,  {\em lens} refers to a collection of diagram operations defined over a multispace of models, which take a configuration of models, corrs and updates and {\em propagate} them, \ie, return another configuration of models, corrs and updates. A lens is called {\em well-behaved}, if propagation operations satisfy a set of algebraic laws specified by equations. This terminological discipline goes back to the first papers, in which lenses were introduced \cite{bpierce-popl05}. We define and discuss well-behaved lenses in the next \sectref{sec:wblens}. In \sectref{sec:vwblens}, we discuss an important special property of lenses: compatibility of update propagation with update composition, which is regulated by the most controversial amongst the lens laws -- the (in) famous PutPut law.}{}{-2em} 

\subsection{Well-behaved lenses}\label{sec:wblens}	

\begin{defin}[Symmetric lenses]\label{def:multi-lenses}
	An $n$-ary {\em symmetric lens} is a pair $\ell=(\mspaA, \ppg)$ with \mspaA\ an $n$-ary multispace called the {\em carrier} of $\ell$, and  $(\ppg_i)_{i\le n}$ an $n$-tuple of operations of the following arities. Operation $\ppg_i$ takes a consistent corr $R$ with boundary $\prt R=\tupleA$,
	and a foot update \frar{u_i}{A_i}{A'_i} as its input, and returns 
	
	%\noindent 
	(a) an $(n-1)$-tuple of updates \frar{u'_j}{A_j}{A''_j} with $1\le j\not= i\le n$; 
	
	%\noindent 
	(b) a {\em reflective} update \frar{u'_i}{A'_i}{A''_i} also called an {\em amendment} of $u_i$, 
	
	%\noindent 
	(c) a new consistent corr $\acorr''\in \tupleAii^\bigstar$. 
	
	\noindent In fact, operation $\ppg_i$ completes a (local) foot update $u_i$ to a (global) tuple update of the entire multimodel, whose  components are $(u_j')_{j\ne i}$ and $u_i;u'_i$ (see \figref{fig:ppgPatterns-reflect}). 
	\qed
\end{defin}
Note that all \ppg\ operations are only defined for consistent corrs and return consistent corrs.
%\begin{mydefin}[Symmetric Lens]
%	A {\em symmetric lens} is a pair $\ell=(\mspaA, \ppg)$ with \mspaA\ a multispace (called the carrier of $\ell$) with model spaces $\spaA_1, \ldots, \spaA_n$, corr set $\R$, and $\ppg = (\ppg_1, \ldots, \ppg_n)$ an $n$-tuple of operations with 
%\[
%\ppg_i: \left\{
%\begin{array}{rcl}
%\xupd{\spaA_i} \times_i \R & \to & \xupd{\spaA_1\times \cdots \times \spaA_n}\times \R \\
%(u_i, R) &\mapsto & (u_1', \ldots, u_n', R'')\\
%\end{array}\right.
%\]	
%for all $i$. $n$ is called the {\em arity} of $\ell$ or, equivalently, $\ell$ is an $n$-ary lens.

%\input{figures/pdfs/alignedMultimodel.tex}
%The notation $\xupd{\spaA_i} \times_i \R$ depicts those pairs $(u_i: A_i\to A_i', R)$ for which $\partial_i(R) = A_i$, or, equivalently, $R\in \R_i(A_i,\_)$, i.e.\ (in the same way as in the binary example) $\ppg_i$ takes as input $R\in \R_i(A_i,\_)$ and an update of $A_i$. For $j\ne i$ it returns (a) updates \frar{u'_j}{A_j}{A''_j} and (b) a {\em reflective} update \frar{u'_i}{A'_i}{A''_i} (also called an {\em amendment} of $u_i$), and (c) a new consistent corr $R''\in \R(A_1'', \ldots, A_n'')$. In fact, operation $\ppg_i$ completes update $u_i$ to a multiupdate 
%
%\[(u_1', \ldots, u_{i-1}', (u_i;u_i'), u_{i+1}', \ldots, u_n')\]
%
%(see \figref{fig:ppgPatterns-reflect})
%\end{mydefin}
%We will employ the following notational conventions. 
{\bf Notation.} If the first argument \acorr\ of operation \ppg$_i$ is fixed, the corresponding family of unary operations (whose only argument is $u_i$) will be denoted by $\ppgr_i$. By taking the $j$th component of the multi-element result, we obtain single-valued unary operations $\ppgr_{ij}$ producing, resp. updates $\frar{u'_j=\ppgr_{ij}(u_i)}{A'_j}{A''_j}$, where $A'_j=A_j$ for all $j\not=i$ (see clause (a) of the definition) while $\ppgr_{ii}$ is the reflective update (b). We also have operation $\ppgr_{i\star}$ returning a new consistent corr $R''=\ppgr_{i\star}(u_i)$ according to (c).
\begin{defin}[Closed updates]
	Given a lens $\ell=(\mspaA,\ppg)$ and a corr $R\in \tupleA^\bigstar$, we call an update \frar{u_i}{A_i}{A'_i} $R$-{\em closed}, if $\ppgr_{ii}(u_i)=\id_{A_i'}$. An update is $\ell$-{\em closed} if it is $R$-closed for all $R$. Lens $\ell$ is called {\em non-reflective} at foot $\spaA_i$, if all updates in $\spA_i$ \ %\xupd{\spA_i} 
	are $\ell$-closed. \qed
\end{defin} 
\zd{Below is an important piece which is not easy to write b/c we don't have really strong arguments. It needs completion.}
\\
\hk{I'm not sure whether you want it to be placed here or better in the introduction. Please decide!}
\par
\zdneww{Update propagation policies discussed in Sect.2 give rise to a 3-ary lens. 
\\
	....
\\
	Consistency restoration is not unique, there are different policies. ....Based on heuristics etc ...
\\
We will not actually define the lens -- it can be done along the lines of how binary symmetric lens are defined with, \eg, triple graph grammars \cite{?}. Our goal in the paper is to describe general laws, and show their consistency with simple mathematical examples described below. 
For the \exIntro, update propagation policies described in \sectref{sec:example} give rise to a lens non-reflective at space $\spA_3$.}{important piece which is not easy to write}{-8em}

\begin{defin}[Well-behaved lenses]\label{def:wblens}
	A lens $\ell=(\mspaA,\ppg)$ is called {\em well-behaved (wb)} if the following laws hold for all $i\le n$, $A_i\in\xob{\spaA_i}$, 
	$R\in \Kcorr _{A_i}\subset A_i^\bigstar$ and \frar{u_i}{A_i}{A'_i}, cf. \figref{fig:ppgPatterns-reflect}
	
	\lawgap=1ex
	%\newcommand\lawind{\ensuremath{$_i$}}

	\smallskip\noindent
	\begin{tabular}{l@{\quad}l}
% = stability law
		\lawnamebr{Stability}{i}&
		$\forall j\in\{1...n\}: \ppgr_{ij}(\id_{A_i})=\id_{A_j}$\mbox{ and } $\ppg^R_{i\star}(id_{A_i}) = R$
%		\\  [\lawgap] &
%		 \lawnamebr{Hippocr}{i} &
%		 Let $A_j=\prt_jR$ for $j\le n$ (and hence $\prt_iR=A_i$).
%		 %\noteq i$, $\ovr{u_i}=(\id_{A_1}...u_i...\id_{A_n})$ and $A'=(A_1...A'_i...A_n)$. 
%		 \\ [0.5ex] &
%		  	If  $R'=u_i^\bigstar(R) \in \Kcorr_{A_i'}$, \ie, realignment returns a consistent corr, 
%		\\ & 
%		then $\ppgr_{ij}(u_i)=\id_{A'_j}$ for all $j\le n$, and $\ppgr_{i\star}(u_i)=R'$.
		\\[\lawgap]
		 \lawnamebr{Reflect1}{i} &	
		$(u_i, \ppgr_{ii}(u_i))\in \Kupd_{A_i'}$ %for all $u_i$ 
		\\[\lawgap]
		\lawnamebr{Reflect2}{i} &
		$\ppgr_{ij}(u_i;\ppgr_{ii}(u_i)) = \ppgr_{ij} (u_i)$ for all $j\noteq i$
		\\  [\lawgap]  
		\lawnamebr{Reflect3}{i} &
			$\ppgr_{ii}(u_i;\ppgr_{ii}(u_i))=\id_{A''_i}$ 
			where $A''_i$ is the target model of $\ppgr_{ii}$.
			% $u_i' =  \ppgr_{ii}(u_i)$ as in Def.~\ref{def:multi-lenses} 
		%	\\  [\lawgap] \lawnamebr{PutPut}$\forall w_i\inn\Kupd_{A''}(u''_i,\_),$ 
		%	& \pputi
		%	\\	[-0.1\lawgap] $\hphantom{\lawnamebr{PutPu}}$
		%	$\forall  j\noteq i$ 
		%	&  \pputii
		%	%	$\ppgr_{ij}(u''_i~; w_i)=\ppgr_{ij}(u''_i) ; \ppg^{\acorr''}_{ij}(w_i)$,  
		%	%	\\ [0.5\lawgap] & 
		%	%	 and $(\ppgr_{ij}(u''_i),~\ppg^{\acorr''}_{ij}(w_i))\in \Kupd_{A''_j}$
	\end{tabular}\\
\end{defin}
\zdmodd{\lawname{Hippocr} law says that if realignment returns a consistent corr, nothing should be done.}{\lawname{Stability} says that lenses do nothing voluntarily}{HIPPO}{-1em}
 \lawname{Reflect1} says that amendment works towards ``completion'' rather than ``undoing'', and  \lawname{Reflect2-3} are idempotency conditions to ensure the completion indeed done. 

\zd{Hippocr implies Stability is commented}
%Because alignment $\mspA^\bigstar$ is a functor, it preserves identities. This together with \lawname{Hippocr} implies \lawname{Stability}, which says that lenses do nothing voluntarily:
%\begin{corollary}[{\sf Stability}]\label{cor:1} 
%%\smallskip\noindent
%%		\begin{tabular}{l@{\qquad}l}
%%				&
%			{\em	If $\ell$ is wb, then for all consistent corrs $R$ and all $i,j\le n$: $\ppgr_{ij}(\id_{A_i})=\id_{A_j}$\mbox{ and } $\ppg^R_{i\star}(\id_{A_i}) = R$}
%%				\\  [1ex]
%%	\end{tabular} 
%\qed
%\end{corollary}
%The last law (called \lawname{PutPut} by the same traditional lens style) says that propagation of compatible updates preserves the composition and thus ignores the intermediate history of the updating path if updates do not conflict.
\begin{defin}[{\sf Invertibility}] \label{def:invert}
	A wb lens is called {\em (weakly) invertible}, if it satisfies the following law for any $i$, update \frar{u_i}{A_i}{A'_i} and $R\in A_i^\bigstar$:
	
	\noindent \begin{tabular}{l@{\quad}l}
		\lawnamebr{Invert}{i}%$_{j\noteq i}$
		& for all $j\noteq i$: 
		$\ppgr_{ij}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ij}(u_i)$	
	\end{tabular}
	\qed 	
\end{defin}
This law deals with ''round-tripping'': operation $\ppgr_{ji}$ applied to 
update $u_j=\ppgr_{ij}(u_i)$ results in update $\hat{u_i}$ equivalent to $u_i$ in the sense that $\ppgr_{ij}(\hat{u_i})=\ppgr_{ij}(u_i)$  (see \cite{me-models11} for a motivating discussion). %it was made apparent that it is a good compromise between proper prevention of unwanted effects on the one hand and leaving enough freedom for the framework on the other hand.
\zdmodno{}{Hmm, \\
	\noindent \begin{tabular}{l@{\quad}l}
		\lawnamebr{Invert{-}strong}{i}%$_{j\noteq i}$
		& for all $j\noteq i$ and all $k$: 
		$\ppgr_{ik}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ik}(u_i)$	
	\end{tabular}
}{I just recognized that the much stronger version on the left would perhaps be more reasonable: to think about }
%<<<<<<< HEAD
%\exIntro\ A natural update propagation policy in the example of Sect.\ref{sec:example} is the following: If a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case, already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id_{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%=======
%\exIntro\ A reasonable update propagation policy would be is if a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%>>>>>>> edits thru the whole paper
%The next two (simple) examples will be used in the forthcoming theorems. 	 
\begin{example}[Trivial lenses \trivlensna]\label{ex:TerminalLens} 
	%\subsection{Terminal categories and lenses.} 
	A category consisting of one object and one (necessary identity) arrow is called {\em terminal}. All terminal categories are isomorphic; we fix one, whose object is denoted by $1$ while the category is denoted by \trmcat\ (bold 1). The terminal category \trmcat\ gives rise to a unique {\em terminal space} with  $\Kupd_1 = \{(id_1,id_1)\}$.
	%\begin{example}[Terminal lens \trmlens]
	
	Any model space \spA\ gives rise to the following {\em trivial} $n$-ary lens \trivlensna. The first foot space $\spA_1=\spA$ while for all $j=2..n$, $\spA_j=\trmcat$.   %\footnote{
	Tuple models are uniquely determined by their first foot, and given such a model $(A,1...1)$, the set of corrs is the singleton $\{\etosing{A}\}$ with $\prt_1\etosing{A}=A$ and $\prt_{2..n}\etosing{A}=1$, and this only corr is considered consistent. Hence, all mutlimodels are consistent and update propagation is not actually needed. For any \spA, lens $\trivl_n(\spA)$ is a wb, invertible lens non-reflective at all its feet in a entirely trivial way.\qed  
\end{example}
%\zd{still I decided to distinguish an element $x$ and a corr made from that element as \etosing{x}. The latex macros is} \verb|\etosing| \zd{(read "element to a singleton") in the file macros/thisPaper. This will be used many times below}

The next example is more interesting.
\begin{example}[Identity Lenses \idlensna]\label{ex:idLens} 
	Let $\spaA$ be an arbitrary model space. It generates an $n$-ary lens \idlensna\ as follows. The carrier $\mspaA$ has $n$ identical feet spaces: $\prtbf_i\mspaA=\spaA$ for all $i=1..n$. The corr set for a tuple model $ A\!\!A=(A_1..A_n)$, \ie, set $A\!\!A^\bigstar$, is the singleton $\{\etosing{A\!\!A }\}$ with $\prt_i\etosing{A\!\!A}=A_i$, and this corr is consistent iff all $A_i=A$ for some model $A\in\xob{\spA}$.  All updates are propagated to themselves (hence the name of \idlensna). Obviously, \idlensna\ is a wb, invertible lens non-reflective at all its feet. \qed 
\end{example}

\subsection{Very well-behaved lenses}\label{sec:vwblens}	


We consider an important property of update propagation---its compatibility with update composition. A simple compositionality law would require that the composition $u_i;v_i$ of two consecutive foot updates \frar{u_i}{A_i}{A'_i}, \frar{v_i}{A'_i}{B_i}, is propagated into the composition of propagations: 
$\ppgr_{ij}(u_i;v_i)=\ppgr_{ij}(u_i);\ppgrx{R''}_{ij}(v_i)$ with $R''$ being the corr provided by the first propagation, $R''=\ppgr_{i\star}(u_i)$. It is however well known that such a simple law (called PutPut) often does not hold. 

\input{figures/pdfs/ex-putput1.tex}
Figure~\ref{fig:ex-putput1} presents a simple example (we use a more compact notations, in which \name-attributes are placed at the OID boxes).  At the initial moment, the binary multimodel $(\ai, \aii)$ with the (implicit) corr given by name matching is consistent: the only intermodel constraint (C1) is satisfied. Update $u_1$ adds a new employment record to model \ai, constraint (C1) is violated, and to restore consistency, a new employment is added to \aii\ by update $u_2=\ppgr_{12}(u_1)$ (the new propagated model and update are shown with blue lines and blank).  Then  update $v_1$ deletes the record added by $u_1$, but as the resulting multimodel $(A''_1, A'_2)$  remains consistent, nothing should be done (the law of (Stability)) and thus $v_1$ is propagated to identity, $v_2=\ppgrx{R''}_{12}(v_1) =\id_{A'_2}$. Now we notice that the composition $(u_1;v_1)$ is identity and hence to be propagated to identity, \ie, $\ppgr_{12}(u_1;v_1) = \id_{A_2}$, while $\ppgr_{12}(u_1);\ppgrx{R''}_{12}(v_1) =u_2;v_2=u_2 \noteq \id_{A_2}$, and $A''_1\noteq A''_2$.  Obviously, the violation story will still hold if models \ai\ and \aii\ are much bigger and updates $u_1$ and $v_1$ are parts of bigger updates (but Mary should not appear in \ai).  

\input{figures/pdfs/ex-putput2.tex}
Figure~\ref{fig:ex-putput2} presents a more interesting ternary example. Multi-model $\nia$ is consistent, but update $u_3$ deletes route \#1 and violates constraint (C2). In this case, the most direct propagation policy would delete all employment records related to \#1\ but, to keep changes minimal, would keep people in $A_1$ and companies in $A_2$ as specified by model $\nia'$ in the figure. Then a new route is inserted by update $v_3$  (note the new OID), which has the same \from\ and \toattr\ attributes as route \#1. There are multiple ways to propagate such an insertion. The simplest is to do nothing as the multimodel $(A'_1.A'_2,A''_3, R'=\varnothing)$ is consistent (recall that mapping \etor\ is not necessarily surjective).  However, we can assume a more intelligent policy that looks for people with address a1 in the first database (and finds John and Mary), then checks somehow (\eg, by other attributes in the database schema $M_1$ which we did not show) if some of them are recent graduates in IT (and, for example, finds that Mary is such) and thus could work for a company at the address a10 (Google). Then such a policy would propagate update $v_3$ to $v_1$ and $v_2$ as shown in the figure. The composition of updates $u_3$ and $v_3$  is, in fact, an identity as object identifiers are normally invisible, and thus $u_3;v_3$ would be propagated to the identity on the multimodel \nia. However, $\nia''\noteq\nia$ and Putput again fails.

Note that a common feature of the two examples is that the second update $v$ fully reverts the effect of the first one, $u$, while their propagations do not fully enjoy such a property due to some ``side effects''. In fact, Putput is violated if update $v$ would just partially revert update $u$. Several other examples and a more general discussion of this phenomenon that forces Putput to fail can be found in \cite{me-bx17}. However, it makes sense to require compositional update propagation for two {\em sequentially compatible} updates in the sense of \defref{def:mspace}; we call the respective version of the law \kputput\ with 'k' recalling the sequential compatibility relation \Kupd. To manage update amendments, we will also need to use update merging operator \merge\ as shown in \figref{fig:putput}  


\begin{defin}[Very well-behaved lenses] \label{def:putput}
	A wb lens is called {\em very well behaved (vwb)}, if it satisfies the following \kputputlaw\ for any $i$, corr $R\in A_i^\bigstar$, and updates \frar{u_i}{A_i}{A'_i}, \frar{v_i}{A'_i}{B_i} (see \figref{fig:putput}).
	
	Let $u'_i:=\ppgr_{ii}(u_i)$. If $(u_i,v_i)\in\Kupd_{A_i'}$  and  $(v_i,u'_i)\in\Kdisj{}_{A_i'}$, 
	then $(\tilde v_i, \tilde u'_i):=\merge(v_i, u'_i)$ is defined (see \figref{fig:putput}) and the following equalities hold:
	
	\smallskip
	\noindent \begin{tabular}{l@{\quad}ll}
		\multirow{2}{*}{\lawnamebr{\kputput}{j\noteq i}}  & % row 1
			$\ppgr_{ij}(u_i;v_i)=
		\ppgr_{ij}(u_i);\ppg^{R''}_{ij}(\widetilde{u'_i})$, 
		\\ [0.5ex]	& % row 2
		and $(\ppgr_{ij}(u_i),\ppg^{R''}_{ij}(\widetilde{u'_i}))\in \Kupd_{A_j''}$,
				\\ [0.5ex] 
			\lawnamebr{\kputput}{ii}	&
		and $\ppgr_{ii}(u_i;v_i) = \widetilde{v_i};\ppg^{R''}_{ii}(\widetilde{u_i'})$,
	\end{tabular}\\
see the dashed arrows in \figref{fig:putput}, which depict the propagation of the composed updates. \qed 	
\end{defin}
\input{figures/diags/putput.tex}


\endinput

Update policies described in \sectref{sec:example} can be extended to cover propagation of all updates $u_i$, $i\in 1...3$ according to the pattern  in \figref{fig:ppgPatterns-reflect}. This is a non-trivial task, but after it is accomplished, we have the following \syncon\ structure. 

\noindent 
\begin{minipage}[t]{0.675\textwidth}
\begin{defin}[Symmetric lenses]\label{def:mlens}
	An $n$-ary {\em symmetric lens} is a pair $\ell=(\mspaA, \ppg)$ with \mspaA\ an $n$-ary multispace called the {\em carrier} of $\ell$, and  \ppg\ the following {\em propagation} operation. It takes a corr $R$ (in fact, a multimodel) with boundary $\prt R=\tupA=\tupleA$,
	and an update \frar{\tupu}{\tupA}{\tupA'} as its input, and returns  a multimodel with corr $R''$ and boundary $\tupA''=\prt R''$ produced by an amendment update \frar{u'}{\tupA'}{\tupA''} as shown in the diagram on the right, in which$\tupu''=\tupu;\tupu'$ (recall that given elements are framed and solid, derived ones are non-framed and dashed). \qed
\end{defin}
\end{minipage}\qquad
\begin{minipage}[t]{0.245\textwidth}
	%\vspace{-2ex}
	\input{figures/diags/lensDef}
\end{minipage}

Note that the tuple model $\tupA'$ is not necessary the boundary of some (consistent) corr $R'$. If it is, then amendment $\tupu$ would be an identity,  $R''=R'$, and $\tupu''=\tupu$.    

\begin{defin}[Notation.]
As operation \ppg\ produces several component, it actually gives rise to several operations \corring\ to the parts of the output: we write
\begin{equation}
\begin{tabular}{l}
$(R'',\tupu')=\ppg(R,\tupu)$,  \\
$R''=\ppg_\star(R, \tupu)$, \\ 
$u'_i=\ppg_i(R,\tupu)$, \\ 
$\tupu'=\ppg_{1..n}(R,\tupu)$ \\
$\tupu''= \tupu;\tupu' = \ppg'_{1..n}(R,\tupu)$. 
\end{tabular}
\end{equation}

If the first argument \acorr\ of operation \ppg\ is fixed, the corresponding family of tuple-valued unary operations (whose only argument is \tupu) will be denoted by $\ppgr$. By taking the $i$th component of the multi-element result, we obtain element-valued unary operations $\ppgr_i$ producing, resp. updates $\frar{u'_i=\ppgr_{i}(\tupu)}{A'_i}{A''_i}$. We write $\ppgr_{1..n}(\tupu)$ for the tuple $(\ppgr_1(\tupu)...\ppgr_n(\tupu))$.
%Note that $A'_j=A_j$ for all $j\not=i$ (see clause (a) of the definition) while $\ppgr_{ii}$ is the reflective update (b). 
We also have operation $\ppgr_{\star}$ returning a new consistent corr $R''=\ppgr_{\star}(u_i)$ according to \defref{def:mlens}
\end{defin}
\begin{defin}[Closed updates]
	Given a lens $\ell=(\mspaA,\ppg)$, a corr $R\in \R{}\tupleA$ and an update \frar{\tupu}{\tupA}{\tupA'}, we call its component  \frar{u_i}{A_i}{A'_i} $R$-{\em closed}, if the \corring\ amendment  is an identity: $\ppgr_{i}(\tupu)=\id_{A_i'}$. A subtuple update $\tupv < \tupu$ is $R$-closed if all its components are $R$-closed. If the entire \tupu\ is $R$-closed, we call it {\em consistency preserving}.
	
	An subtuple update is $\ell$-{\em closed} if it is $R$-closed for all $R$. Lens $\ell$ is called {\em non-reflective} at foot $\spaA_i$, if all updates in \xupd{\spaA_i} are $\ell$-closed. \qed
\end{defin} 
\zdhl{For the \exIntro, update propagation policies described in \sectref{sec:example} give rise to a lens non-reflective at space $\spA_3$.}{TO BE CHECKED} 
%\endinput
%\vspace{-2ex}
\begin{defin}[Well-behavedness]\label{def:wblens}
A lens $\ell=(\mspaA,\ppg)$ is called {\em well-behaved (wb)} if the following laws hold for all \tupA, $R\in\R{}(\tupA)$ and 
 \frar{\tupu}{\tupA}{\tupA'}, cf. \figref{fig:ppgPatterns-reflect}

%\newcommand\lawind{\ensuremath{$_i$}}
\smallskip\noindent
\begin{tabular}{l@{\qquad}l}
	\lawnamebr{Stability}{}&
	 $\ppg(R,\id)=(R, \id)$  %\mbox{ and } $\ppg^R_{\star}(id) = R$
	\\ [1ex] 
	\lawnamebr{Hippocr1}{} &	
	if $ R\in \consK$ and $R'=\tupu^\bigstar(R)\in\consK$, then $\ppg(R,\tupu)=(R', \id_{\tupA'})$
	\\ [1ex]
	\lawnamebr{Idempotency}{i} &
	$\ppg(R, \ppg'_{1..n}(R,u)) = (\ppg_{\star}(R, \tupu), \id_{\tupA''})$
	\\ [1ex]
		\lawnamebr{Hippocr2}{} &	
	$ \tupu \in \Kspan{}$ implies $(\tupu,\ppg_{1..n}(R, \tupu)) \in \Kupd_{\tupA'}$ 
\end{tabular}\\
%where $u_i' =  \ppgr_{ii}(u_i)$ as in Def.~\ref{def:multi-lenses}.\qed
\end{defin}
\lawname{Stability} says that lenses do nothing voluntarily. \lawname{Idempotecny} says .... 
\zd{To be completed. And I am not sure we need hippo1-2 in this paper.}
 %\lawname{Reflect1} says that amendment works towards ``completion'' rather than ``undoing'', and  \lawname{Reflect2-3} are idempotency conditions to ensure the completion indeed done. %(a sort of \lawname{PutGetPut} law in the lens terminological tradition).
%\footnote{In the lens terminological tradition,
%a sort of \lawname{PutGetPut} law in the lens terminological tradition, \lawname{Reflect1} could be called {\em self-Hippocraticness}, while \lawname{Reflect2} is a sort of \lawname{PutGetPut} law.}  
%%%The converse implication is ensured by the existence of $\acorr''\inn \K(A''_i,\_)$. Law \lawname{Idempt} says that amendment just adjust different  granularities of changes in the feet of the lens.  
%The last law (called \lawname{PutPut} by the same traditional lens style) says that propagation of compatible updates preserves the composition and thus ignores the intermediate history of the updating path if updates do not conflict.
%\exIntro. \lawname{Reflect1} means that an update $u_1$: Add Mary to $A_1$, and its amendment $u'_1$: Add employment (Mary, IBM) to $A'_1$, are considered non-conflicting. \lawname{Reflect2} ensures resulting updates in $A_2$ and $A_3$ to be the same irrespective to whether we propagate $u_1$ or $u_1;u'_1$, and  \lawname{Reflect3} says that no amendment is necessary for propagating $u_1;u'_1$. % the results of propagation if we want to propagate them back (from $A_{2,3}$ to $A_1$) or again (no amendment to $u_1;u'_1$). 
	
	\zd{HERE I STOPPED FOR TODAY. INVERTIBILITY SEEMS TO BE A TOUGH ISSUE}
	
	\begin{definition}[Invertibility] \label{def:invert}
		A wb lens is called {\em (weakly) invertible}, if it satisfies the following law for any $i$, update \frar{u_i}{A_i}{A'_i} and $R\in\R{i}(A_i,\_)$:
		
		\noindent \begin{tabular}{l@{\quad}l}
			\lawnamebr{Invert}{i}%$_{j\noteq i}$
			& for all $j\noteq i$: 
			$\ppgr_{ij}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ij}(u_i)$	
		\end{tabular}
		\qed 	
	\end{definition}
This law deals with ''round-tripping'': operation $\ppgr_{ji}$ applied to 
update $u_j=\ppgr_{ij}(u_i)$ results in update $\hat{u_i}$ equivalent to $u_i$ in the sense that $\ppgr_{ij}(\hat{u_i})=\ppgr_{ij}(u_i)$  (see \cite{me-models11} for a motivating discussion). %it was made apparent that it is a good compromise between proper prevention of unwanted effects on the one hand and leaving enough freedom for the framework on the other hand.
\zdmodno{}{Hmm, \\
	\noindent \begin{tabular}{l@{\quad}l}
	\lawnamebr{Invert{-}strong}{i}%$_{j\noteq i}$
	& for all $j\noteq i$ and all $k$: 
	$\ppgr_{ik}(\ppgr_{ji}(\ppgr_{ij}(u_i))) = \ppgr_{ik}(u_i)$	
\end{tabular}
}{I just recognized that the much stronger version on the left would perhaps be more reasonable: to think about }
%<<<<<<< HEAD
%\exIntro\ A natural update propagation policy in the example of Sect.\ref{sec:example} is the following: If a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case, already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id_{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%=======
%\exIntro\ A reasonable update propagation policy would be is if a person-company-pair $(p,c)$ is known in $A_1$ and $A_2$, then addition / deletion of an employment of $p$ at $c$ in $A_1$ requires doing the same in $A_2$ and vice versa. This symmetry is a typical example for invertibility. In this case already $\ppg^R_{21}(\ppg^R_{12}(u_1)) = u_1$. The weaker law is needed, if update $u_1:A_1\to A_1'$ causes no changes (\eg, some completely unknown person moves to downtown), hence $u_2 = \id{A_2}$, thus $\ppg^R_{21}(\ppg^R_{12}(u_1)) = \id_{A_1}$ by \lawnamebr{Stability}. Nevertheless, $\ppg^R_{12}(\ppg^R_{21}(\ppg^R_{12}(u_1))) = \id_{A_2} = \ppg_{12}^R(u_1)$, as required.  
%>>>>>>> edits thru the whole paper
%The next two (simple) examples will be used in the forthcoming theorems. 	 
\begin{example}[Identity Lens \idlensna]\label{ex:idLens} 
Let $\spaA$ be an arbitrary model space. It generates an $n$-ary lens \idlensna\ as follows: The carrier $\mspaA$ has $n$ identical model spaces: $\spaA_i=\spaA$ for all $i\in\{1,..,n\}$, it has $\R{} = \xob{\spaA}$, and boundary functions are identities. All updates are propagated to themselves (hence the name of \idlensna). Obviously, \idlensna\ is a wb, invertible lens non-reflective at all its feet. \qed 
\end{example}

==> sections/lensesFinal/multimodSpaces-Newest.tex <==
\subsection{Correspondences and Multimodels}
\zd{This is the newer non-functorial version of the section. To switch to the functorial one -- switch from multimodSpaces-Newest to multimodSpaces-new}
We will work with families of model spaces indexed by a finite set $I$, whose elements can be seen as space {\em names}. To simplify notation, we will assume that $I=\{1,\ldots,n\}$ \zdmoddno{although ordering will not play any role in our \fwk.}{}{Importantly!!}{-2ex} Given a tuple of model spaces $\spA_1, \ldots, \spA_n$, we will refer to objects and arrows of the product category $\prod\spA=\spaA_1\timm\cdots\timm\spaA_n$ as {\em tuple models}  and {\em tuple updates},  
%(sometimes, as {\em discrete multimodels /multiupdates},)
 and denote them by letters without indexes, \eg, \frar{\tupu}{\tupA}{\tupA'} is a family \frar{u_i}{A_i}{A'_i}, $i=1..n$.  
%For family of model spaces  $\spA=(\spA_1, \ldots, \spA_n)$, 
%An n-ary {\em alignment} \fwk\ %over \spA\ is a functor \frar{}{}{}
We will call components of tuple models and updates their {\em feet}. We also call elements of a particular space $\spA_i$ {\em foot} models and {\em foot} updates. %Another terminology we will also use is {\em foot} models and updates for elements of a particular space, and {\em feet} models and updates for elements of the product category, \ie, tuples. 

\zdmodd{For this paper, we are interested in a special class of tuple updates, whose all feet besides one are identities, \ie, updates of the type $(\id_{A_1}..u_i..\id_{A_n})$ for some $i\le n$; we will call such updates {\em singular}. % and denote the full subcategory of $\prod\spA$ consisting of singular updates by $\prosing\spA$. 
	%Given $i\le n$, we call an update \frar{u_i}{A_i}{A'_i} in space $\spA_i$ an $i${\em -update} for some given }{Important!}{-4em}
Given a tuple model $A=(A_1...A_n)$, any foot update \frar{u_i}{A_i}{A'_i} gives rise to a unique singular update \frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % in \prosing\spA, 
where $\ovr{A'_i}=(A_1..A'_i..A_n)$ and $\ovr{u_i}=(\id_{A_1}..u_i..\id_{A_n})$ (and any singular update is such). Note also that any tuple update $u=u_1...u_n$ can be represented as a sequential composition $\ovr{u_1}...\ovr{u_n}$ of singular updates (taken in any order). 
}{}{not sure but i seems we don;t need it}{-4em}



%\input{sections/lensesFinal/multispace-old}
%\input{sections/lensesFinal/multispace-total} see below
\begin{defin}[Multispaces, Alignment, Consistency]
\label{def:mspace}
	Let $n\ge 2$ be a natural number. An {\em n-ary multi-space \zdmod{(with alignment)}{}{}} \mspA\ is a given by the following three components. The first one is a tuple of model spaces $\spA = (\spaA_1, \ldots, \spaA_n)$ called the {\em boundary} of \mspA\ (and denoted by \bounmspA\ if we need an explicit reference to the multispace). The second component is a class \Corrsma\ of elements called {\em correspondences} or {\em corrs} together with a family of {\em boundary} mappings \frar{\prt_i}{\Corrsma}{\xob{\spA_i}}, $i\le n$.  A corr $R\in\Corrsma$ is understood as a correspondence specification interrelating models $A_i=\prt_iR\eqdef\prt_i(R)$; the latter are also called {\em R's feet}, and we say that models $A_i$ are aligned via $R$.
	
	We require all boundary mappings $\prt_i$ to be surjective so that for any model tuple  $A=(A_1...A_n)\in\xob{(\prod\spA)}$, the set 
	$$A^\bigstar\eqdef\compr{R\in\Corrsma}{\prt R=A, \ie, \prt_iR=A_i \mbox{ for all $i\le n$}}$$
	is not empty. %We will also write $A=\prt R$ if the condition above holds. 
	To make the notation discipline above uniform, we will write $A_i^\bigstar\eqdef \compr{R\in\spA^\bigstar}{\prt_i R=A}$ for the class of all corrs with a given foot $A_i\in\xob{\spA_i}$, and $\Corrsa$ for the class of all corrs \Corrsma.
	
	% === from the functorial def 
	%\[\frar{{\_}^\bigstar_{\mspaA}}{\prodmspA}{\setcat}\]
	%where \prodmspA\ denotes the category 
	%$\prod\bounmspA =\spaA_1\timm\ldots\timm\spA_n$. We will omit the subindex $\__\mspA$ if it is clear from the context. 
	%
%		\[\frar{\mspA^\bigstar}{\prosing\spA}{\setcat}\]
%		such that all sets $\mspA^\bigstar(A)$, $A=(A_1..A_n) \inn \xob{(\prod\spA)}$, are disjoint.
%	 To simplify notation, given an update %\frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % 
%	 \frar{u}{A}{A'}
%	 from a model tuple $A=(A_1..A_n)$ to a model tuple $A'=(A'_1..A'_n)$, 
%	 we will write $A^\bigstar$ for the set $\mspA^\bigstar(A)$, and \frar{u^\bigstar}{A^\bigstar}{A'^\bigstar} %{\ovr{A'_i}^\bigstar}
%	  for the function $\mspA^\bigstar(u)$. 
%	 Analogously, given a tuple model $A$ and a foot update \frar{u_i}{A_i}{A'_i}, function $\ovr{u_i}^\bigstar$ is denoted by $u_i^\bigstar$.	%\zd{so, i decided to keep the notation used in the Fase paper for consistency of the two papers, but in the present one we will use the simplified variant}
%	
%	Given a model tuple $\tupA = (A_1..A_n)$, elements of the set $ \xstar{\tupA}$ are called {\em \corrce s} or just {\em corrs} over \tupA. Intuitively, a corr $R\in\xstar{\tupA}$ is understood as a correspondence specification interrelating models $A_i$; we will also say that the latter are {\em aligned} via $R$, and that \tupA\ is the {\em boundary} of $R$ and we write $\tupA=\prt R$ (recall the disjointness condition above). A foot update \frar{u_i}{A_i}{A'_i} creates a new corr $R'=u_i^\bigstar(R)\in \ovr{A'_i}^\bigstar$ called the {\em realignment} of the model $(A,R)$.Due to functoriality of $\mspA^\bigstar$, the operation of realignment is fully determined by realignment caused by  singular updates: given $u=(u_1...u_n)$, $u^\bigstar=u^\bigstar_1;...;u^\bigstar_n$.

	The third component is a class of {\em consistent} corrs $\Korrsma\subset\Corrsa$. We write $\Kcorr_A$ for $\Korrsma\cap A^\bigstar$ and $\Kcorr_{A_i}$ for $\Korrsma\cap A_i^\bigstar$. 
%	\[ 
%	\comprfam{\Kcorr_A\subseteq A^\bigstar}%
%	{{A=(A_1..A_n) \in \xob{(\prod\spA)}}} 
%	\]
% indexed by model tuples. %Note that for an update \frar{u_i}{A_i}{A'_i} and a corr $R\in \Kcorr_A$, we do not require its realignment $R'=u_i^\bigstar(R)$ to be necessary consistent, \ie, it may happen that $R'\notin \Kcorr_{A'}$ and thus consistency restoration is needed. 
% \par	
%We will write $\spA^\bigstar$ for the class of all corrs, $\Kcorr_\spA$ for its subclass of consistent corrs and, for a given model $A_i\in\xob{\spA_i}$, $A_i^\bigstar\eqdef \compr{R\in\spA^\bigstar}{\prt_i R=A}$ for the class of all corrs with a fixed foot $A_i\in \xob{\spA_i}$ and $\Kcorr_{A_i}\subset A_i^\bigstar$ for the subclass of all such consistent corrs. 
\qed
\end{defin}
\zd{the new def above is in the section "lensesFinal/multimodSpaces-Newest" while the previuous functorial def is in section ".../multimodSpaces".}
\begin{defin}[Multimodels]\label{def:mmodel}	
  An {\em (aligned) multimodel} over a multispace \mspA\ is a couple $\nia=(A, R)$ of a model tuple $\tupA=(A_1..A_n)$\ with a corr $R\in\xstar{\tupA}$ relating the component models. We then write $\nia\in\mspA$ although this is a more complex relation than set membership. A model is {\em consistent} if the corr $R$ is consistent.
%A {\em multimodel update} \frar{\tupu}{\nia}{\nia'} is a tuple of updates (\frar{u_1}{A_1}{A'_1}, \ldots, \frar{u_n}{A_n}{A'_n}). Equality $\xstar{\tupu}(R)=R'$ is not required.

\zdmoddok{For a given model $\nia=(A,R)$, any foot update \frar{u_i}{A_i}{A'_i} (we will also say {\em local} update) gives rise to a ({\em global}) feet update  $\ovr{u_i}=(\id_{A_1}...u_i...\id_{A_n})$, and we write $u_i^\bigstar(R)$ for the corr $R'\eqdef \ovr{u_i}^\bigstar(R)\in A'^\bigstar$ where $A'=(A_1,..,A_{i-1}, A'_i, A_{i+1}, ..,A_n)$. Again, if even $R$ is consistent, its realignment $R'$ may be inconsistent, and then we say that update $u_i$ destroyed the consistency of model \nia.}{}{it seems it's just a repetition}{-4em}
Note that any corr $R$ uniquely defines a multimodel via the corr's boundary function.
%	
	%Obviously, multimodels and their updates form a category denoted by $\mspA^\#$. As a rule, we will omit the superindex thus denoting the multispace and the category it generates by the same symbol \mspA\ relying on the context to resolve ambiguity. %Normally, the context will suggest what the symbol means and, thus, \xob{\mspA} denotes the set of all multimodels and $\mspA(\tupA,\tupA')$ is the respective hom-set. 	As equality $\xstar{\tupu}(R)=R'$ is not required for multimodel updates, we have $\mspA^\#(\nia,\nia')=\mspA^\Pi(\prt\nia,\prt\nia')$
	\qed
\end{defin}
%\exIntro\ 
\begin{example}
The \exIntro\ of Sect.\ref{sec:example} %, the tuple $\spA_{1,2,3}$ 
gives rise to a 3-ary multimodel space. For $i\le3$, space $\spA_i$ consists of all models instantiating metamodel $M_i$ in  Fig.\ref{fig:multiMetamod-uml} and their updates. Given a model tuple $A=(A_1, A_2, A_3)$, a corr $R\in A^\bigstar$ is given by a triple of relations: $\ptop^R, \ctoc^R, \etor^R$ as described in \riii, \rii\
on p.~\pageref{pg:constr}. 
%R=(R_\Person, R_\Company, R_\Route)$, where $R_\Person\subset \Person^{A_1}\timm\Person^{A_2}$, $R_\Company\subset \Company^{A_1}\timm\Company^{A_2}$ and $R_\Route \subset \Route^{\ai{*}\aii}\times \Route^\aiii$ (see p.~\pageref{pg:constr} for the definition of $\Route^{\ai{*}\aii}$).  
If we rely on person and company names as keys, then relations $\ptop^R$, $\ctoc^R$ are derived from foot models $A_1$ and $A_2$, but if these keys are not reliable, then the two relations are independent components of the multimodel. Relation $\etor^R$ is always an independent component. 

\zdmodd{
Realignment (for foot, and hence all) updates is defined as follows. Derivable relations are simply recomputed for the target model tuple after a local update $u_i$. The case of non-derivable relations is more interesting. Suppose, for example, that \ptop\ is an independent relation, and a new person was added to, say, model $A_1$. Nothing changes in the correspondences as deciding whether this new person in $A'_1$ is identical to an existing person in $A_2$  cannot be done automatically in the absence of keys. If a person is deleted from $A_1$, and this person appeared in $\ptop^R$, then the \corring\ pair is to be deleted from $\ptop^R$ yielding an updated relation $\ptop'$.   
In a more refined setting, relation $\ptop^R$ can be encoded as a binary span between $A_1$ and $A_2$, and an update \frar{u_1}{A_1}{A'_1} is also a binary span (relation), cf.\ the introductory remarks in Sect.~\ref{sec:modelspaces}. Then realignment amounts to relation composition (denoted  by $\Join$): $\ptop'=\ptop^R\Join \restr{u_1}{\Person}$ where \restr{u_1}{\Person} is the part of the update affecting set $\Person^{A_1}$.
%
Two other correspondence relations, \ctoc\ and \etor, can be processed similarly, \eg, $\etor'=\etor^R\Join \restr{u_1}{\Empl}$. % only keeps in \etor\ those links that are kept by \restr{u_1}{\Empl}. 
Thus, we \hkmodok{obtain}{can automatically compute}{important!} the entire new correspondence $R'$ by defining  $\ptop^{R'}=\ptop'$, $\ctoc^{R'}=\ctoc'$, and $\etor^{R'}=\etor'$. Finally, we set $u_1^\bigstar(R)=R'$. Functoriality of $\_^\bigstar$ follows from the associativity of relational composition: the idea is given by the following schema 
	//
$(u_1;v_1)^\bigstar(R)=(u_1;v_1)\Join R= (u_1\Join v_1)\Join R=u_1\Join(v_1\Join R)=u_1^\bigstar(v_1^\bigstar(R))$. 
//
An accurate proof needs an accurate definition of all components, see \cite{DBLP:conf/ecmdafa/KonigD17} 
}{}{ALIGN}{-20em} %\qed

\par
\hkmodok{
Consistency is determined by intermodel constraints (C1-3) considered on p.~\pageref{pg:constr}, and the multimodel shown in \figref{fig:multimod-uml} is inconsistent. To make it consistent, 
% multimodel $(A_1A_2A_3, R)$ from that one shown in in , 
we can add, \eg,  to \ai\ an \eer-link connecting Mary to IBM, add to \aiii\ a commute with attributes $\from=a1$ and $\too=a15$, and relate it to John's and Mary's employment with IBM. %$\etor^{R'}=\{()\}form a corr-set $R=\{(p_1',p_2'),(c_1,c_2')\}$  (all other corr-links are derivable from this data).  
}{}{This piece seems to be misplaced here. Moreover, it is redundant (with parts of Chapt. 2)}
%\zd{To be completed with the alignment operations}
\end{example}

\endinput

%\subsection{Consistency and compatibility (to be polished)}
\begin{defin}[Consistency and compatibility]
	(i) For every model tuple \tupA, a subset $\Kcorr_{\tupA}\subset\tupA^\bigstar$ of {\em consistent} corrs is given. We thus have their union $\mspK^\bigstar\subset\mspA^\bigstar$.
	%
	%  -- multimodel version
	%(ii) For any two multimodels $\nia,\nia'$, a subset  $\Kpar_{\nia,\nia'}\subset \mspA(\nia,\nia')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%-- model tuple version
	(ii) For any two model tuples $\tupA,\tupA'$, a subset  $\Kpar_{\tupA,\tupA'}\subset \mspA^\Pi(\tupA,\tupA')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%
	(iii)  For any model tuple $\tupA$,  a subset 
	%we require every model space $\spaA$ to be endowed with a family 
	$\Kupd_{\tupA}\subset\mspA^\Pi(\_, \tupA)\timm\mspA^\Pi(\tupA, \_)$
	of {\em conseqcutively compatible} updates is defined: $(\tupu, \tupu')\in\Kupd_{\tupA}$ if $(u_i, u'_i) \in \Kupd_{A_i}$  for all $i$.
\end{defin}


==> sections/lensesFinal/multimodSpaces-last-new.tex <==
\subsection{Correspondences and Multimodels}
\zdmodtok{This is the newer non-functorial version of the section. To switch to the functorial one -- switch from multimodSpaces-last to multimodSpaces-new}{}{}
We will work with families of model spaces indexed by a finite set $I$, whose elements can be seen as space {\em names}. To simplify notation, we will assume that $I=\{1,\ldots,n\}$ \zdmoddno{although ordering will not play any role in our \fwk.}{}{Importantly!!}{-2ex} Given a tuple of model spaces $\spA_1, \ldots, \spA_n$, we will refer to objects and arrows of the product category $\prod\spA=\spaA_1\timm\cdots\timm\spaA_n$ as {\em tuple models}  and {\em tuple updates},  
%(sometimes, as {\em discrete multimodels /multiupdates},)
 and denote them by letters without indexes, \eg, \frar{\tupu}{\tupA}{\tupA'} is a family \frar{u_i}{A_i}{A'_i}, $i=1..n$.  
%For family of model spaces  $\spA=(\spA_1, \ldots, \spA_n)$, 
%An n-ary {\em alignment} \fwk\ %over \spA\ is a functor \frar{}{}{}
We will call components of tuple models and updates their {\em feet}. We also call elements of a particular space $\spA_i$ {\em foot} models and {\em foot} updates. %Another terminology we will also use is {\em foot} models and updates for elements of a particular space, and {\em feet} models and updates for elements of the product category, \ie, tuples. 

\zdmoddtok{For this paper, we are interested in a special class of tuple updates, whose all feet besides one are identities, \ie, updates of the type $(\id_{A_1}..u_i..\id_{A_n})$ for some $i\le n$; we will call such updates {\em singular}. % and denote the full subcategory of $\prod\spA$ consisting of singular updates by $\prosing\spA$. 
	%Given $i\le n$, we call an update \frar{u_i}{A_i}{A'_i} in space $\spA_i$ an $i${\em -update} for some given }{Important!}{-4em}
Given a tuple model $A=(A_1...A_n)$, any foot update \frar{u_i}{A_i}{A'_i} gives rise to a unique singular update \frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % in \prosing\spA, 
where $\ovr{A'_i}=(A_1..A'_i..A_n)$ and $\ovr{u_i}=(\id_{A_1}..u_i..\id_{A_n})$ (and any singular update is such). Note also that any tuple update $u=u_1...u_n$ can be represented as a sequential composition $\ovr{u_1}...\ovr{u_n}$ of singular updates (taken in any order). 
}{}{not sure but i seems we don;t need it}{-4em}



%\input{sections/lensesFinal/multispace-old}
%\input{sections/lensesFinal/multispace-total} see below
\begin{defin}[Multispaces, Alignment, Consistency]
\label{def:mspace}
	%Let $n\ge 2$ be a natural number. An {\em n-ary multi-space \zdmodtok{(with alignment)}{}{}} \mspA\ is a given by the following \zdmodtok{three}{two}{} components. The first one is a tuple of (wb) model spaces $\spA = (\spaA_1, \ldots, \spaA_n)$ called the {\em boundary} of \mspA\ (and denoted by \bounmspA\ if we need an explicit reference to the multispace). The second component is a functor
	Let $n\ge 2$ be a natural number. An {\em n-ary (wb) multi-space \zdmodtok{(with alignment)}{}{}} is a pair $(\spA, \corr)$, whose first component is a tuple of (wb) model spaces $\spA = (\spaA_1, \ldots, \spaA_n)$ called the {\em boundary} of \mspA\ (and denoted by \bounmspA\ if we need an explicit reference to the multispace). The second component is a functor
%$$	
\begin{equation}\label{eq:corr-fun}
		\frar{\corr{}}{\spaA_1\times\ldots\times\spaA_n}{\catcat}
\end{equation}
%$$
that assigns to every tuple of models $A=(A_1...A_n)\in \xob{\prod\!\spA}$ a category of {\em [consistent] correspondences ({\em or, shortly, {\em corrs}}) over $A$} and their {\em updates}. All categories \corrx{A} are assumed to be disjoint.%
%\footnote{\textcolor{blue}{Formally speaking, a mutlispace is just a functor \eqref{eq:corr-fun} and the multispace's boundary is nothing but the domain of the functor, but a strictly formal terminology may be too ``dried'' for talking in the applied context.}} 

A corr $R\in\xob{\corrx{A}}$ is understood as a correspondence specification interrelating models $A_i$. The latter are also called {\em R's feet} and denoted by $\prt_iR$; we say that models $A_i$ are {\em aligned} via $R$. To ease notation, we will often write $R\in\corrx{A}$ for $R\in\xob{\corrx{A}}$; we also write $\prt R$ for the tuple $(\prt_1R...\prt_nR)$.
%Will be said later {Although in this paper all corrs are considered consistent by default, we will often mention their consistency explicitly to recall the context.}

We  write $\int \corr$ or $\Corr$ for the class of all corrs $\coprod\compr{\corrx{A}}{A\in\xob{\prod\spA}}$, and 
%
$\Corrx{A_i}$ for the class $ \compr{R\in{\Corr}}{\prt_i R=A_i}$ of all corrs with a given foot $A_i\in\xob{\spA_i}$.

Although in this paper all corrs are considered consistent by default, we will often mention their consistency explicitly to recall the context and to ease comparison with similar but more general \fwk s, in which inconsistent corrs are also considered \cite{me-models11,me-jss15}. 

If %$u= (\frar{u_1}{A_1}{A'_1}, \ldots, \frar{u_n}{A_n}{A'_n})$ 
$u=(u_1,...,u_n)$ is a tuple of model updates \frar{u_i}{A_i}{A'_i}, $i=1..n$, then functor \frar{u_*\eqdef\corrx{u}}{\corrx{A}}{\corrx{A'}} is to be understood as a trivial realignment of corrs over $A$ to corrs over $A'$. A typical case is deletion of a correspondence link from $R\in\corrx{A}$ as soon as one of the components of the link is deleted by at least one of $u_i$, while additions of new elements by $u_i$ does not influence $R$ unless we compute corrs based on some reliable keys.  
\qed
\end{defin}
%%\subsubsection{Total category of corrs.} 
%\begin{defin}[Total category of corrs] Given a multispace as above, we construct the following category \Corr. Objects of \Corr\ are pairs $(A,R)$ with $A\in\xob{\prodx{\spA}}$ a tuple model and $R\in\corrx{A}$ a corr. Arrows from $(A,R)$ to $(A',R')$ are pairs $(u,r)$ with $\frar{u}{A}{A'} \in\xarr{\prod\spA}$ being a tuple update and \frar{r}{u_*(R)}{R'} a corr update in \corrx{A'}, where $u_*$ denotes the functor \frar{\corrx{u}}{\corrx{A}}{\corrx{A'}}. We then shortly write \frar{r}{R}{R'} and call it a {\em corr update}; the underlying feet update $u=(u_1...u_n)$ and its components $u_i$ are denoted by $\prt r$ and $\prt_i r$ resp. It is straightforward to check that \Corr\ is indeed a category with identity loops being pairs $(\id_A, \id_R)$, and the boundary mapping is a functor \frar{\prt}{\Corr}{\prod\!\spA}%
%\footnote{The above is just an instance of the well-known Grothendieck construction explained in any textbook on category theory, \eg, \cite{fiadeiroBook}. Functor $\prt$ is an opfibration with special properties, which can be shown is equivalent to functor \eqref{eq:corr-fun} in some precise sense, but we will not use this equivalence in this paper. }
%
%We will write %write $\int \corr$ or $\Corrx{\spA}$ for the class of all corrs $\coprod\compr{\corrx{A}}{A\in\xob{\prod\spA}}$, and 
%$\Corrx{A_i}$ for the class $ \compr{R\in\xob{\Corr}}{\prt_i R=A_i}$ of all corrs with a given foot $A_i\in\xob{\spA_i}$. 
%\end{defin}
%%
%Due to functoriality of $\msp\corr{A}$, the operation of realignment is fully determined by realignment caused by  singular updates: given $u=(u_1...u_n)$, $u^\bigstar=u^\bigstar_1;...;u^\bigstar_n$.

%	\zdmodtok{The third component of a multispace is a class of {\em consistent} corrs $\Korrsma\subset\Corrsa$. We write $\Kcorr_A$ for $\Korrsma\cap \corr{A}$ and $\Kcorr_{A_i}$ for $\Korrsma\cap \corr{A_i}$.}{}{}
%	\[ 
%	\comprfam{\Kcorr_A\subseteq \corr{A}}%
%	{{A=(A_1..A_n) \in \xob{(\prod\spA)}}} 
%	\]
% indexed by model tuples. %Note that for an update \end{defin}
%\zdmodtok{the new def above is in the section "lensesFinal/multimodSpaces-last" while the previuous functorial def is in section ".../multimodSpaces" or maybe ".../multimodSpaces-new".}{}{}
\begin{defin}[Multimodels]\label{def:mmodel}	
  A {\em (consistent) multimodel} over a multispace $(\spA, \corr)$ is a couple $\nia=(A, R)$ of a model tuple $\tupA=(A_1..A_n)$\ with a (consistent) corr $R\in\corrx{\tupA}$ relating the component models. %We then write $\nia\in\mspA$ although this is a more complex relation than set membership. \zdmodtok{A model is {\em consistent} if the corr $R$ is consistent.}{}{}
\zdmodno{A {\em multimodel update} \frar{\mathcal{u}}{\nia}{\nia'} is a pair $(u,r)$ with 
	%$u= (\frar{u_1}{A_1}{A'_1}, \ldots, \frar{u_n}{A_n}{A'_n})$ 
	\frar{u}{A}{A'} a tuple of feet model updates and \frar{r}{u_*(R)}{R'} is a corr update in category $\corrx{A'}$; we will write the latter shortly as \frar{r}{R}{R'}.  
	We also write $\prt \mathcal{u}$ for $u$ and $\prt_i \mathcal{u}$ for $u_i$.  
	
It is straightforward to check that maultimodels and their updates make a category (denoted by \mspA)  with identity loops being pairs $(\id_A, \id_R)$, and the boundary mapping is a functor \frar{\prt}{\mspA}{\prod\!\spA}.%
\footnote{The above is just an instance of the well-known Grothendieck construction explained in any textbook on category theory, \eg, \cite{fiadeiroBook}. Functor $\prt$ is an opfibration with special properties, which can be shown is equivalent to functor \eqref{eq:corr-fun} in some precise sense, but we will not use this equivalence in this paper.}
}{}{}
	\qed
\end{defin}
Note that any corr $R$ uniquely defines a multimodel via the corr's boundary function.
\zd{The above should be written as a general remark about the notation and terminolofy when having a function \frar{f}{X}{Y}, we say ``having a pair $(x,f)$''}%	
	%Obviously, multimodels and their updates form a category denoted by $\mspA^\#$. As a rule, we will omit the superindex thus denoting the multispace and the category it generates by the same symbol \mspA\ relying on the context to resolve ambiguity. %Normally, the context will suggest what the symbol means and, thus, \xob{\mspA} denotes the set of all multimodels and $\mspA(\tupA,\tupA')$ is the respective hom-set. 	As equality $\xstar{\tupu}(R)=R'$ is not required for multimodel updates, we have $\mspA^\#(\nia,\nia')=\mspA^\Pi(\prt\nia,\prt\nia')$

%\exIntro\ 
\begin{example}
The \exIntro\ of Sect.\ref{sec:example} %, the tuple $\spA_{1,2,3}$ 
gives rise to a 3-ary multimodel space. For $i=1..3$, space $\spA_i$ consists of all models instantiating metamodel $M_i$ in  Fig.\ref{fig:multiMetamod-uml} and their updates. Given a model tuple $A=(A_1, A_2, A_3)$, a consistent corr $R\in \corrx{A}$ is given by a triple of relations: $\ptop^R, \ctoc^R, \etor^R$  described in \riii, \rii\
on p.~\pageref{pg:constr} such that the intermodel constraints (C1-3) are satisfied.
%R=(R_\Person, R_\Company, R_\Route)$, where $R_\Person\subset \Person^{A_1}\timm\Person^{A_2}$, $R_\Company\subset \Company^{A_1}\timm\Company^{A_2}$ and $R_\Route \subset \Route^{\ai{*}\aii}\times \Route^\aiii$ (see p.~\pageref{pg:constr} for the definition of $\Route^{\ai{*}\aii}$).  
If we rely on person and company names as keys, then relations $\ptop^R$, $\ctoc^R$ are derived from foot models $A_1$ and $A_2$, but if these keys are not reliable, then the two relations are independent components of the multimodel. Relation $\etor^R$ is always an independent component. 

\zdmoddtok{
Realignment (for foot, and hence all) updates is defined as follows. Derivable relations are simply recomputed for the target model tuple after a local update $u_i$. The case of non-derivable relations is more interesting. Suppose, for example, that \ptop\ is an independent relation, and a new person was added to, say, model $A_1$. Nothing changes in the correspondences as deciding whether this new person in $A'_1$ is identical to an existing person in $A_2$  cannot be done automatically in the absence of keys. If a person is deleted from $A_1$, and this person appeared in $\ptop^R$, then the \corring\ pair is to be deleted from $\ptop^R$ yielding an updated relation $\ptop'$.   
In a more refined setting, relation $\ptop^R$ can be encoded as a binary span between $A_1$ and $A_2$, and an update \frar{u_1}{A_1}{A'_1} is also a binary span (relation), cf.\ the introductory remarks in Sect.~\ref{sec:modelspaces}. Then realignment amounts to relation composition (denoted  by $\Join$): $\ptop'=\ptop^R\Join \restr{u_1}{\Person}$ where \restr{u_1}{\Person} is the part of the update affecting set $\Person^{A_1}$.
%
Two other correspondence relations, \ctoc\ and \etor, can be processed similarly, \eg, $\etor'=\etor^R\Join \restr{u_1}{\Empl}$. % only keeps in \etor\ those links that are kept by \restr{u_1}{\Empl}. 
Thus, we \hkmodok{obtain}{can automatically compute}{important!} the entire new correspondence $R'$ by defining  $\ptop^{R'}=\ptop'$, $\ctoc^{R'}=\ctoc'$, and $\etor^{R'}=\etor'$. Finally, we set $u_1^\bigstar(R)=R'$. Functoriality of $\_^\bigstar$ follows from the associativity of relational composition: the idea is given by the following schema 
	//
$(u_1;v_1)^\bigstar(R)=(u_1;v_1)\Join R= (u_1\Join v_1)\Join R=u_1\Join(v_1\Join R)=u_1^\bigstar(v_1^\bigstar(R))$. 
//
An accurate proof needs an accurate definition of all components, see \cite{DBLP:conf/ecmdafa/KonigD17} 
}{}{ALIGN}{-20em} %\qed

\par
\hkmodok{
Consistency is determined by intermodel constraints (C1-3) considered on p.~\pageref{pg:constr}, and the multimodel shown in \figref{fig:multimod-uml} is inconsistent. To make it consistent, 
% multimodel $(A_1A_2A_3, R)$ from that one shown in in , 
we can add, \eg,  to \ai\ an \eer-link connecting Mary to IBM, add to \aiii\ a commute with attributes $\from=a1$ and $\too=a15$, and relate it to John's and Mary's employment with IBM. %$\etor^{R'}=\{()\}form a corr-set $R=\{(p_1',p_2'),(c_1,c_2')\}$  (all other corr-links are derivable from this data).  
}{}{This piece seems to be misplaced here. Moreover, it is redundant (with parts of Chapt. 2)}
%\zd{To be completed with the alignment operations}
\end{example}

\endinput

%\subsection{Consistency and compatibility (to be polished)}
\begin{defin}[Consistency and compatibility]
	(i) For every model tuple \tupA, a subset $\Kcorr_{\tupA}\subset\corr{\tupA}$ of {\em consistent} corrs is given. We thus have their union $\mspK^\bigstar\subset\mspA^\bigstar$.
	%
	%  -- multimodel version
	%(ii) For any two multimodels $\nia,\nia'$, a subset  $\Kpar_{\nia,\nia'}\subset \mspA(\nia,\nia')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%-- model tuple version
	(ii) For any two model tuples $\tupA,\tupA'$, a subset  $\Kpar_{\tupA,\tupA'}\subset \mspA^\Pi(\tupA,\tupA')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%
	(iii)  For any model tuple $\tupA$,  a subset 
	%we require every model space $\spaA$ to be endowed with a family 
	$\Kupd_{\tupA}\subset\mspA^\Pi(\_, \tupA)\timm\mspA^\Pi(\tupA, \_)$
	of {\em conseqcutively compatible} updates is defined: $(\tupu, \tupu')\in\Kupd_{\tupA}$ if $(u_i, u'_i) \in \Kupd_{A_i}$  for all $i$.
\end{defin}


==> sections/lensesFinal/multimodSpaces-new.tex <==
\subsection{Correspondences and Multimodels}
\zd{This is an earlier version of the section with (i) corrs are a functor and (ii) consistent corrs are a subclass K. To switch to the new -- switch from multimodSpaces-new to multimodSpaces-Newest}
We will work with families of model spaces indexed by a finite set $I$, whose elements can be seen as space {\em names}. To simplify notation, we will assume that $I=\{1,\ldots,n\}$ \zdmoddno{although ordering will not play any role in our \fwk.}{}{Importantly!!}{-2ex} Given a tuple of model spaces $\spA_1, \ldots, \spA_n$, we will refer to objects and arrows of the product category $\prod\spA=\spaA_1\timm\cdots\timm\spaA_n$ as {\em tuple models}  and {\em tuple updates},  
%(sometimes, as {\em discrete multimodels /multiupdates},)
 and denote them by italic letters without indexes, \eg, \frar{\tupu}{\tupA}{\tupA'} is a family \frar{u_i}{A_i}{A'_i}, $i=1..n$.  
%For family of model spaces  $\spA=(\spA_1, \ldots, \spA_n)$, 
%An n-ary {\em alignment} \fwk\ %over \spA\ is a functor \frar{}{}{}
We will call components of tuple models and updates their {\em feet}. We also call elements of a particular space $\spA_i$ {\em foot} models and {\em foot} updates. %Another terminology we will also use is {\em foot} models and updates for elements of a particular space, and {\em feet} models and updates for elements of the product category, \ie, tuples. 

For this paper, we are interested in a special class of tuple updates, whose all feet besides one are identities, \ie, updates of the type $(\id_{A_1}..u_i..\id_{A_n})$ for some $i\le n$; we will call such updates {\em singular}. % and denote the full subcategory of $\prod\spA$ consisting of singular updates by $\prosing\spA$. 
	%Given $i\le n$, we call an update \frar{u_i}{A_i}{A'_i} in space $\spA_i$ an $i${\em -update} for some given }{Important!}{-4em}
Given a tuple model $A=(A_1...A_n)$, any foot update \frar{u_i}{A_i}{A'_i} gives rise to a unique singular update \frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % in \prosing\spA, 
where $\ovr{A'_i}=(A_1..A'_i..A_n)$ and $\ovr{u_i}=(\id_{A_1}..u_i..\id_{A_n})$ (and any singular update is such). Note also that any tuple update $u=u_1...u_n$ can be represented as a sequential composition $\ovr{u_1}...\ovr{u_n}$ of singular updates (taken in any order). 

%\input{sections/lensesFinal/multispace-old}
%\input{sections/lensesFinal/multispace-total} see below
\begin{defin}[Multispaces, Alignment, Consistency]
\label{def:mspace}
	Let $n\ge 2$ be a natural number. An {\em n-ary multi-space (with alignment)} \mspA\ is a given by the following three components. The first one is a tuple of model spaces $\spA = (\spaA_1, \ldots, \spaA_n)$ called the {\em boundary} of \mspA\ and denoted by \bounmspA. The second component is a functor 
	%\[\frar{{\_}^\bigstar_{\mspaA}}{\prodmspA}{\setcat}\]
	%where \prodmspA\ denotes the category 
	%$\prod\bounmspA =\spaA_1\timm\ldots\timm\spA_n$. We will omit the subindex $\__\mspA$ if it is clear from the context. 
	%
		\[\frar{\mspA^\bigstar}{\prosing\spA}{\setcat}\]
		such that all sets $\mspA^\bigstar(A)$, $A=(A_1..A_n) \inn \xob{(\prod\spA)}$, are disjoint.
	 To simplify notation, given an update %\frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % 
	 \frar{u}{A}{A'}
	 from a model tuple $A=(A_1..A_n)$ to a model tuple $A'=(A'_1..A'_n)$, 
	 we will write $A^\bigstar$ for the set $\mspA^\bigstar(A)$, and \frar{u^\bigstar}{A^\bigstar}{A'^\bigstar} %{\ovr{A'_i}^\bigstar}
	  for the function $\mspA^\bigstar(u)$. 
	 Analogously, given a tuple model $A$ and a foot update \frar{u_i}{A_i}{A'_i}, function $\ovr{u_i}^\bigstar$ is denoted by $u_i^\bigstar$.	%\zd{so, i decided to keep the notation used in the Fase paper for consistency of the two papers, but in the present one we will use the simplified variant}
	
	Given a model tuple $\tupA = (A_1..A_n)$, elements of the set $ \xstar{\tupA}$ are called {\em \corrce s} or just {\em corrs} over \tupA. Intuitively, a corr $R\in\xstar{\tupA}$ is understood as a correspondence specification interrelating models $A_i$; we will also say that the latter are {\em aligned} via $R$, and that \tupA\ is the {\em boundary} of $R$ and we write $\tupA=\prt R$ (recall the disjointness condition above). A foot update \frar{u_i}{A_i}{A'_i} creates a new corr $R'=u_i^\bigstar(R)\in \ovr{A'_i}^\bigstar$ called the {\em realignment} of the model $(A,R)$.Due to functoriality of $\mspA^\bigstar$, the operation of realignment is fully determined by realignment caused by  singular updates: given $u=(u_1...u_n)$, $u^\bigstar=u^\bigstar_1;...;u^\bigstar_n$.

	The third component is a family of {\em consistent} corr sets %
	\[ 
	\comprfam{\Kcorr_A\subseteq A^\bigstar}%
	{{A=(A_1..A_n) \in \xob{(\prod\spA)}}} 
	\]
 indexed by model tuples. Note that for an update \frar{u_i}{A_i}{A'_i} and a corr $R\in \Kcorr_A$, we do not require its realignment $R'=u_i^\bigstar(R)$ to be necessary consistent, \ie, it may happen that $R'\notin \Kcorr_{A'}$ and thus consistency restoration is needed. 
 \par	
We will write $\spA^\bigstar$ for the class of all corrs, $\Kcorr_\spA$ for its subclass of consistent corrs and, for a given model $A_i\in\xob{\spA_i}$, $A_i^\bigstar\eqdef \compr{R\in\spA^\bigstar}{\prt_i R=A}$ for the class of all corrs with a fixed foot $A_i\in \xob{\spA_i}$ and $\Kcorr_{A_i}\subset A_i^\bigstar$ for the subclass of all such consistent corrs. 
\qed
\end{defin}
\begin{defin}[Multimodels]\label{def:mmodel}	
  An {\em (aligned) multimodel} over a multispace \mspA\ is a couple $\nia=(A, R)$ of a model tuple $\tupA=(A_1..A_n)$\ with a corr $R\in\xstar{\tupA}$ relating the component models. We then write $\nia\in\mspA$ although this is a more complex relation than set membership. A model is {\em consistent} if the corr $R$ is consistent.
%A {\em multimodel update} \frar{\tupu}{\nia}{\nia'} is a tuple of updates (\frar{u_1}{A_1}{A'_1}, \ldots, \frar{u_n}{A_n}{A'_n}). Equality $\xstar{\tupu}(R)=R'$ is not required.

\zdmoddok{For a given model $\nia=(A,R)$, any foot update \frar{u_i}{A_i}{A'_i} (we will also say {\em local} update) gives rise to a ({\em global}) feet update  $\ovr{u_i}=(\id_{A_1}...u_i...\id_{A_n})$, and we write $u_i^\bigstar(R)$ for the corr $R'\eqdef \ovr{u_i}^\bigstar(R)\in A'^\bigstar$ where $A'=(A_1,..,A_{i-1}, A'_i, A_{i+1}, ..,A_n)$. Again, if even $R$ is consistent, its realignment $R'$ may be inconsistent, and then we say that update $u_i$ destroyed the consistency of model \nia.}{}{it seems it's just a repetition}{-4em}
Note that any corr $R$ uniquely defines a multimodel via the corr's boundary function.
%	
	%Obviously, multimodels and their updates form a category denoted by $\mspA^\#$. As a rule, we will omit the superindex thus denoting the multispace and the category it generates by the same symbol \mspA\ relying on the context to resolve ambiguity. %Normally, the context will suggest what the symbol means and, thus, \xob{\mspA} denotes the set of all multimodels and $\mspA(\tupA,\tupA')$ is the respective hom-set. 	As equality $\xstar{\tupu}(R)=R'$ is not required for multimodel updates, we have $\mspA^\#(\nia,\nia')=\mspA^\Pi(\prt\nia,\prt\nia')$
	\qed
\end{defin}
%\exIntro\ 
\begin{example}
The \exIntro\ of Sect.\ref{sec:example} %, the tuple $\spA_{1,2,3}$ 
gives rise to a 3-ary multimodel space. For $i\le3$, space $\spA_i$ consists of all models instantiating metamodel $M_i$ in  Fig.\ref{fig:multiMetamod-uml} and their updates. Given a model tuple $A=(A_1, A_2, A_3)$, a corr $R\in A^\bigstar$ is given by a triple of relations: $\ptop^R, \ctoc^R, \etor^R$ as described in \riii, \rii\
on p.~\pageref{pg:constr}. 
%R=(R_\Person, R_\Company, R_\Route)$, where $R_\Person\subset \Person^{A_1}\timm\Person^{A_2}$, $R_\Company\subset \Company^{A_1}\timm\Company^{A_2}$ and $R_\Route \subset \Route^{\ai{*}\aii}\times \Route^\aiii$ (see p.~\pageref{pg:constr} for the definition of $\Route^{\ai{*}\aii}$).  
If we rely on person and company names as keys, then relations $\ptop^R$, $\ctoc^R$ are derived from foot models $A_1$ and $A_2$, but if these keys are not reliable, then the two relations are independent components of the multimodel. Relation $\etor^R$ is always an independent component. 

Realignment (for foot, and hence all) updates is defined as follows. Derivable relations are simply recomputed for the target model tuple after a local update $u_i$. The case of non-derivable relations is more interesting. Suppose, for example, that \ptop\ is an independent relation, and a new person was added to, say, model $A_1$. Nothing changes in the correspondences as deciding whether this new person in $A'_1$ is identical to an existing person in $A_2$  cannot be done automatically in the absence of keys. If a person is deleted from $A_1$, and this person appeared in $\ptop^R$, then the \corring\ pair is to be deleted from $\ptop^R$ yielding an updated relation $\ptop'$.   
\hkmodok{}{In a more refined setting, relation $\ptop^R$ can be encoded as a binary span between $A_1$ and $A_2$, and an update \frar{u_1}{A_1}{A'_1} is also a binary span (relation), cf.\ the introductory remarks in Sect.~\ref{sec:modelspaces}. Then realignment amounts to relation composition (denoted  by $\Join$): $\ptop'=\ptop^R\Join \restr{u_1}{\Person}$ where \restr{u_1}{\Person} is the part of the update affecting set $\Person^{A_1}$.}{Now referring to the place where we mention the span category}
Two other correspondence relations, \ctoc\ and \etor, can be processed similarly, \eg, $\etor'=\etor^R\Join \restr{u_1}{\Empl}$. % only keeps in \etor\ those links that are kept by \restr{u_1}{\Empl}. 
Thus, we \hkmodok{obtain}{can automatically compute}{important!} the entire new correspondence $R'$ by defining  $\ptop^{R'}=\ptop'$, $\ctoc^{R'}=\ctoc'$, and $\etor^{R'}=\etor'$. Finally, we set $u_1^\bigstar(R)=R'$. Functoriality of $\_^\bigstar$ follows from the associativity of relational composition: the idea is given by the following schema 
$$(u_1;v_1)^\bigstar(R)=(u_1;v_1)\Join R= (u_1\Join v_1)\Join R=u_1\Join(v_1\Join R)=u_1^\bigstar(v_1^\bigstar(R)).$$ 
An accurate proof needs an accurate definition of all components, see \cite{DBLP:conf/ecmdafa/KonigD17} \qed
\par
\hkmodok{
Consistency is determined by intermodel constraints (C1-3) considered on p.~\pageref{pg:constr}, and the multimodel shown in \figref{fig:multimod-uml} is inconsistent. To make it consistent, 
% multimodel $(A_1A_2A_3, R)$ from that one shown in in , 
we can add, \eg,  to \ai\ an \eer-link connecting Mary to IBM, add to \aiii\ a commute with attributes $\from=a1$ and $\too=a15$, and relate it to John's and Mary's employment with IBM. %$\etor^{R'}=\{()\}form a corr-set $R=\{(p_1',p_2'),(c_1,c_2')\}$  (all other corr-links are derivable from this data).  
}{}{This piece seems to be misplaced here. Moreover, it is redundant (with parts of Chapt. 2)}
%\zd{To be completed with the alignment operations}
\end{example}

\endinput

%\subsection{Consistency and compatibility (to be polished)}
\begin{defin}[Consistency and compatibility]
	(i) For every model tuple \tupA, a subset $\Kcorr_{\tupA}\subset\tupA^\bigstar$ of {\em consistent} corrs is given. We thus have their union $\mspK^\bigstar\subset\mspA^\bigstar$.
	%
	%  -- multimodel version
	%(ii) For any two multimodels $\nia,\nia'$, a subset  $\Kpar_{\nia,\nia'}\subset \mspA(\nia,\nia')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%-- model tuple version
	(ii) For any two model tuples $\tupA,\tupA'$, a subset  $\Kpar_{\tupA,\tupA'}\subset \mspA^\Pi(\tupA,\tupA')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%
	(iii)  For any model tuple $\tupA$,  a subset 
	%we require every model space $\spaA$ to be endowed with a family 
	$\Kupd_{\tupA}\subset\mspA^\Pi(\_, \tupA)\timm\mspA^\Pi(\tupA, \_)$
	of {\em conseqcutively compatible} updates is defined: $(\tupu, \tupu')\in\Kupd_{\tupA}$ if $(u_i, u'_i) \in \Kupd_{A_i}$  for all $i$.
\end{defin}


==> sections/lensesFinal/multimodSpaces.tex <==
\subsection{Correspondences and Multimodels}
We will work with families of model spaces indexed by a finite set $I$, whose elements can be seen as space {\em names}. To simplify notation, we will assume that $I=\{1,\ldots,n\}$ \zdmoddno{although ordering will not play any role in our \fwk.}{}{Importantly!!}{-2ex} Given a tuple of model spaces $\spA_1, \ldots, \spA_n$, we will refer to objects and arrows of the product category $\prod\spA=\spaA_1\timm\cdots\timm\spaA_n$ as {\em tuple models}  and {\em tuple updates},  
%(sometimes, as {\em discrete multimodels /multiupdates},)
 and denote them by italic letters without indexes, \eg, \frar{\tupu}{\tupA}{\tupA'} is a family \frar{u_i}{A_i}{A'_i}, $i=1..n$.  
%For family of model spaces  $\spA=(\spA_1, \ldots, \spA_n)$, 
%An n-ary {\em alignment} \fwk\ %over \spA\ is a functor \frar{}{}{}
We will call components of tuple models and updates their {\em feet}. We also call elements of a particular space $\spA_i$ {\em foot} models and {\em foot} updates. %Another terminology we will also use is {\em foot} models and updates for elements of a particular space, and {\em feet} models and updates for elements of the product category, \ie, tuples. 

For this paper, we are interested in a special class of tuple updates, whose all feet besides one are identities, \ie, updates of the type $(\id_{A_1}..u_i..\id_{A_n})$ for some $i\le n$; we will call such updates {\em singular}. % and denote the full subcategory of $\prod\spA$ consisting of singular updates by $\prosing\spA$. 
	%Given $i\le n$, we call an update \frar{u_i}{A_i}{A'_i} in space $\spA_i$ an $i${\em -update} for some given }{Important!}{-4em}
Given a tuple model $A=(A_1...A_n)$, any foot update \frar{u_i}{A_i}{A'_i} gives rise to a unique singular update \frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % in \prosing\spA, 
where $\ovr{A'_i}=(A_1..A'_i..A_n)$ and $\ovr{u_i}=(\id_{A_1}..u_i..\id_{A_n})$ (and any singular update is such). Note also that any tuple update $u=u_1...u_n$ can be represented as a sequential composition $\ovr{u_1}...\ovr{u_n}$ of singular updates (taken in any order). 

%\input{sections/lensesFinal/multispace-old}
%\input{sections/lensesFinal/multispace-total} see below
\begin{defin}[Multispaces, Alignment, Consistency]
\label{def:mspace}
	Let $n\ge 2$ be a natural number. An {\em n-ary multi-space (with alignment)} \mspA\ is a given by the following three components. The first one is a tuple of model spaces $\spA = (\spaA_1, \ldots, \spaA_n)$ called the {\em boundary} of \mspA\ and denoted by \bounmspA. The second component is a functor 
	%\[\frar{{\_}^\bigstar_{\mspaA}}{\prodmspA}{\setcat}\]
	%where \prodmspA\ denotes the category 
	%$\prod\bounmspA =\spaA_1\timm\ldots\timm\spA_n$. We will omit the subindex $\__\mspA$ if it is clear from the context. 
	%
		\[\frar{\mspA^\bigstar}{\prosing\spA}{\setcat}\]
		such that all sets $\mspA^\bigstar(A)$, $A=(A_1..A_n) \inn \xob{(\prod\spA)}$, are disjoint.
	 To simplify notation, given an update %\frar{\ovr{u_i}}{A}{\ovr{A'_i}}, % 
	 \frar{u}{A}{A'}
	 from a model tuple $A=(A_1..A_n)$ to a model tuple $A'=(A'_1..A'_n)$, 
	 we will write $A^\bigstar$ for the set $\mspA^\bigstar(A)$, and \frar{u^\bigstar}{A^\bigstar}{A'^\bigstar} %{\ovr{A'_i}^\bigstar}
	  for the function $\mspA^\bigstar(u)$. 
	 Analogously, given a tuple model $A$ and a foot update \frar{u_i}{A_i}{A'_i}, function $\ovr{u_i}^\bigstar$ is denoted by $u_i^\bigstar$.	%\zd{so, i decided to keep the notation used in the Fase paper for consistency of the two papers, but in the present one we will use the simplified variant}
	
	Given a model tuple $\tupA = (A_1..A_n)$, elements of the set $ \xstar{\tupA}$ are called {\em \corrce s} or just {\em corrs} over \tupA. Intuitively, a corr $R\in\xstar{\tupA}$ is understood as a correspondence specification interrelating models $A_i$; we will also say that the latter are {\em aligned} via $R$, and that \tupA\ is the {\em boundary} of $R$ and we write $\tupA=\prt R$ (recall the disjointness condition above). A foot update \frar{u_i}{A_i}{A'_i} creates a new corr $R'=u_i^\bigstar(R)\in \ovr{A'_i}^\bigstar$ called the {\em realignment} of the model $(A,R)$.Due to functoriality of $\mspA^\bigstar$, the operation of realignment is fully determined by realignment caused by  singular updates: given $u=(u_1...u_n)$, $u^\bigstar=u^\bigstar_1;...;u^\bigstar_n$.

	The third component is a family of {\em consistent} corr sets %
	\[ 
	\comprfam{\Kcorr_A\subseteq A^\bigstar}%
	{{A=(A_1..A_n) \in \xob{(\prod\spA)}}} 
	\]
 indexed by model tuples. Note that for an update \frar{u_i}{A_i}{A'_i} and a corr $R\in \Kcorr_A$, we do not require its realignment $R'=u_i^\bigstar(R)$ to be necessary consistent, \ie, it may happen that $R'\notin \Kcorr_{A'}$ and thus consistency restoration is needed. 
 \par	
We will write $\spA^\bigstar$ for the class of all corrs, $\Kcorr_\spA$ for its subclass of consistent corrs and, for a given model $A_i\in\xob{\spA_i}$, $A_i^\bigstar\eqdef \compr{R\in\spA^\bigstar}{\prt_i R=A}$ for the class of all corrs with a fixed foot $A_i\in \xob{\spA_i}$ and $\Kcorr_{A_i}\subset A_i^\bigstar$ for the subclass of all such consistent corrs. 
\qed
\end{defin}
\begin{defin}[Multimodels]\label{def:mmodel}	
  An {\em (aligned) multimodel} over a multispace \mspA\ is a couple $\nia=(A, R)$ of a model tuple $\tupA=(A_1..A_n)$\ with a corr $R\in\xstar{\tupA}$ relating the component models. We then write $\nia\in\mspA$ although this is a more complex relation than set membership. A model is {\em consistent} if the corr $R$ is consistent.
%A {\em multimodel update} \frar{\tupu}{\nia}{\nia'} is a tuple of updates (\frar{u_1}{A_1}{A'_1}, \ldots, \frar{u_n}{A_n}{A'_n}). Equality $\xstar{\tupu}(R)=R'$ is not required.

\zdmoddok{For a given model $\nia=(A,R)$, any foot update \frar{u_i}{A_i}{A'_i} (we will also say {\em local} update) gives rise to a ({\em global}) feet update  $\ovr{u_i}=(\id_{A_1}...u_i...\id_{A_n})$, and we write $u_i^\bigstar(R)$ for the corr $R'\eqdef \ovr{u_i}^\bigstar(R)\in A'^\bigstar$ where $A'=(A_1,..,A_{i-1}, A'_i, A_{i+1}, ..,A_n)$. Again, if even $R$ is consistent, its realignment $R'$ may be inconsistent, and then we say that update $u_i$ destroyed the consistency of model \nia.}{}{it seems it's just a repetition}{-4em}
Note that any corr $R$ uniquely defines a multimodel via the corr's boundary function.
%	
	%Obviously, multimodels and their updates form a category denoted by $\mspA^\#$. As a rule, we will omit the superindex thus denoting the multispace and the category it generates by the same symbol \mspA\ relying on the context to resolve ambiguity. %Normally, the context will suggest what the symbol means and, thus, \xob{\mspA} denotes the set of all multimodels and $\mspA(\tupA,\tupA')$ is the respective hom-set. 	As equality $\xstar{\tupu}(R)=R'$ is not required for multimodel updates, we have $\mspA^\#(\nia,\nia')=\mspA^\Pi(\prt\nia,\prt\nia')$
	\qed
\end{defin}
%\exIntro\ 
\begin{example}
The \exIntro\ of Sect.\ref{sec:example} %, the tuple $\spA_{1,2,3}$ 
gives rise to a 3-ary multimodel space. For $i\le3$, space $\spA_i$ consists of all models instantiating metamodel $M_i$ in  Fig.\ref{fig:multiMetamod-uml} and their updates. Given a model tuple $A=(A_1, A_2, A_3)$, a corr $R\in A^\bigstar$ is given by a triple of relations: $\ptop^R, \ctoc^R, \etor^R$ as described in \riii, \rii\
on p.~\pageref{pg:constr}. 
%R=(R_\Person, R_\Company, R_\Route)$, where $R_\Person\subset \Person^{A_1}\timm\Person^{A_2}$, $R_\Company\subset \Company^{A_1}\timm\Company^{A_2}$ and $R_\Route \subset \Route^{\ai{*}\aii}\times \Route^\aiii$ (see p.~\pageref{pg:constr} for the definition of $\Route^{\ai{*}\aii}$).  
If we rely on person and company names as keys, then relations $\ptop^R$, $\ctoc^R$ are derived from foot models $A_1$ and $A_2$, but if these keys are not reliable, then the two relations are independent components of the multimodel. Relation $\etor^R$ is always an independent component. 

\zdmodd{
Realignment (for foot, and hence all) updates is defined as follows. Derivable relations are simply recomputed for the target model tuple after a local update $u_i$. The case of non-derivable relations is more interesting. Suppose, for example, that \ptop\ is an independent relation, and a new person was added to, say, model $A_1$. Nothing changes in the correspondences as deciding whether this new person in $A'_1$ is identical to an existing person in $A_2$  cannot be done automatically in the absence of keys. If a person is deleted from $A_1$, and this person appeared in $\ptop^R$, then the \corring\ pair is to be deleted from $\ptop^R$ yielding an updated relation $\ptop'$.   
In a more refined setting, relation $\ptop^R$ can be encoded as a binary span between $A_1$ and $A_2$, and an update \frar{u_1}{A_1}{A'_1} is also a binary span (relation), cf.\ the introductory remarks in Sect.~\ref{sec:modelspaces}. Then realignment amounts to relation composition (denoted  by $\Join$): $\ptop'=\ptop^R\Join \restr{u_1}{\Person}$ where \restr{u_1}{\Person} is the part of the update affecting set $\Person^{A_1}$.
%
Two other correspondence relations, \ctoc\ and \etor, can be processed similarly, \eg, $\etor'=\etor^R\Join \restr{u_1}{\Empl}$. % only keeps in \etor\ those links that are kept by \restr{u_1}{\Empl}. 
Thus, we \hkmodok{obtain}{can automatically compute}{important!} the entire new correspondence $R'$ by defining  $\ptop^{R'}=\ptop'$, $\ctoc^{R'}=\ctoc'$, and $\etor^{R'}=\etor'$. Finally, we set $u_1^\bigstar(R)=R'$. Functoriality of $\_^\bigstar$ follows from the associativity of relational composition: the idea is given by the following schema 
	//
$(u_1;v_1)^\bigstar(R)=(u_1;v_1)\Join R= (u_1\Join v_1)\Join R=u_1\Join(v_1\Join R)=u_1^\bigstar(v_1^\bigstar(R))$. 
//
An accurate proof needs an accurate definition of all components, see \cite{DBLP:conf/ecmdafa/KonigD17} 
}{}{ALIGN}{-20em} %\qed

\par
\hkmodok{
Consistency is determined by intermodel constraints (C1-3) considered on p.~\pageref{pg:constr}, and the multimodel shown in \figref{fig:multimod-uml} is inconsistent. To make it consistent, 
% multimodel $(A_1A_2A_3, R)$ from that one shown in in , 
we can add, \eg,  to \ai\ an \eer-link connecting Mary to IBM, add to \aiii\ a commute with attributes $\from=a1$ and $\too=a15$, and relate it to John's and Mary's employment with IBM. %$\etor^{R'}=\{()\}form a corr-set $R=\{(p_1',p_2'),(c_1,c_2')\}$  (all other corr-links are derivable from this data).  
}{}{This piece seems to be misplaced here. Moreover, it is redundant (with parts of Chapt. 2)}
%\zd{To be completed with the alignment operations}
\end{example}

\endinput

%\subsection{Consistency and compatibility (to be polished)}
\begin{defin}[Consistency and compatibility]
	(i) For every model tuple \tupA, a subset $\Kcorr_{\tupA}\subset\tupA^\bigstar$ of {\em consistent} corrs is given. We thus have their union $\mspK^\bigstar\subset\mspA^\bigstar$.
	%
	%  -- multimodel version
	%(ii) For any two multimodels $\nia,\nia'$, a subset  $\Kpar_{\nia,\nia'}\subset \mspA(\nia,\nia')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%-- model tuple version
	(ii) For any two model tuples $\tupA,\tupA'$, a subset  $\Kpar_{\tupA,\tupA'}\subset \mspA^\Pi(\tupA,\tupA')$ of {\em conflict-free} or {\em concurrently compatible} updates is given.
	%
	(iii)  For any model tuple $\tupA$,  a subset 
	%we require every model space $\spaA$ to be endowed with a family 
	$\Kupd_{\tupA}\subset\mspA^\Pi(\_, \tupA)\timm\mspA^\Pi(\tupA, \_)$
	of {\em conseqcutively compatible} updates is defined: $(\tupu, \tupu')\in\Kupd_{\tupA}$ if $(u_i, u'_i) \in \Kupd_{A_i}$  for all $i$.
\end{defin}


==> sections/lensesFinal/multispace-old.tex <==
\begin{mydefin}[Model and Update Tuples]\label{def:modelTupleUpdTuple}
A family $(A_1, \ldots, A_n) \in \xob{\spA_1}\times \cdots \times \xob{\spA_n}$ is called a {\em model tuple} (or sometimes a {\em discrete} multimodel). Given two tuples $(A_1, \ldots, A_n)$ and $(A_1', \ldots, A_n')$ and updates \frar{u_i}{A_i}{A_i'} of $\xupd{\spaA_i}$, resp., $(u_1, \ldots, u_n)$ is called an {\em update tuple}\footnote{
By the definition of cartesian product of categories, the collection of all update tuple is the same as $\xupd{\spaA_1\times \cdots\times \spaA_n}$.
}.\qed
\end{mydefin}

{\color{blue}Next para may be moved}\\ 
Assume $n=2$ for the moment, \ie, there are two model spaces \spaA\ and \spaB. E.g., \spaA\ may encompass all possible object structures that conform to a fixed class diagram and \spaB\ contains all object structures that conform to a second fixed class diagram. A different example is, if \spaA\ is a set of UML class diagrams and \spaB\ is a set of relational schemas. A pair $(A,B)$ of interrelated models normally comes with a traceability mapping so that our typical situation to consider is a triple $(A,R,B)$ with $A$ a model from \spaA, $B$ a model from \spaB, and $R$ some specification of correspondences between them. There may be many different correspondences between the same $A$ and $B$, but not all of them satisfy some a priori given notion of consistency. Hence, in order to describe exactly legal triples $(A,R,B)$ one has to specify the admissible set $\R$ of consistent correspondence specification together with the respective model pairs that they coordinate, \ie one must specify two mappings $\partial_\spaA:\R\to \xob{\spaA}$ and $\partial_\spaB:\R\to \xob{\spaB}$.

We can now provide the corresponding generalization for arbitrary $n$:
\input{sections/lenses/multispace-fibred}



==> sections/lensesFinal/multispace-total.tex <==



==> sections/lensesFinal/piece-abstract2concrete.tex <==
% -- a piece about concrete interpretation of abstract model space
A prominent example of model spaces is the category of graphs where deltas are encoded as (equivalence classes of) binary spans between them. They are heavily used in the theory of Graph Transformations \cite{gtbook06}. In this way,a delat $u:A\to A'$ can be a deletion or an addition or a combination of both. 
\zd{a bigger version is under "endinput" in the source} 

\endinput

It is also useful to have a more concrete notion of a model space as based on a category \spE\ of models and model embeddings, and then define an update \frar{u}{A}{A'} as a span of embeddings \flar{u_l}{A}{K}  and \frar{u_r}{K}{A'} where $K$ is a submodel of $A$ consisting of all elements preserved by $u$ so that embeddings $u_l$ and $u_r$ specify the deleted and the inserted elements resp. Then a model space \spA\ appears as the category $\Span(\spE)$ for some given \spE. Two ``extreme'' cases for the latter are a) the category of graphs and their inclusions, $\gracat_\subset$, which does not distinguish between objects/references and primitive values/attributes, and b) the Object-Slot-Value model developed in \cite[Sect.3]{me-gttse09} , which does make the distinction between objects and values but does not consider references/links between objects. Integrating a) and b) gives us the category of attributed graphs \cite{gtbook06}. Some of the notions that we axiomatically define below can be given formal definitions for a concrete choice of the category \spE, and we refer to paper \cite{orejas-bx13}, in which some of these definitions can be found for $\spE=\gracat_\subset$.

\zd{In general, I agree, but let's keep this piece for some and finally decide later -- I mean that a systematic use of viewing \spA\ as \Span(\spE) is not assumed but maybe there will be a place where having it will be a useful thing.}


==> sections/lensesFinal/reifiedCorrs.tex <==
\section{Towards lenses with reified correspondences}

\input{figures/diags/ppgPatterns-reflect-reified}
\newcommand\sprx[1]{\ensuremath{\spR(#1)}}
\begin{defin}[Multimodels] \label{def:mmodel-rei}An {\em n-ary corr-reified multispace} is a wide span 
	$\nir=\comprfam{\frar{\prt_i}{\spR}{\spA_i}}{i=1..n}$ consisting of $n$ functors $\prt_i$ with a common source \spR. %	in the category \catcat\ of small categories and functors. 
	Objects of \spR\ are called {\em corrs} or {\em multimodels}, and arrows are their {\em updates}. Each $n$-tuple of models $A=(A_1...A_n)$ determines its own specific category of corrs/multimodels \sprx{A}: objects are pairs $(A, R)$ with $R\in\xob{\spR}$ such that $\prt_iR=A_i$ for all $i=1..n$, and arrows from $(A,R)$ to $(A,R')$ are \spR-arrows \frar{r}{R}{R'} such that $\prt_ir=\id_{A_i}$.
\end{defin}
Given a corr-reified multispace \nir\ as above, if we denote the set of \spR-objects by \Corr, \ie, \Corr=\xob{\spR}, and forget about \spR-arrows, then we get a multispace $(\spA, \Corr)$ as defined in \defref{def:mspace} (below we will denote this multispace by $|\nir|$). The notion of a multimodel as defined in \defref{def:mmodel} is the same as above, but multimodel updates are essentially different notions. For the reified definition, a multimodel update is just an arrow in \spR, say, \frar{r}{R}{R'}, whose boundary is a tuple of feet updates $\prt r=\comprfam{\frar{\prt_ir}{\prt_iR}{\prt_iR'}}{i=1..n}$. For the non-reified \fwk, a multimodel update is a pair $\mathcal{u}=(u, (R,R'))$ with $u=\comprfam{\frar{u_i}{A_i}{A'_i}}{i=1..n}$ being a tuple of feet updates analogously to the reified case,  but the corr-part of the update is just a pair $(R,R')$ of the old and the new corrs.  Clearly, there may be {\em different} reified multimodel updates $r,q,s... \in \spR(R,R')$ over the same feet update, $u=\prt r=\prt q=\prt s...$. We may say that \defref{def:mmodel-rei} is a categorification of \defref{def:mspace} and \defref{def:mmodel}. 

A wide class of reified multimodel spaces is provided  by the following construction. 

==> sections/section2-5.tex <==
%\mysubsubsection{5}{Lens terminology.}
\subsection{Lens terminology}
The domain of change propagation is inherently complicated and difficult to model formally. The lens \fwk\ that approaches the task is still under development and even the basic concepts are not entirely settled and co-exist in several versions (\eg, there are {\em strong} and {\em weak invertibility}, several versions of Putput, and different names for the same property of propagating idle updates to idle updates). This results in a diverse collection of different types of lenses, each of which has a subtype of so called {\em well-behaved (wb)} lenses (actually, several such as the notion of being wb varies), which are further branched into different notions of {\em very wb} lenses depending on the Putput version accepted. % (an attempt to overview this diversity can be found in \cite{me-grand17}). 
The diversity of lens types and their properties, on the one hand, and our goal to provide accurate formal statements, on the other hand, would lead  to overly wordy formulations. To make them more compact, we use two bracket conventions.   

Square brackets.  If we say {\em A wb lens is called {\em [weakly]} invertible, when...}, we mean that using adjective {\em weakly} is optional for this paper as the only type of invertibility we consider is the weak invertibility. However, we need to mention it because the binary lens notion that we generalize in our multiary lens notion, is the weak invertibility to be distinguished from the strong one.  Thus, we mention `weakly' in square brackets for the first time and then say just `invertible' (except in a summarizing result like a theorem, in which we again mention [weakly]).   

Round brackets. If a theorem reads {\em A span of (very) wb asymmetric lenses ... gives rise to a (very) wb symmetric lens ...} it mean that actually we have two versions of the theorem: one is for wb lenses, and the other is for very wb lenses. 


